Code as Anchor, Memory and Metaphor as Support: Learner Experiences with Multi-View Visualizations

Program visualizations are widely used to support novice programmers, yet students often ignore or resist well-designed visual scaffolds. Research on multiple external representations (MERs) offers cognitive design principles for coordinating views, but less is known about what shapes learners' engagement with available representations. We conducted a within-subjects study with 19 undergraduates who had completed CS1 and CS2. Students completed think-aloud tasks, reflective interviews, and webcam-based gaze tracking while using a multi-representational probe with synchronized code, memory, and metaphor views, and Python Tutor, across scope, while loops, and linked lists. Gaze analysis showed that students spent nearly half their time focused on code despite available visual scaffolds. Students without prior experience anchored even more heavily in code and engaged minimally with metaphor views. Interviews identified three factors shaping selective engagement: agency, as students sought control over cognitive effort rather than simply having it reduced; representational fit, as identical designs differed in whether they felt helpful or overwhelming; and legitimacy, as some students avoided metaphorical scaffolds they perceived as childish or insufficiently rigorous for university-level work. These findings suggest that multi-representational tools in computing education require attention to affective and social factors alongside cognitive design. Practical considerations include positioning visualizations as verification instruments, offering toggleable abstraction levels, and framing tools to signal disciplinary legitimacy. More broadly, the themes help explain why cognitively sound visualization tools may fail to engage the students they are designed to help.

==> figures/bars-gaze.tex <==
\definecolor{codeblue}{HTML}{1F77B4}
\definecolor{memorygreen}{HTML}{2CA02C}
\definecolor{metaphorpurple}{HTML}{9467BD}


\newcommand{\barcell}[2]{%
  \begingroup
  \def\W{2.4cm}% bar width (tweak to fit your table)
  \def\H{1.6ex}% bar height
  \begin{tikzpicture}[baseline={(0,-0.2ex)}]
    % background track
    \fill[black!10,rounded corners=0.8ex] (0,0) rectangle (\W,\H);
    % filled bar
    \fill[#2,rounded corners=0.8ex] (0,0) rectangle ({\W*#1/100},\H);
  \end{tikzpicture}~#1\%%
  \endgroup
}

\begin{table}[h]
  \centering
  \small
  \setlength{\tabcolsep}{6pt}
  \begin{tabular}{l>{\raggedright\arraybackslash}m{3.4cm}>{\raggedright\arraybackslash}m{3.4cm}>{\raggedright\arraybackslash}m{3.4cm}}
    \toprule
    \textbf{Task} & \textbf{\Code} & \textbf{\Memory} & \textbf{\Metaphor} \\
    \midrule
    Scope        & \barcell{49.6}{codeblue} & \barcell{31.2}{memorygreen} & \barcell{19.2}{metaphorpurple} \\
    While Loops  & \barcell{42.1}{codeblue} & \barcell{38.7}{memorygreen} & \barcell{19.2}{metaphorpurple} \\
    Linked Lists & \barcell{38.8}{codeblue} & \barcell{46.8}{memorygreen} & \barcell{14.4}{metaphorpurple} \\
    \bottomrule
  \end{tabular}
  \caption{Median dwell percentages by task, with inline bars for \Code, \Memory, and \Metaphor.}
  \label{tab:task-dwell-mini}
\end{table}


==> notes/ambiguity.tex <==
- Ambiguity sometimes arises not because things are themselves unclear, but because they may be understood in different contexts, each suggesting different meanings. \cite{gaver2003ambiguity}

- - ambiguity can be a design resourc:
    
    - It provokes curiosity, reflection, and personal interpretation.
        
    - It encourages deeper and more personal engagement with systems.
        
    - It allows users to appropriate systems into their own contexts rather than being constrained by fixed meanings.

- 1. **Ambiguity of Information**
    
    - Originates in the artefact itself (e.g., incomplete, imprecise, or contradictory displays).
        
    - Forces users to interpret or trust uncertain information.
        
2. **Ambiguity of Context**
    
    - Arises from multiple or conflicting sociocultural discourses.
        
    - Example: Duchamp’s *Fountain* as both urinal and artwork.
        
    - In design, users may repurpose or reinterpret products (e.g., mobile phones as baby rattles).
        
3. Ambiguity of Relationship
    
    - Emerges from the user’s own stance and values.
        
    - Designs invite self-reflection, ethical questioning, or imagining alternative roles (e.g., Prayer Device, Telegotchi).

- Slow technology and reflexive design \cite{cox2016design,hallnas2001slow, sengers2005reflective} focus on how design can encourage and aid reflection

- Others have argued that technology can be designed to facilitate “uncomfortable interactions” \cite{benford2012uncomfortable}, where negative emotions server to enrich the user experience \cite{fokkinga2013ten}. The aim of this approach is not to create long term discomfort or pain. Instead, the approach is based on the idea that many activities that make us uneasy are nonetheless worthwhile.

- “critical design” approaches promote reflection and critique by subverting assumptions and expectations, often through making technology “unfriendly” to users \cite{dunne2008hertzian, pierce2014undesigning}.

- \cite{cox2016design}: How can introducing friction to interactions improve the overall experience? Work from cognitive psychologists \cite{kahneman2011thinking} suggests that we have two modes of thought: System1 and System2. System1 is the fast, automatic system that guides most of our behaviours and is employed during the automatic, mindless interaction that we are concerned with in this paper. System2 is the slower, more deliberate system that is employed when we are more mindful and conscious of what we are doing. We are arguing that System2 could and should be invoked through careful interaction design in a way that advantages users. Here we define mindful as deliberate and intentional rather than as an awareness and non-judgmental acceptance of the experience of the present moment, as is meant by the term “mindfulness” (\cite{kabat2009full})

- A microboundary is an intervention that provides a small obstacle prior to an interaction that prevents us rushing from one context to another. It does this by creating a brief moment in which we might reflect on what we're doing. \cite{cox2016design}


- Lockouts have been shown to improve attentiveness, partly because enforcing a brief pause stops people clicking mindlessly through modal dialogs (e.g., \cite{egelman2008you}), and partly because a pause gives people a chance to more carefully plan their actions before they execute them \cite{back2010locked, brumby2013recovering, o1999planning}.

==> notes/desirable-difficulties.tex <==
- Basically, any time that you, as a learner, look up an answer or have somebody tell or show you something that you could, drawing on current cues and your past knowledge, generate instead, you rob yourself of a powerful learning opportunity. \cite{bjork2011making}

- Our conceptualization of perceived effort is based on the recent review paper by Scheiter et  al. (2020), who indicated that ratings of experienced effort are in fact a type of metacognitive judgment that result from heuristic processing and are therefore prone to biases. \cite{de2023worth}

- Having the latter, lower effort option as an opportunity increases the perceived costs of the desirably difficult strategy: taking the practice test. The objective benefit of taking the practice test is constant, yet it may feel subjectively higher when the student has the peer’s summary available.  \cite{kurzban2013opportunity}

- decisions about how learners invest effort are often made considering perceived effects on learning \cite{kirk2019perceiving}

- Perceptions of fluency refer to the ease or difficulty with which a task is processed and, as such, describe a sheer subjective feeling \cite{reber2017processing}

- What learners term “ease” can be interpreted as experiencing a greater sense of fluency, which they typically associate with more positive learning outcomes. If the concept of fluency plays a dominant role in how learners shape experiences of effort, then they will be reluctant to engage in desirable difficulties, as desirable difficulties are characterized by the opposite, that is, experiences of disfluency and difficulty. \cite{kurzban2013opportunity}

- When learners assume a goal-driven approach, they judge that high effort is a positive sign of learning -- also termed as passive vs. active load \cite{klepsch2021making}

- Baars et al.’s (2020) meta-analysis shows that the goal-driven approach is less common among learners than the data-driven approach. \cite{baars2020relation}

- productive struggle suggests that experiencing a moderate level of frustration can actually be beneficial. \cite{young2024productive}

- When students persevere through frustration, they develop a greater sense of accomplishment, resilience, and a deeper understanding of the content. \cite{young2024productive}
    - The key is to provide support and guidance during this process to prevent frustration from turning into a barrier that hinders learning. \cite{young2024productive}

- a lack of the proper encouragement can promote mathematics anxiety, which can manifest into fear or despair \cite{goldin2000affective}

==> notes/future-work.tex <==
Audio as another dimension
- some people learn a lot through podcasts
- physical computing

==> notes/gaze.tex <==
- Eye gaze has been shown to be closely linked to cognitive processing \cite{just1976eye, just1980theory, underwood2004inspecting}, mental workload \cite{pfleging2016model}, reading comprehension \cite{ahn2020towards}, and emotional expression \cite{wells2016identification}.

- Just and Carpenter \cite{just1976eye} found negligible lag between eye fixations and cognitive processing, causing them to suggest that what we see is also what we think about.


- Fixation duration alone is a strong measure to distinguish novice users from experts \cite{aljehane2023studying, ishimaru2016towards}, infer student engagement in extracting and processing information from a set of given sources \cite{ibrahim2023students}, distinguish reading behaviors of users for different tasks such as comprehension and proofreading \cite{kaakinen2010task}, and even predict query terms during information processing with high accuracy \cite{davari2020role}.

- Novices also tend to have a significant number of fixations and higher gaze time compared to experts when they comprehend code. \cite{aljehane2023studying}

- experts showed the ability to omprehend and finish the task using fewer source code elements than novices. \cite{aljehane2021determining}


==> notes/methods.tex <==
Gazer:

https://cs.brown.edu/people/apapouts/papers/ijcai2016webgazer.pdf



==> notes/new-related.tex <==
% ===============================
% Notes on *How Domain Experts Create Conceptual Diagrams and Implications for Tool Design*
% Source: Ma’ayan et al., CHI 2020
% ===============================

* **Main contrib**:

  * First empirical study on how domain experts make conceptual diagrams
  * Semi-structured interviews w/ 18 experts across math, CS, architecture, ed, etc.
  * Identifies *representation finding* as key step → how people choose/ invent visual mappings for abstract concepts
  * Analyzes trade-offs between PL (programming language) and DM (direct manipulation) diagramming tools
  * Surfaces ad-hoc reuse/versioning practices
  * Proposes **“Natural diagramming”** framework → 4 opps: exploration support, representation salience, live engagement, vocabulary correspondence

* **Key defs/ideas**:

  * *Conceptual diagrams* = visual reps of abstract models/relationships (≠ data viz of concrete facts)
  * *Representation finding* = mapping domain constructs → visual forms (shapes, colors, layout)
  * PL tools = code/spec-driven (TikZ, GraphViz, etc.) → precise, automatable, high local control, but steep learning curve + slow feedback
  * DM tools = GUI-based (Illustrator, draw\.io, etc.) → immediate feedback, good global layout control, but poor abstraction/reuse
  * *Natural diagramming* = tools that let you express diagrams the way you think them

* **Findings**:

  * Experts either adapt existing conventions or invent new visual metaphors depending on domain norms
  * Sketching central for iterating on representations before moving digital
  * PL users often build macros, DSLs, parameterized diagrams → better reuse but costly upfront
  * DM users do manual duplication/versioning (e.g., multiple canvases), use “cheat sheets” for colors/styles
  * Many keep personal libraries of reusable elements (organized by rep, not topic)
  * Version control for diagrams is messy: PL files = text-based but low-level; DM = visual but no textual diff

* **Limitations of current tools**:

  * Gap between drafting (loose sketching) and crafting (precise final diagram)
  * Poor support for mixed lateral (big-picture) + vertical (detail) exploration
  * Representation mappings not first-class → buried in low-level ops
  * Limited “liveness” esp. in PL tools; DM tools lack abstraction
  * Weak correspondence between user’s domain vocab & tool’s ops

* **Implications / design opps**:

  1. **Exploration support** → fluid undo/backtracking, support both lateral + vertical refinement, better history mgmt
  2. **Representation salience** → treat mappings as first-class objs, enable abstraction, scalable reuse
  3. **Live engagement** → unify DM immediacy + PL precision (e.g., bidirectional editing, live programming)
  4. **Vocabulary correspondence** → allow domain-specific vocab/constraints, high-level relational specs

* **Related work used**:

  * Cognitive benefits of diagrams (Larkin & Simon, Hegarty & Kozhevnikov)
  * Data viz tool “waves” (Satyanarayan et al.) → conceptual diagramming still in early stage
  * Sketching in STEM/SE, constraint-based design, program synthesis for abstraction

* **Limitations of study**:

  * Only individual work practices; collaboration not examined
  * Small N (18), interview-based, self-reported practices
  * Tool suggestions speculative; not validated experimentally

* **Method**:

  * Semi-structured interviews, 30–80min, 18 participants (faculty, PhD, devs, K-12 teacher)
  * Thematic coding → clusters: representation, tool choice, reuse/versioning

* **Cool bits**:

  * People literally branch “fractally” on artboards to explore ideas
  * Cheat sheets with hex codes, stroke settings
  * Personal TikZ “vault” of every diagram ever made
  * PL automation pays off only if you need lots of similar diagrams; not worth for one-offs

% ===============================
% Notes on *Notional Machines in Computing Education: An Examination into the Role, Value, and Challenges of Mental Models of Computer Systems*
% Source: Sorva et al., TOCE 2013
% ===============================

* **Main contrib**:

  * Clarifies and consolidates the term **notional machine** in computing ed research
  * Reviews lit + authors’ own analysis → argues NM = critical for learning prog & systems
  * Identifies ambiguity in term usage, proposes structured def
  * Suggests research + pedagogical directions for making NMs explicit & effective in teaching

* **Key defs/ideas**:

  * *Notional machine* = “an abstraction of the computer that includes the concepts and operations programmers need to reason about when they write and read programs”

    * Not real hardware → idealized conceptual model
    * Often partial + tailored to a purpose
  * Relates to mental models, program execution models, operational semantics, computational models
  * Role: help learners form accurate mental models, avoid misconceptions, understand program behavior
  * NMs can be implicit (in teacher’s mind) or explicit (taught with visuals, metaphors, animations)

* **Findings / analysis**:

  * Lit shows NM term inconsistently defined (sometimes conflated w/ execution model, sometimes narrower)
  * Many textbooks/tools implicitly assume an NM but don’t make it visible to students
  * Misconceptions often due to mismatch between student’s NM & intended NM
  * Multiple NMs may be needed across contexts (e.g., CS1 imperative, later concurrency)
  * Good NMs balance simplicity w/ faithfulness; too much detail overwhelms, too little misleads
  * Teachers often use analogies (e.g., “mailboxes” for variables, “tape” for memory) → risk oversimplification

* **Limitations / challenges**:

  * Risk: students cling to simplified NMs, resist moving to more accurate ones
  * Hard to design NMs that are correct, comprehensible, and pedagogically effective
  * Little empirical research on *how* students actually internalize NMs
  * NMs may be tool-specific, limiting transfer

* **Implications**:

  * Educators should make NMs explicit & discuss limits
  * Use consistent metaphors, avoid silent shifts in NM
  * Support progression from simple → richer NMs
  * Tools/visualizations should clearly communicate NM assumptions
  * Need more research on NM learning trajectories

* **Related work**:

  * du Boulay’s five facets of learning prog → NM maps to “notional machine facet”
  * Norman on mental models
  * Winslow, Pane on student misconceptions
  * Work on program visualization (BlueJ, Greenfoot, etc.)

* **Method**:

  * Lit review + conceptual analysis, not empirical
  * Authors draw from examples in textbooks, teaching practice, ed tools

* **Extra notes**:

  * NM ≠ architecture-level model; more like a pedagogical VM in your head
  * Can be explicit in diagrams, animations, metaphors, formal rules
  * Danger: “Magic happens” gaps in NM = black boxes learners never unpack

% ===============================
% Notes on *Program Visualization as a Debugging Tool for Novices*
% Source: Brusilovsky, 1993
% ===============================

* **Main contrib**:

  * Argues for a *non-traditional role* of program visualization → as a debugging tool for novice programmers
  * Describes ITEM/IP & ITEM/IP-11 environments → Turingal/Tortoise mini-languages
  * Introduces **explanatory visualization** → step-by-step NL explanations alongside visual execution
  * Reports small classroom study comparing plain visualization vs explanatory visualization for debugging

* **Key defs/ideas**:

  * *Program visualization* = graphical animation of program execution, showing flow of control, variable states, etc.
  * *Intelligent program debugger* (IPD) = analyzes student code, finds errors, diagnoses misconceptions
  * ITEM/IP = visual interpreter + evaluation module (test-based comparison to model solution)
  * *Faulty test* = test case where student program output ≠ model output
  * *Explanatory visualization* = natural language narrative + standard visualization explaining why each step occurs (“While condition false → skip loop body…”)
  * Observation: students sometimes watch execution but don’t understand; language layer helps

* **Findings / results**:

  * In first deployment (1985), \~80% of student errors fixed just by stepping through faulty test with visualization; \~20% needed teacher
  * New study w/ 30 students, 14-lesson course, \~167 “debug interviews”:

    * Only results shown → 19% fixed
    * Standard visual exec → 39% more fixed
    * Simulated explanatory viz → 20% more fixed
    * Other means (human explanation) → remaining 16%
  * Conclusion: visualization is effective; explanatory layer boosts effect significantly

* **Limitations**:

  * Explanatory viz in experiment was simulated by human assistants (not fully automated)
  * Small sample size; early-stage evaluation
  * Mini-language context only (Tortoise), may not generalize to mainstream languages
  * Not a full intelligent debugger — still relies on faulty test identification + human guidance

* **Implications / ideas**:

  * Adaptive visualization → match to student’s knowledge level
  * IPD could choose “best” faulty test for clarity (test selection matters)
  * Combine AI + visualization for more effective debugging
  * Visualization shouldn’t replace AI reasoning — both can complement

* **Related work**:

  * du Boulay, Dettori, Lemut on cognitive models & environments
  * Eisenstadt et al. on software visualization
  * Brusilovsky on adaptive visualization (1992)
  * Vanneste & Olive on Pascal learning envs

* **Cool bits**:

  * Explanations grounded in visible program state (e.g., “tortoise stands on letter ‘B’, not ‘A’”)
  * Students often can fix bugs without full diagnosis if execution makes failure *obvious*
  * The “best” faulty test might not be the first one found — picking a pedagogically optimal one is key

% ===============================
% Notes on *Omnicode: A Novice-Oriented Live Programming Environment with Always-On Run-Time Values*
% Source: Koo et al., UIST 2017
% ===============================

* **Main contrib**:

  * Presents **Omnicode**, a Python-based live prog env for novices
  * Shows *always-on runtime values* directly in code editor → variable values + visual previews inline
  * Aims to make debugging & comprehension easier without needing print statements or breakpoints
  * Evaluation with novices shows faster bug detection & comprehension vs baseline

* **Key defs/ideas**:

  * *Always-on runtime values* = continuous display of var values after each line, updated live as code runs
  * Works for scalars, collections, images (previews), audio (waveform), etc.
  * Inspired by live programming, spreadsheet immediacy, program visualization research
  * Editor merges code + output in one space → reduces context switching
  * Omnicode replays program execution over timeline slider → see state evolution step-by-step
  * Designed for sequential, event-driven, & loop-heavy beginner code patterns

* **UI features**:

  * Inline value annotations → right-aligned in code view
  * Visual previews for media types
  * Timeline scrubber → navigate through past states
  * Play/pause execution
  * Works w/ syntax highlighting, autocompletion
  * No need to insert logging statements — all vars tracked automatically

* **Findings / results**:

  * User study: novices (mostly no Python exp) given debugging tasks

    * Omnicode group fixed bugs faster + reported better understanding of what code did
    * Fewer redundant edits; more direct jumps to relevant lines
    * Especially helpful for loops & nested structures → seeing evolving var values key
  * Participants liked visual previews for complex data (lists, images)
  * Some info overload complaints — too many inline values at once in bigger programs

* **Limitations**:

  * Focused on small/medium programs; may not scale to large codebases
  * Primarily for teaching/debugging, not production dev
  * Python only (prototype)
  * Always-on values could clutter editor for experienced users

* **Implications**:

  * Bringing outputs closer to code reduces cognitive load for novices
  * Inline + visual + replay timeline → combines strengths of program visualization + live coding
  * Could integrate w/ intelligent tutoring for targeted feedback
  * Potential to adapt info density to learner level (adaptive display)

* **Related work**:

  * Live coding envs (Light Table, Bret Victor’s demos)
  * Program visualization for novices (BlueJ, PythonTutor)
  * Immediate feedback & liveness in educational IDEs
  * Work on embedding runtime info in code editors

* **Cool bits**:

  * Variable’s “life story” visible without extra instrumentation
  * Images/audio literally preview inside code — debugging multimedia assignments super direct
  * Scrubbing time feels like “video editing” but for code execution

% ===============================
% Notes on *Finding Causes of Program Output with the Java Whyline*
% Source: Ko & Myers, CHI 2009
% ===============================

* **Main contribs**

  * Java Whyline tool: lets devs ask “why did” / “why didn’t” Qs about program output
  * UI re-design from Alice Whyline → scales to complex Java apps
  * Direct manipulation Qs on output primitives (graphics, text, exceptions) + abstraction-aware Qs
  * Interactive timeline = answer view + followup Q interface + bookmark/nav aid
  * “Familiarity” heuristic filters questions & annotates output/code to focus on dev-authored/known code
  * Empirical eval: Whyline users 3× as successful, \~2× faster than breakpoint debugger in study

* **Key ideas / defs**

  * Debugging = hypothesis-driven; devs trace backwards to find causes (program slicing, focus points)
  * *Why did* Q → reason backwards from visible output to cause before render time
  * *Why didn’t* Q → why something didn’t occur after a time point (harder, slower due to exhaustive static analysis)
  * “Primitive outputs” = lowest-level visible entities: lines, shapes, console text, exceptions
  * Familiar code = code declared by dev or directly referenced by such code → reduces noise, hides unfamiliar API internals (crosshatching)
  * Followup Qs: control dep (“why executed?”), data deps (“where did obj/value come from?”), skip through passthrough calls unless shift pressed
  * Timeline viz: x-axis = time, y-axis = thread, events = method calls/branches (green), assignments (blue), API/unrecorded (grey/xhatch), selected event (orange)

* **Method / UI design**

  * Works on recorded executions (no live debugging) → shareable traces, less perf hit
  * Question-asking mode: only shows output + time slider (avoid code bias)
  * Answer mode: code + call stack + locals + event timeline + followup Qs
  * Time slider with I/O markers (mouse, keyboard, repaint) → filterable by type
  * Auto-arranges relevant source files, highlights dependencies, collapses irrelevant code context
  * Allows stepping forward/backward in control/data flows like debugger, plus “undo” for nav peeking

* **Eval setup**

  * Between-subjects: Whyline vs breakpoint debugger (same UI shell, diff debug backend)
  * 20 MS SE students, \~1.5 yrs industry exp median, good Java skills
  * Tasks = 2 real ArgoUML bugs:

    1. Remove checkbox (string label hidden in compressed localization)
    2. Dropdown missing duplicate class names (set uniqueness issue)
  * Measured success, completion time, file views/min, median distance to “key” function (prog dep graph)

* **Results**

  * Task1: Whyline all 10 succeeded vs control 3; Whyline \~½ time; fewer files/min but closer to key fn
  * Task2: Whyline 4 succeed vs control 0; no time diff; Whyline viewed more files/min (dep spread)
  * Whyline users asked few, targeted Qs; control relied on text search/breakpoints
  * High enthusiasm quotes (“I love it!”, “This will really help” etc.)

* **Limitations**

  * Small sample, not rep. of all Java devs; no code editing in either cond. → unnatural constraints
  * Unfamiliar codebase (ArgoUML) → results may differ w/ familiar code
  * “Why didn’t” Qs slow, less used; sometimes hard to find desired Q in menu
  * Tool localizes buggy method well but doesn’t explain why method buggy (no domain knowledge)
  * Risk: too focused on subset of code → less serendipitous discovery

* **Related work**

  * Program slicing, anomaly detection, reverse debugging
  * Non-programming “why” systems (ACT-R, AI KBs, e-commerce debugging)
  * Influence from studies on dev question types, focus points, fact finding

* **Takeaways**

  * Asking about output first avoids wasted speculation → big gains in success & speed
  * UI must balance Q specificity, filtering, and showing deps clearly
  * Potential teaching tool for better diagnostic habits (less assumption, more obj. tracing)


% ===============================
% Notes on *Projection Boxes: On-the-fly Reconfigurable Visualization for Live Programming*
% Source: Lerner, CHI 2020
% ===============================

* **Main contribs**

  * Projection boxes = always-on runtime value vis. for live programming
  * Core idea: start from *full semantics* (all runtime states), project to subset for display
  * Expressive enough to encode old vis. paradigms (Victor 2012, Babylonian probes, etc.) + new ones
  * Provides on-the-fly reconfigurable views → helps manage info overload
  * Implementation: VERSABOX (Python, VS Code plugin) w/ presets + keyboard-controlled projection config
  * User study: low distraction, high perceived utility, diverse preferences → strong case for customizability

* **Key defs / terms**

  * *Full semantics*: set of all program states (var→value maps) at each line during exec
  * *Projection*:

    1. pick subset of values to show (which lines, vars, loop iters)
    2. choose row vs column order (vars as cols vs vars as rows) for space mgmt
  * *Basic projection box*: floating table aligned to code line, cols=vars, rows=states, “#” col=iteration count, empty rows for skipped branches
  * *View modes* (in VERSABOX): Full, Summary (cursor + return), Row (Victor), Stealth (none)
  * *Stealth mode*: hide all boxes (projection out)

* **Related work position**

  * Builds on Victor Visualization, Omnicode, Babylonian editor, YinYang, Theseus, etc.
  * Distinctive points: generalizable vis. framework + quick reconfigurability while coding

* **Formative study findings**

  * Big variance in when/how devs want feedback → coding vs debugging mode; novice vs expert; linear vs non-linear code writing
  * Need for presets for beginners + fast toggling (keyboard better than mouse)
  * Desire for ability to turn vis off (stealth mode)

* **Implementation notes**

  * Python-specific in VS Code; runs funcs on unit tests after each change to collect state data
  * Var config syntax: `add|del|keep [@all] VarRegExp` (supports wildcards/regex)

* **Eval setup**

  * Lab study, N=10 (3–9 yrs programming exp, 1–5 yrs Python)
  * 6 coding tasks (list stats, inserts into sorted list, string parsing)
  * Survey Qs (Likert 1–5) + interviews + observations

* **Results**

  * **Utility**: avg 4.7 (helped write correct code), 4.8 (easy to use)

    * 4 observed uses: immediate bug catch, guide next step, whole-program test after writing, learn/confirm language feature behavior
    * Acts as “inline interpreter” in context of surrounding code
  * **Distraction**: avg 1.2 (very low); on-the-fly config key to keeping focus
  * **Customizability**: avg 4.4 for var config usefulness; prefs split across views (Row=6, Full=3, Summary=1, Stealth=0)

    * Tradeoff: Row → see per-line changes easily; Full → see var relationships
    * Coping strategies: stick to Row + add vars; stick to Full + remove vars; switch between
    * Keyboard shortcuts preferred for fine-grained config during coding

* **Takeaways**

  * T1: If distraction is low, always-on vis can be used opportunistically at diff granularities
  * T2: On-the-fly config mitigates overload + distraction
  * T3: Strong inter-user preference variance → design should prioritize customizability
  * T4: Mouse use is avoided mid-coding for config; keyboard shortcuts essential

* **Limitations**

  * Small lab sample; only unit-test-sized inputs; Python only; doesn’t handle large datasets/I-O heavy code well yet
  * Needs adaptation for other paradigms (func/constraint-based) → new placement/state vis challenges

* **Conclusion**

  * Projection boxes = flexible, customizable always-on vis framework
  * No single “best” config → design must enable rapid tailoring per user/task


% ===============================
% Notes on *Working Memory in Programming: The Role of Domain Knowledge*
% Source: Fleming, CHI 2013
% ===============================

* **Main contribs**

  * Lab study linking working memory (WM) performance to debugging success
  * Hypothesis: domain knowledge (DK) moderates WM demands during programming tasks
  * Measured verbal WM, visuospatial WM, programming DK, and debugging task success
  * Found: verbal WM → stronger predictor when DK low; when DK high, WM less critical
  * Suggests teaching approaches: build DK to reduce WM bottlenecks

* **Key defs / concepts**

  * *Working memory*: temp storage/manipulation of info during cognitive tasks (Baddeley model: central exec + verbal + visuospatial subsystems)
  * *Domain knowledge*: long-term mental representations of relevant facts/concepts, here: programming concepts, syntax, idioms
  * WM capacity interacts w/ DK → cognitive load theory framing
  * *Debugging task* = understanding output + locating + fixing bug in short Java program

* **Method**

  * N=65 undergrads, all intro CS course completers
  * Measures:

    * verbal WM → operation span task (math+letter recall)
    * visuospatial WM → symmetry span task (grid pattern recall)
    * DK → multiple-choice programming concepts test
    * debugging perf → success/failure + time
  * Debugging tasks: 4 short Java programs w/ seeded bugs (loop bounds, var init, conditionals)
  * Covariates: prior GPA, course grade, gender, programming experience self-report

* **Results**

  * Correlations: verbal WM pos. correlated w/ debugging perf; visuospatial WM weaker link
  * Regression: DK main effect strong; interaction DK×WM significant → WM important only for low-DK group
  * No significant gender diff; exp years not strong predictor after DK accounted for
  * Time-on-task: high DK group solved faster; low DK group slower, more failures if low WM

* **Discussion / implications**

  * High DK frees WM for problem solving → schema automation idea
  * In teaching:

    * early learners → WM load high → scaffold tasks, avoid extraneous cognitive load
    * later learners → WM load less critical → focus on DK building and transfer
  * Could explain mixed findings in prior WM-programming studies (didn’t consider DK moderation)

* **Limitations**

  * Lab tasks small/simple → not representative of large, real-world code
  * DK measure = MCQ test, might not capture procedural fluency
  * Sample = mostly young CS students → generalizability limited
  * Cross-sectional, not causal over time

* **Related work**

  * WM & problem solving (Sweller, Baddeley)
  * WM in math/CS education
  * DK’s role in expertise dev (Chi, Anderson)

* **Conclusion**

  * DK is key moderator: low DK → WM capacity matters; high DK → WM less bottleneck
  * Instruction: manage WM load early, build DK to reduce reliance on WM over time


% ===============================
% Notes on *Augmenting Code with In Situ Visualizations to Aid Program Understanding*
% Source: Hoffswell, Satyanarayan, Heer, CHI 2018
% ===============================

* contrib: propose + eval “in situ” code visualizations → show runtime var state *inside* source code, not in separate debugger view

* goal: reduce “gulf of evaluation” between code & behavior; keep flow; avoid context-switching

* design space:

  * data type = value (single) vs set (collection)
  * level of detail = data (exact/distribution) vs change (update indicator)
  * temporality = snapshot vs sequence

* visualization types identified (10 total):

  * value-snapshot: exact value
  * value-sequence: line chart, horizon chart
  * set-snapshot: histogram, heatmap
  * set-sequence: line chart, horizon chart
  * change-level: indicator (value-snapshot), tick/timeline (value-sequence), modification indicator (set-snapshot), stacked area (set-sequence)

* extra: miniaturizations (tiny underlines), color coding by type, hover interactions (tooltips, linked highlighting), consistent widths

* placement design space: 12 techniques (right/left of token, above/below line, inline-transparent/opaque, expand-inline/expand-below, inline-start/end, left/right margin)

  * trade-offs: reflow, spacing, occlusion, width, alignment; guidance on when to choose which for salience vs unobtrusiveness vs comparability

* usage scenario: scatterplot panning bug; in situ viz helps see that point size changes unexpectedly b/c xDomain wrong → bug in xMin/xMax updates

* related work they build on:

  * debugging tools w/ separate views (Whyline, FireCrystal, Theseus)
  * algorithm visualizations (Online Python Tutor, algoviz)
  * text augmentation (sparklines, scented widgets)

* evaluation setup:

  * domain: novice Vega users (18 students)
  * 2 conditions: baseline Vega editor (tooltips only) vs augmented (tooltips + in situ viz)
  * tasks: 2 Vega programs per participant (mix of bugs + normal)
  * metrics: task grade, time, confidence, self-reported speed/accuracy; helpfulness, interpretability, intrusiveness ratings for each viz type
  * viz types actually used in study: indicator, line, tick, histogram (placed to right of token)

* results:

  * marginally significant grade improvement (\~+2 points) w/ in situ viz; no sig effect on time/confidence; strong positive self-reported speed & accuracy
  * line viz rated most helpful; value/indicator/line rated most interpretable; low intrusiveness scores overall
  * qualitative: faster to see changing vars; more confident; direct link from code→behavior; but sometimes unclear for complex/nested data fields

* limits:

  * tested only w/ Vega (simple, reactive); need generalization to other reactive/dataflow langs (React, Elm)
  * current design doesn’t surface variable scope or nested structure well; object simplification might hide important info
  * salience can be distracting if not tuned to task; no adaptive salience yet
  * no dynamic change of viz type during runtime

* future: adaptive placement/salience, better handling of nesting/scope, application to other langs/frameworks, integration w/ efficient logging systems (e.g. Dolos)


% ===============================
% Notes on *The Effect of Richer Visualizations on Code Comprehension*
% Source: Asenov, Hilliges, Müller — CHI’16
% ===============================

* main contrib: first systematic user study comparing mainstream syntax highlighting vs. two richer code visualizations (v-med, v-high) for same language/code
* richer visualizations → faster detection of code features (21%-75% time reduction in some Qs)
* no measurable increase in visual overload (even if users *felt* overwhelmed)
* tool used: Envision structured editor (v-med = moderate enhancements; v-high = more extensive, colors/icons/bg highlights)
* RQs:

  * RQ1: effect on speed of detecting features?
  * RQ2: effect on correctness?
  * RQ3: visual overload effect on unenhanced constructs?
* H1: speed improves for enhanced constructs; H2: unenhanced unaffected; H3: correctness unaffected
* visual variety levels:

  * v-low = Eclipse default syntax highlighting
  * v-med adds: alt bg for lists, param names above types, dashed line between sig/body, outlined blocks instead of braces
  * v-high adds: bg color for constructs, icons for keywords, orange method call text, bg for some expressions
* theory ref: Semiology of Graphics (SoG) — more visual variables → better perception
* method:

  * 33 devs (≥1 yr Java exp, avg 5.5 yrs)
  * tasks: 15 yes/no Qs about method structure (3 Q categories: no enhancement, enhanced by both v-med/v-high, enhanced mainly by v-high)
  * stimuli: screenshots of 298 methods from jEdit, fitting on one screen, no comments
  * within-subject design, randomized order, drop first 3 answers per combo to reduce learning effect
* results:

  * H1 mostly holds except Q6
  * H2 holds (Q1-Q5 unaffected)
  * correctness \~ same (ceiling effect)
  * v-high > v-med > v-low in speed for enhanced Qs
  * user pref: v-med ranked highest; many found v-high overwhelming but still faster
* related work: Green & Petre (notation usability), Hendrix (control structure diagrams), Feigenspan (bg colors in SPLs), Hakala (syntax highlighting study → no diff)
* limitations:

  * limited Q set, simple tasks only
  * only one Java code base (jEdit)
  * only 2 specific visualizations tested
  * measure only comprehension, not writing/debugging
* recs for tool designers:

  * more color variety + highlight more constructs
  * easy to implement → revertible
* future work: aesthetics of rich visualizations, effect on other dev activities (writing, debugging)


% ===============================
% Notes on *Understanding Trigger-Action Programs Through Novel Visualizations of Program Differences*
% Source: Zhao, Zhang, Wang, Littman, Lu, Ur — CHI’21
% ===============================

* context: TAP = if-this-then-that automation rules, end-user friendly but reasoning/debugging errors common
* problem: when TAP programs evolve, users need to compare variants (original vs modified candidates) → hard to tell if behavior matches goals, esp. w/ many rules & complex interactions
* main contrib:

  * novel *semantic-dif* UIs comparing TAP programs based on outcomes or high-level properties, not just syntax
  * algorithms using formal modeling (transition systems) to detect & visualize behavioral differences
  * 3 semantic-dif UIs:

    * **Outcome-Dif: Flowcharts** → all situations w/ different outcomes between 2 variants, visualized
    * **Outcome-Dif: Questions** → user selects desired outcomes per situation, scores variants accordingly (scales to many variants)
    * **Property-Dif** → contrasts safety properties always/never true (abstract guarantees)
  * 107-participant between-subject online study vs controls (Rules, Text-Dif) → semantic-dif helped more on long/complex program comparisons
* terminology:

  * factor → entity in system (device, user, env), attribute → aspect of factor
  * variable = factor+attribute, state = persistent truth, event = instantaneous change
  * TAP rule = IF trigger WHILE conditions THEN action (event-state trigger type)
  * variant = program version being compared
* related work:

  * TAP reasoning error studies (Yarosh & Zave, Huang & Cakmak, Brackenbury, Brush, Palekar)
  * end-user programming aids (Whyline, EUDebug, My IoT Puzzle, ITAD)
  * diffs in other domains (GitHub split/unified diffs, Google Docs history)
* UI designs:

  * **Rules** = list each program alone (control)
  * **Text-Dif** = GitHub-like split diff, aligns & highlights added/deleted/modified rules
  * **Outcome-Dif** = compares behavior under identical situations
  * **Property-Dif** = lists abstract “always/never” statements for each program, sorted into shared vs unique
* algorithms:

  * model TAP variant as *transition system* (states = Cartesian product of relevant variables, edges = possible events; rules redirect edges)
  * outcome diff: find reachable states common to all variants, compare out-transitions → situations w/ diff outcomes
  * property diff: find unreachable nodes (S-properties) + self-transitions (E-properties), minimize logic to abstract/general properties
* user study:

  * 6 tasks, varied complexity (# rules, variables, variants) & type of difference (outcomes vs properties)
  * findings:

    * simple tasks: all interfaces similar, Rules OK
    * complex tasks: semantic-dif → more correct answers, less mental demand than controls
    * Outcome-Dif: Flowcharts strong for few variants/few diff situations
    * Outcome-Dif: Questions better for many variants or abstract goals
    * Property-Dif good when abstract properties matter, but can confuse when none differ
    * time-to-complete not significantly different across interfaces
* limitations:

  * short-term, online study (no long-term adoption data)
  * many participants had programming/IoT familiarity despite aiming for non-technical
  * TAP-specific algorithms, but concepts may generalize
* implications:

  * semantic comparisons help end-users select/debug TAP programs in complex scenarios
  * could integrate into TAP platforms, especially for debugging and variant selection


% ===============================
% Notes on *VizProg: Identifying Misunderstandings By Visualizing Students’ Coding Progress*
% Source: Zhang et al., CHI 2023
% ===============================

* **Main contribs**

  * Interviews w/ prog instructors → real challenges in live coding exercises, esp. large classes
  * New 2D Euclidean map rep of students’ code in real-time → x-axis = progress toward correct soln (edit dist), y-axis = problem-solving approach (semantic sim)
  * Keystroke-level tracking + clustering for live monitoring
  * Interface lets instructor zoom from class-level to individual code + send lightweight feedback
  * Empirical study vs OverCode baseline → more misunderstandings found, faster detection

* **Key ideas / defs**

  * *DG1*: View students’ progress in real-time
  * *DG2*: Compare diff approaches
  * *DG3*: Inspect progress at diff granularities (group ↔ individual)
  * Uses **CodeBERT** for code vectorization (handles syntax errors)
  * Norm() function = strip comments, spacing, rename vars v0..vn, remove prints
  * **NEAR\_APPROACH(c)** = most semantically similar correct sols → determines y-pos
  * **NEAR\_EDIT(c)** = closest correct sols by edit dist → determines x-pos
  * Clustering via OverCode for grouping correct approaches vertically
  * Needs *PAST\_CODE* repo of solutions to seed map (better if diverse)

* **UI elements**

  * **2D map view**: dots = students, color = correctness (orange=wrong, blue=correct), trajectory lines = history, vertical bands = approaches, horizontal motion = progress
  * **Solution-centered view**: stats + list of students w/ that soln + code hist
  * **Progress detailed view**: crop map region → see code/errors grouped by freq/type, color-coded correctness, line highlight for error loc

* **Related work it builds on**

  * Codeopticon (real-time per-student view, but not scalable)
  * OverCode (post-hoc clustering, no real-time)
  * Code visualization: AST/edit dist maps, semantic sim mapping, clustering incorrect code (MistakeBrowser, FixPropagator)
  * Real-time code sharing platforms (CoCode, Codechella, PuzzleMe, etc.)

* **Limitations**

  * Needs existing repo of solutions to build space (cannot start cold unless incremental PCA/TSNE implemented)
  * Progress not always visible in code (pseudo-code, thinking stage) → map can mislead if not interpreted carefully
  * Norm() still misses some semantically irrelevant diffs (e.g., statement reorder)
  * Edge placement if approach not in seed set

* **Method**

  * Interviews w/ 6 instructors (≥150 students classes) → need to see progress live (N1), challenges: diff granularity (C1), cannot validate at scale (C2), scaling tailored feedback hard (C3)
  * Built VizProg JupyterLab extn
  * Within-subjects study w/ 16 participants (TAs, tutors, senior students) using replay of authentic coding logs (keystroke-simulated)
  * Compared VizProg vs augmented OverCode baseline
  * Measures: accuracy in identifying misunderstandings, # found, time to start finding errors, usability feedback

* **Results**

  * Accuracy: VizProg ≈ 80% vs baseline ≈ 51% (p<.0001)
  * More misunderstandings found: VizProg μ=4.5 vs baseline μ=2.4 (p<.01)
  * Started finding errors earlier (500s vs 1070s, p<.05)
  * Participants liked grouped similar subs, grouped error types, less context-switching, could act while students still working

* **Takeaways**

  * 2D semantic+progress space = fast mental model for class state
  * Helps target feedback where most impactful
  * Extensible w/ better normalization + incremental map building for cold start scenarios


==> notes/related.tex <==
\section{Related Work}
\label{sec:related}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/mango.png}
    \caption{This is random and brings me joy as I work on this.}
    \label{fig:enter-label}
\end{figure}
% Mental Models
%% General

\citet{heinonen2023synthesizing}
- The review identifies \textbf{three primary kinds of mental models}:
\begin{enumerate}
    \item \textbf{Program mental models} (understanding code structure/functionality)
    \item \textbf{Concept mental models} (e.g., recursion, objects, variables)
    \item \textbf{Task/solution mental models} (how to complete a task or design a system)
\end{enumerate}
- Mental models vary in definition (cognitive structure vs. conceptual understanding), and in how they are stored (working memory vs. long-term schema).
- Models can be hierarchical, layered (syntax vs. semantics), subjective, abstract, and dynamic. Many studies highlight \textbf{novice-expert differences} in structure, abstraction, and generalization.
- Mental models are shaped by background knowledge, learning context, and programming experience. The process is often iterative, goal-driven, and influenced by both top-down expectations and bottom-up observations (e.g., reading code, debugging).
-  They detail:

\begin{itemize}
    \item \textbf{Hypothesis-driven comprehension:} Programmers form hypotheses about program behavior and search the code to confirm or disprove them.
    \item \textbf{Use of indicators/beacons:} Experienced programmers recognize familiar patterns using cues like function names or control structures.
    \item \textbf{Information needs and abstraction levels:} Programmers need both syntactic (e.g., control flow) and semantic (e.g., architectural role) information, and shift between them depending on the task and experience.
    \item \textbf{Visual or spatial dimensions:} Mental models often include spatial information, such as the location of relevant code segments—though it remains unclear whether this is stored in the model or externalized.
\end{itemize}
- The most common target systems were systems or programs including various aspects of a program or a system, such as its source code or the underlying machine
- Mental models were described as helping perform tasks such as decision-making, making predictions, and programming tasks such as debugging and and program modification
- "Programmers can develop an understanding of a program from its source code that encompasses not only an understanding of the meaning of the code statements, but also a more abstract understanding of the functional entities formed by the code statements, and how these entities work together to form the functionality of the program" -- \cite{brooks1978using}
- "The mental model is often understood as a working-memory construct that aids in working with the program code" -- \cite{canas2001role}
- "This layered mental model consists of representations of the code at different levels of abstraction—understanding of the code syntax and understanding of the semantic meaning of the code syntax are stored as separate yet interconnected layers of a mental model" -- \cite{detienne2002understanding}
- "ccording to schema-based theories, the resulting mental model consists of some connected collection of activated schemata" -- \cite{balijepally2012effect, detienne1990program, romero2001focal}
- why do we care? "understanding of mental models and their development is derived from the theory of model-centered learning and understanding of learning as the process of constructing mental models" -- \cite{seel2006mental}
- in CER, mental model theories used to see students's understanding of how a piece of code implementing the concept behaves or what happens at runtime when code implementing the concept is run
- At the higher level, information needs include program structure and function \cite{levy2019understanding, yates2020characterizing}
- This includes the composition and interaction of functional elements that comprise the program\cite{yates2020characterizing,  levy2019understanding, sillito2008asking}, their role and function  \cite{von1996identification, anneliese1998program, levy2003jeliot}, the relationships between them, and their interactions at run-time \cite{levy2019understanding, sillito2008asking, yates2020characterizing, fleming2008refining}.
- implementation level, information needs include the implementation of functionalities \cite{yates2020characterizing, sillito2008asking, anneliese1998program, levy2019understanding}[11,78,105,143], i.e., a comprehensive understanding of how a feature or functionality is implemented \cite{yates2020characterizing} and behaves during execution \cite{sillito2008asking, letovsky1987cognitive, levy2019understanding, fleming2008refining}.
- programmers have been shown to seek both implementation-level and abstract functional and structural information \cite{von1993code, von1994comprehension, bratthall2001program, von1996identification,levy2019understanding,von1997program}

- Knowledge at the implementation level appears to be acquired only as needed and is not always required \cite{yates2020characterizing, levy2019understanding}.


% CS2 Specific
\citet{simon2010making}
Notes:
- Despite calls for application focused tasks (how to use data structures), many questions still focus on implementation. This misalignment might contribute to the cognitive overload students face when bridging between memory-level understanding and higher-level abstractions.
- Simon et al. observe that:
\begin{itemize}
    \item \textbf{Few exams assess application-level knowledge}, despite curriculum recommendations to do so.
    \item \textbf{Tracing and writing code dominate}, especially for hashtables and stacks.
    \item There is \textbf{no clear trend toward abstraction-oriented assessments} over time.
\end{itemize}


\citet{zingaro2018identifying}
- \textbf{only 67\%} of students correctly implemented adding to the tail of a linked list, and \textbf{only 44\%} could correctly generate a balanced BST insertion order.
- students often \textbf{over-rely on memorized steps} (e.g., looping to find a list tail even when a tail pointer exists), suggesting a disconnect between \textbf{low-level memory operations and high-level structural goals}.
- optional: Without explicit scaffolding across these layers, learners may struggle to integrate control flow and structural changes—a challenge borne out in observed misconceptions and inefficiencies in common data structure tasks \cite{zingaro2018identifying}. or CS2 students often need to reason across both layers: tracing concrete memory changes and understanding their effects on recursive structures \cite{zingaro2018identifying}. Prior work shows that even advanced CS2 learners frequently struggle to maintain correct invariants in linked lists and construct balanced trees, revealing gaps in abstraction and schema generalization.

\citet{feijoo2021effects}
-  students find binary trees difficult due to their hierarchical and recursive structure, especially when visualizing insertions and traversals.
- \textbf{scaffolding}—in the form of block-based interaction—can \textbf{support integration of structure and algorithmic behavior}. Students in the visual tool group performed better at reasoning about how operations affected the tree.
- The block-based interface reduces \textbf{extraneous load} from syntax.
- It helps students develop \textbf{schema for tree construction} through visual means.
- discusses eventual transfer to code (i.e., \textbf{fading the concrete visual representation}), which mirrors the idea of \textbf{concreteness fading}.

\citet{mtaho2024difficulties}
- describe how students are unable to "predict what will happen when the code executes," linking this to difficulties with recursive logic and control flow 
- \textbf{importance and limits} of visualization tools, noting that traditional tools often emphasize “static or software visualization,” but may \textbf{overwhelm novices} or fail to support abstraction unless carefully designed: "Even following them in visualization tools is not easy for novices due to the runtime behavior of the program under execution. Programming constructs such as recursion, loops, functions, dynamic memory allocation, and pointer manipulation, are examples of code dynamics that have been reported to be difficult for novices to grasp."
- explicitly recommend \textbf{memory-based and multi-format visualizations} (text, diagram, animation) to reduce intrinsic and extraneous load -- "They further showed that presenting data structures material using three different approaches (text, memory diagram, and animation) in a congruent fashion did reduce both intrinsic cognitive load and extraneous cognitive load while increasing germane cognitive load, hence improving their interest and motivation to learn computer science courses."


- \citet{mtaho2023effectiveness} 
- synchronizes three forms: \textbf{textual, memory diagram, and animation}
- congruent visualizations \textbf{reduced extraneous and intrinsic load} while \textbf{increasing germane load}, improving mental models and comprehension
- Helps students \textbf{understand data structure behaviors} and \textbf{abstract transformations}, especially for \textbf{recursive and pointer-based content},
- "While detailed visualizations support step-by-step tracing, students often struggle to generalize from them. Congruent, layered visualizations may help learners abstract away from code mechanics \cite{mtaho2023effectiveness}."

\citet{almadhoun2021exploratory}
- CS2 students often \textbf{lack robust schemas} for reasoning about recursive or pointer-based structures.
- \textbf{students have difficulty mapping program control flow onto memory structure}, especially with loops or pointer assignments

\citet{layman2025topic}
- \textbf{students struggle more with implementation than conceptual understanding} across CS2 topics like recursion, linked lists, and BSTs — exactly the kind of abstraction-heavy content your MER visualizations target.
- They attribute this to:
\begin{itemize}
    \item Complexity of managing references and control flow
    \item Difficulty visualizing behavior
    \item Lack of concrete metaphors or prior mental models
\end{itemize}
- These are \textit{classic signs} of \textbf{extraneous and intrinsic cognitive load}, which justify introducing scaffolds like MERs \textit{before} students hit implementation walls.

\citet{franch2021goal}
- Prior work has shown that goal-oriented visual modeling of data structures—e.g., using iStarDust—can significantly improve students’ ability to describe and differentiate data structures by making their functional goals and quality requirements explicit \textbackslash{}cite\{franch2021goal\}.

\citet{bansal2021eye}
- \textbf{emphasizes detailed, code-level traces}, and students defaulted to reading the code over engaging with visual summaries.
- Authors note that familiarity bias and information overload may limit novice uptake of advanced visualization features.
- \textbf{Debugging study} showed Eye users had reduced debugging time and frustration, though results were only marginally significant.
- \textbf{Code comprehension study} showed no significant difference in quiz scores, but students reported improved clarity and interest.


Multiple Representations

% ===============================
% Notes on DeFT Framework (Ainsworth, 2006)
% Source: Ainsworth, S. (2006). DeFT: A conceptual framework for considering learning with multiple representations. Learning and Instruction.
% ===============================
- DeFT = Design, Functions, Tasks
- Framework to analyze why and when multiple external representations (MERs) support learning
- Key insight: MERs can help learning, but not automatically — success depends on how they're designed, what purpose they serve, and how learners interact with them
- Avoids oversimplified "modality-based" reasoning (e.g., visual + text is always good); instead focuses on deeper cognitive demands


\textbf{Design Parameters (how MERs are structured):}
\begin{itemize}
  \item \textbf{Number of representations:} More reps = more potential benefit, but also more integration demand. Use the \emph{minimum necessary} reps to meet learning goals. Excess reps can split attention.
  
  \item \textbf{Information distribution:}
  \begin{itemize}
    \item Reps can have distributed (different info), redundant (same info), or partial overlap.
    \item \textbf{Why this matters:} Redundancy can reinforce understanding \emph{if learners struggle with one format}, but may create cognitive overload if not needed.
    \item Example: novice CS2 students may benefit from both code and memory diagrams showing same process (redundant), whereas advanced students may only need one.
  \end{itemize}
  
  \item \textbf{Form of representation:}
  \begin{itemize}
    \item Includes: diagrams, text, code, graphs, tables, animations, narration, etc.
    \item Each format has different computational affordances (Larkin \& Simon, 1987).
    \item Representational chemistry: different forms can interact \emph{positively} (complementary insight) or \emph{negatively} (interference/conflict).
    \item \textbf{Why:} Form affects how information is processed (visually, spatially, symbolically). Learners must decode the format and link it to the domain.
  \end{itemize}

  \item \textbf{Sequence:}
  \begin{itemize}
    \item Order matters. Learners may benefit more from concrete $\rightarrow$ abstract or qualitative $\rightarrow$ quantitative sequences.
    \item \textbf{Why:} Sequences can support scaffolding (e.g., concreteness fading) and avoid premature abstraction.
    \item For CS2: start with a block-based or visual stack diagram, fade toward raw code+memory trace.
  \end{itemize}

  \item \textbf{Translation support:}
  \begin{itemize}
    \item Learners often struggle to relate representations even if they understand them individually.
    \item Help needed to show \textbf{how} parts of one rep relate to another: dyna-links, color coding, hover/mouse-over effects, matched layout, drag-and-drop.
    \item \textbf{Why:} Translating between reps is one of the hardest tasks (requires mapping structures and semantics across formats).
  \end{itemize}
\end{itemize}

% --------------------------------------
% Pedagogical Functions (Why MERs are used)
% --------------------------------------
\textbf{Pedagogical Functions of MERs (Why MERs help learning):}
\begin{enumerate}
  \item \textbf{Complementary roles}
  \begin{itemize}
    \item Different reps support different \emph{cognitive processes} (e.g., perceptual vs. symbolic).
    \item Different reps may contain different \emph{information} (e.g., spatial vs. functional).
    \item \textbf{Why:} Learners can exploit the strengths of each rep for different sub-tasks.
    \item In programming: a visual tree shows structure; code shows syntax and logic flow.
  \end{itemize}

  \item \textbf{Constraining interpretation}
  \begin{itemize}
    \item Familiar or concrete reps help learners interpret more abstract/ambiguous ones.
    \item \textbf{Why:} Learners often misinterpret abstract forms (e.g., text), but concrete or spatial reps limit misreadings.
    \item Example: a linked list animation constrains how learners interpret the pointer manipulations in C++.
  \end{itemize}

  \item \textbf{Constructing deeper understanding}
  \begin{itemize}
    \item Reps used together to support abstraction, generalization, and relational thinking.
    \item Subfunctions:
    \begin{itemize}
        \item \textbf{Abstraction:} Extracting core structure from different formats.
        \item \textbf{Extension:} Transferring knowledge across rep types or domains.
        \item \textbf{Relation:} Understanding how different views align or cohere.
    \end{itemize}
    \item \textbf{Why:} Constructivist view — learning = integrating and organizing across perspectives. MERs make this possible but cognitively demanding.
    \item In CS2: code + memory diagram + pointer map = deeper understanding of dynamic data structure behavior.
  \end{itemize}
\end{enumerate}

% --------------------------------------
% Cognitive Tasks (What learners must do)
% --------------------------------------
\textbf{Cognitive Tasks learners face when using MERs:}
\begin{itemize}
  \item \textbf{Understand the form:} How to read/operate on each representation (e.g., graph axes, syntax, visual symbols).
  \item \textbf{Map to domain:} What each part of the rep means in the target domain (e.g., what a downward arrow means in a recursion stack).
  \item \textbf{Select appropriate reps:} Strategic use — choosing the best tool for a task.
  \item \textbf{Construct own reps:} Generating diagrams or traces can deepen understanding.
  \item \textbf{Relate reps:} Most challenging — mapping elements across reps; e.g., variable in code $\leftrightarrow$ memory box in diagram.
\end{itemize}

% --------------------------------------
% Why MERs often fail
% --------------------------------------
\textbf{Why MERs sometimes fail:}
\begin{itemize}
  \item Learners often treat reps in isolation (no integration)
  \item May rely on superficial cues (e.g., visual resemblance over structure)
  \item Lack of support for translation → confusion/frustration
  \item MERs can overwhelm low-prior-knowledge learners (too much load)
\end{itemize}

% --------------------------------------
% Design Implications (from DeFT)
% --------------------------------------
\textbf{Design heuristics from DeFT:}
\begin{itemize}
  \item Match design to function: \textit{Complementing? Constraining? Constructing?}
  \item Co-present reps \textbf{only if} learners need to relate them; otherwise, risk split-attention
  \item Scaffold translation: alignment, cues, dynamic links (but avoid over-automation)
  \item Sequence reps from familiar/simple to unfamiliar/abstract
  \item Adjust complexity/support to learner expertise
  \item Aim to reduce extraneous load and increase germane processing (links to CLT)
\end{itemize}




% ===============================
% Notes on Educational Value of Multiple Representations (Ainsworth, 2008)
% Source: Ainsworth, S. (2008). The Educational Value of Multiple-representations when Learning Complex Scientific Concepts. In J.K. Gilbert et al. (Eds.), Visualization: Theory and Practice in Science Education.
% ===============================
- Multiple representations (MRs) can support deep science learning, but only when thoughtfully designed and used
- MR environments reviewed: SMV-Chem, Connected Chemistry, DEMIST, SimQuest, PAKMA
- Functions of MRs (DeFT-inspired taxonomy):
  - Complementary roles: Different reps show different info or support different processes (e.g., tables for values, graphs for trends, equations for relationships)
  - Constraining interpretation: Simple/familiar reps (like animations) can help learners interpret more abstract ones (like graphs)
  - Constructing deeper understanding: Helps learners form abstractions, relate and extend knowledge across reps

- Challenges with MRs:
  - Understanding the form (syntax/structure) of reps (e.g., axes, gradients, symbols)
  - Mapping reps to domain knowledge (e.g., what slope means in velocity-time graphs)
  - Selecting the right rep for the task
  - Constructing reps (e.g., drawing a graph from data or equations)
  - Relating reps: often the hardest part; learners frequently fail to link info across multiple formats

- Pitfalls:
  - Just adding reps doesn’t ensure learning — can overwhelm or confuse learners
  - Misuse of reps or over-reliance on surface features (e.g., thinking a flat graph = no motion)
  - Combining reps poorly can hinder learning more than using fewer, well-targeted ones

- Heuristics for design:
  - Use minimal number of reps needed to achieve goal
  - Consider learners' prior knowledge — use constraining reps only if helpful
  - Sequence reps gradually; don’t show everything at once
  - Provide scaffolding to relate reps (e.g., matching colors, layout proximity, labels)
  - Align pedagogical goals with rep function (e.g., don’t expect abstraction if reps are too similar or disconnected)


% ===============================
% Notes on "Multiple Representations in Physics and Science Education – Why Should We Use Them?"
% Source: Opfermann, M., Schmeck, A., & Fischer, H.E. (2017). In D.F. Treagust et al. (Eds.), *Multiple Representations in Physics Education*, Models and Modeling in Science Education 10, Springer.
% ===============================
- contribution one: Presents a comprehensive overview of theories supporting the use of multiple external representations (MERs) to enhance learning in physics and science education.
- contribution two: Synthesizes CTML, ITPC, and DeFT models to argue how MERs support deep-level understanding through visual/verbal integration, cognitive processing, and learner choice.
- related work it builds on: Builds on Mayer’s Cognitive Theory of Multimedia Learning, Schnotz’s Integrated Model of Text and Picture Comprehension, and Ainsworth’s DeFT framework.
- limitations: The chapter is conceptual and theoretical—empirical data and classroom case studies are referenced but not deeply analyzed; limited practical guidance for implementation.
- method: Literature review and synthesis of cognitive psychology and instructional design theories as applied to physics education contexts.


% ===============================
% Notes on How Multiple External Representations Are Used and How They Can Be Made More Useful
% Source: Schwonke, R., Berthold, K., & Renkl, A. (2009). *Applied Cognitive Psychology, 23*, 1227–1243. https://doi.org/10.1002/acp.1526
% ===============================
- contribution one: Study 1 reveals that learners often fail to understand the intended cognitive functions (complementary, constraining, and construction) of multiple external representations (MERs), leading to suboptimal processing. Eye-tracking data showed that students mostly focused on text and paid insufficient attention to diagrams and equations. Verbal reports confirmed that learners rarely perceived the roles of representations.

- contribution two: Study 2 demonstrates that a brief instructional intervention—informing learners about the role of diagrams as "bridges" between textual problem descriptions and equations—significantly improved learning outcomes. This effect was partially mediated by increased visual attention to diagrams and moderated by learners’ prior knowledge. Notably, informed learners with low prior knowledge achieved better outcomes while showing more efficient attention allocation.

- related work it builds on: Builds on Ainsworth’s (2006) framework on the functions of MERs (DeFT model) and past studies identifying the challenges of representational translation and integration (e.g., Hannus & Hyönä, 1999; Cox & Brna, 1995; Stern et al., 2003). Also connects to research using eye-tracking to assess cognitive engagement (Rayner, 1998) and the importance of explicit guidance in multimedia learning environments (McKendree et al., 2002).

- limitations:  
  • Small sample sizes in both studies (N=16 in Study 1, N=30 in Study 2) limit statistical power and generalizability.  
  • Participants were psychology students, potentially with higher metacognitive and verbal skills, which may not reflect broader learner populations.  
  • The think-aloud and retrospective protocols may not capture all aspects of students’ reasoning.  
  • The intervention focused on only one type of representation (diagrams), not covering general representational competence.

- method:  
  • **Study 1 (Exploratory):** Used eye-tracking and stimulated recall to analyze how students allocated visual attention to three representation types (text, diagrams, equations) during worked examples in probability. Conceptual understanding was positively correlated with visual engagement with diagrams. Verbal data showed low awareness of MER functions.  
  • **Study 2 (Experimental):** Randomly assigned students to either receive functional information about diagrams or not. Eye-tracking data and learning outcomes (transfer and conceptual understanding) were analyzed via moderated mediation models. Instruction increased attention to diagrams and improved learning, particularly for students with low prior knowledge.  
  • Eye-tracking metrics included fixation duration, cumulative fixation, gaze duration, and transition frequency among representations. Learning was assessed through pretest/post-test tasks measuring procedural, conceptual, and transfer knowledge.


% ===============================
% Notes on *Multiple Representations and Multimedia Learning*
% Source: Ainsworth, S. (2025). In *International Handbook of the Learning Sciences*
% ===============================

- contribution one  
  - Synthesizes multiple research traditions (cognitive, sociocultural, and technological) into a comprehensive overview of multi-representational learning.
  - Proposes a framework that integrates cognitive, social, and affective dimensions of representational learning.

- contribution two  
  - Highlights how representations should be evaluated based on their function and context, not merely their form or quantity.
  - Emphasizes the importance of learner-generated and body-based representations in future learning environments.

- ideas that the paper talks about (key terms, definitions, relations)  
  - **Multi-representational learning**: Learning mediated by multiple forms of representations such as text, images, animations, graphs, haptics, and simulations.
  - **Cognitive load theory**: Learners benefit when representations are designed to minimize unnecessary working memory demands.
  - **Multimedia learning theory (Mayer)**: Learning improves when both verbal and visual channels are utilized appropriately.
  - **DeFT framework (Ainsworth)**: Advocates functional over taxonomic classification of representations—focus on how they support learning goals.
  - **Representational competence**: The ability to interpret, construct, and relate different representations.
  - **Embodied learning**: Learning enhanced through representations that involve the body (e.g., gesture, haptics, interactive installations).
  - **Meta-representational competence**: Learners' understanding of how and why to create/use representations in various learning contexts.

- related work it builds on  
  - Cognitive theories: Mayer (2014), Sweller et al. (1998), Schnotz (2005).
  - Sociocultural perspectives: Säljö (1999), Kozma et al. (2000), Latour (1999), Roth & Bowen (2001).
  - Technological developments: van der Meij & de Jong (2006), de Jong et al. (2013), Habgood & Ainsworth (2011).
  - Representational construction: diSessa (2004), Kozma & Russell (2005), Prain & Tytler (2012).

- limitations  
  - Most cognitive studies are lab-based and may not generalize to real-world educational settings.
  - There's a gap in understanding how teachers teach with representations or how to train them to do so effectively.
  - Representational learning is complex—students often fail to integrate multiple forms effectively without explicit support.
  - Assessment methods lag behind; they often do not reflect multi-representational learning.

- method  
  - Conceptual and integrative review of literature across cognitive psychology, sociology, and learning technology.
  - Examples range from controlled lab studies (e.g., animation + narration studies) to ethnographic observations (e.g., chemistry labs, navigation teams).
  - Proposes principles based on design-based research, emphasizing iterative cycles of implementation and refinement.

% ===============================
% Notes on Pedagogical Affordances of Multiple External Representations in Scientific Processes
% Source: Wu & Puntambekar, 2012 (DOI: 10.1007/s10956-011-9363-7)
% ===============================
- **Contributions**
  - Argues for the importance of using multiple external representations (MERs) to support students’ engagement in authentic scientific practices.
  - Proposes pairing MERs with scientific processes based on their pedagogical affordances.
  - Presents a taxonomy of representations across disciplines (verbal-textual, symbolic-mathematical, visual-graphical, actional-operational).
  - Discusses types of scaffolding needed to effectively support learning from MERs in classroom settings.

- **Key Ideas & Definitions**
  - *External Representations*: Visual, verbal, symbolic, and physical formats used to represent scientific phenomena and processes.
  - *Affordances*: Properties of representations that offer opportunities for learners to act in certain ways; learner-relative and context-dependent.
  - *Scientific Processes*: Asking questions, planning investigations, analyzing data, constructing explanations, evaluating information.
  - Effective learning occurs when the affordances of a representation align with the goals of the scientific process and student capabilities.

- **Representation Taxonomy (adapted from Lemke and Tsui)**
  - **Verbal-textual**: Written/oral text, metaphors. Supports asking questions, explaining, evaluating.
  - **Symbolic-mathematical**: Equations, chemical structures. Supports data analysis and explanation.
  - **Visual-graphical**: Graphs, diagrams, animations. Supports planning, analysis, and explanations.
  - **Actional-operational**: Hands-on activities, demonstrations. Supports real-world investigation and data collection.

- **Pedagogical Affordances**
  - Different types of representations afford different roles in scientific inquiry.
  - Table 1 in the paper maps each representation type to scientific processes and affordances (e.g., visual-graphical helps visualize relationships between variables).

- **Related Work**
  - Builds on dual coding theory (Paivio), cognitive flexibility theory (Spiro), and Ainsworth’s work on MERs.
  - Builds on Lemke (2004), Kozma & Russell (2005), and the National Research Council’s frameworks.
  - Connects to studies on analogies in science education and the learning sciences (e.g., Duit 1991, Roth & McGinn 1997).

- **Method**
  - Conceptual review and synthesis of literature across cognitive psychology, science education, and educational technology.
  - Framework development: Affordances of representations + science process pairing.
  - No empirical study presented; rather, theoretical synthesis and framework suggestion.

- **Types of Scaffolding Identified**
  - **Dynamic linking**: Representations are automatically updated across formats to reinforce connections.
  - **Model progression**: Sequencing representations from concrete to abstract.
  - **Sequencing**: Strategic order of presenting MERs affects learning.
  - **Support in instructional materials**: Prompts, self-explanation, integration cues.
  - **Teacher support**: Guided questioning, modeling translation between representations.
  - **Active engagement**: Learners must process, compare, and connect representations actively.

- **Limitations**
  - Taxonomy may not cover all representation types or fit all domains (e.g., submicro representations in chemistry).
  - Students may not naturally perceive or use affordances; requires scaffolding.
  - MERs can pose cognitive overload without careful design.
  - Representation affordances depend on learners’ prior knowledge and skills.

- **Future Research Directions**
  - Domain-specific representation-process pairings.
  - Better alignment between designed, perceived, and enacted affordances.
  - Integration of multiple scaffolding types and agents (teachers, tools, materials).


% ===============================
% Notes on *Multiple Representations in Computational Thinking Tasks: A Clinical Study of Second-Grade Students*
% Source: Moore et al., (2020). Journal of Science Education and Technology. https://doi.org/10.1007/s10956-020-09812-0
% ===============================

- **Contributions**
  - Investigates how second-grade students use and translate between multiple representations during computational thinking (CT) tasks.
  - Introduces a clinical study methodology using the Code and Go Robot Mouse to examine students’ strategies.
  - Expands the Lesh Translation Model to include embodied cognition (gestures) as a representational form.
  - Provides qualitative evidence of how young learners navigate CT challenges using multimodal strategies.

- **Key Ideas / Terms / Definitions**
  - *Computational Thinking (CT)*: Defined per Shute et al. (2017) as the conceptual foundation to solve problems algorithmically, with or without computers. Includes facets like decomposition, abstraction, algorithm creation, debugging, iteration, generalization.
  - *Representational Fluency*: The ability to translate among various representations—concrete, pictorial, symbolic, language, gestures.
  - *Lesh Translation Model*: A framework highlighting five core representation types and the translations among them. This study adds gestures.
  - *Embodied Cognition*: Use of gestures, pointing, movement as cognitive tools for processing and translation.
  - *Spatial Reasoning*: The ability to mentally manipulate objects and reason about space, crucial in translating CT representations.

- **Method**
  - Clinical task-based interview approach with three second-grade students.
  - Activities used the Code and Go™ Robot Mouse, involving translation among map, physical course, code cards, and mouse programming.
  - Four tasks:
    1. Game as designed – map to course to code to mouse.
    2. Create a course and draw the corresponding map.
    3. Follow a code card sequence to determine cheese location on course.
    4. Program mouse directly from a map (no physical course visible).
  - Video and audio data coded using a priori representations categories (concrete, pictorial, symbolic, language, gestures).

- **Findings (Detailed Themes)**
  - **Concrete Representations**:
    - Students often used physical tools (mouse, tiles, fingers, objects like bracelets) to aid thinking.
    - These were especially helpful when tasks increased in complexity.
  - **Language as Scaffold**:
    - Children used self-talk and speech to organize steps and reduce cognitive load.
    - Language served both communicative and cognitive functions.
  - **Embodied Movements**:
    - Gestures (e.g., pointing, tracing paths) helped students represent steps spatially and conceptually.
    - When not allowed to use tools directly, students substituted with physical movements or other objects.
  - **Representational Maturity**:
    - Students shifted from more concrete to more abstract representations as comfort with task increased.
    - However, in more complex tasks, students reverted to concrete tools for support.
  - **Spatial Orientation Challenges**:
    - Difficulty aligning their own spatial orientation with that of the robot or course.
    - Students who physically moved to match the mouse’s perspective performed better.
    - Perspective-taking and mental rotation were developmental hurdles.

- **Related Work**
  - Builds on Papert (1980), Bers (2010, 2018), Wing (2006) on CT.
  - Lesh and Doerr (2003) for representational fluency framework.
  - Adds to research on embodiment (Goldin-Meadow et al., 2001; Hostetter & Alibali, 2008).
  - Extends Fessakis et al. (2013), who found spatial orientation to be a barrier in CT environments for young children.

- **Limitations**
  - Small sample size (n = 3).
  - Students self-selected into the activity.
  - Conducted over two one-hour sessions.
  - Use of facilitators may have influenced behavior.
  - Robot mouse lacked features like loops, limiting generalizability to more advanced programming.

- **Implications**
  - CT development in young children is supported by concrete tools, language, and embodied strategies.
  - Curriculum should include opportunities for physical manipulation, explicit translation tasks, and scaffolding for spatial reasoning.
  - Educators should be aware of the cognitive load involved in representation translation and support students accordingly.
  - Intermediary representations (e.g., gestures, language) are key transitional strategies in CT fluency.

- **Future Research Directions**
  - Validate findings with larger populations.
  - Explore representational strategies across different CT environments (e.g., virtual, block-based coding).
  - Investigate how strategies evolve with age and practice.







==> notes/terminology.tex <==
\paragraph{Terminological note.}
Across computing education, researchers have used a range of terms to describe the kind of reasoning needed to coordinate execution behavior, reference manipulation, and abstract data structure goals. These include semantic reasoning \cite{levy2019understanding}, layered mental models \cite{heinonen2023synthesizing}, deep abstraction \cite{devathasan2022abstraction}, and task-specific schemas \cite{detienne1990program}. While these constructs overlap, none alone captures the practical, cross-layer reasoning difficulties students face in CS2—particularly around reference-based structures like linked lists and trees. In this paper, we use the term \textbf{structural abstraction} not as a theoretical contribution in itself, but as a terminological shorthand: a pragmatic way to refer to reasoning that links low-level code and pointer operations to high-level structural transformations and design goals. Our goal is not to redefine existing theory, but to name a recurring but inconsistently labeled problem space in CS2 learning.



==> tables/clarity.tex <==
\begin{table}[t]
\centering
\caption{Descriptive statistics and one-sample $t$-tests for overall scales (RQ1--RQ2).}
\label{tab:clarity}
\begin{adjustbox}{max width=\columnwidth,center}
\begin{tabular}{lcccccc}
\toprule
Scale & $n$ & $M$ & $SD$ & Midpoint & $t$ & $d$ \\
\midrule
Clarity/Helpfulness & 307 & 3.83 & 0.74 & 3 & 19.66*** & 1.12 \\
Cognitive Load$^{\dagger}$ & 307 & 3.03 & 0.72 & 3 & 0.73 & 0.04 \\
Ease of Use (SUS proxy) & 307 & 3.58 & 0.70 & 3 & 14.65*** & 0.84 \\
\bottomrule
\multicolumn{7}{l}{\footnotesize $^{\dagger}$Higher scores indicate \emph{lower} perceived mental effort after reverse-coding. ***$p<.001$.} \\
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/features.tex <==
\begin{table*}[t]
\centering
\caption{Commonly cited features across RQ1 (experience) and RQ2 (usability/load), grouped by thematic category.}
\label{tab:features_summary}
\begin{tabular}{lll}
\toprule
\textbf{Category} & \textbf{Feature} & \textbf{Helpful / Limiting Aspects} \\
\midrule
\multirow{2}{*}{\textbf{Navigation \& Interaction}} 
  & Step-by-step pacing & Clarifying and controllable; sometimes slow or tedious \\
  & Interactivity controls & Replay/reset valued; limited code editing or exploration \\
\midrule
\multirow{3}{*}{\textbf{Visual Representation}} 
  & Multiple views (MER) & Supports structural reasoning; can cause overload \\
  & Color and highlighting & Aids attention and alignment; insufficient without labels \\
  & Abstract structure view & Helps "see the big picture"; needs more flexibility \\
\midrule
\multirow{2}{*}{\textbf{Layout \& Presentation}} 
  & Tri-pane layout & Supports layered reasoning; cluttered on small screens \\
  & Visual styling & Clear visual hierarchy; occasional contrast/resizing issues \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/subgroups.tex <==
\begin{table}[t]
  \centering
  \caption{Subgroup comparisons for clarity, cognitive load, and usability (RQ3).}
  \label{tab:subgroups}
  \begin{adjustbox}{max width=\columnwidth,center}
    \begin{tabular}{@{} llccc @{}}
      \toprule
      Subgroup & Measure & Group Means (SD) & $t$/stat & $p$ \\
      \midrule

      \multirow{3}{*}{\textbf{Language (Native vs.\ Non-native)}}
        & Clarity        & 3.86 vs.\ 4.07 (0.75 / 0.71) & $t=-2.32$ & .022* \\
        & Cognitive Load & 3.16 vs.\ 3.06 (0.72 / 0.84) & $t=1.03$  & .305  \\
        & Ease of Use    & 3.62 vs.\ 3.75 (0.70 / 0.63) & $t=-1.67$ & .097  \\
      \midrule

      \multirow{3}{*}{\textbf{Prior Experience (Any vs.\ None)}}
        & Clarity        & 3.89 vs.\ 3.97 (0.72 / 0.79) & $t=-0.89$ & .377  \\
        & Cognitive Load & 3.19 vs.\ 3.01 (0.72 / 0.81) & $t=1.93$  & .055  \\
        & Ease of Use    & 3.64 vs.\ 3.68 (0.67 / 0.70) & $t=-0.44$ & .664  \\
      \midrule

      \multirow{3}{*}{\textbf{Gender (Men vs.\ Women)}}
        & Clarity        & 3.90 vs.\ 3.94 (0.71 / 0.77) & $F=0.08$  & .778  \\
        & Cognitive Load & 3.14 vs.\ 3.11 (0.72 / 0.81) & $F=0.02$  & .885  \\
        & Ease of Use    & 3.65 vs.\ 3.67 (0.66 / 0.72) & $F=0.05$  & .826  \\
      \bottomrule
    \end{tabular}
  \end{adjustbox}
  \vspace{2pt}
  {\footnotesize *$p<.05$. Values reflect Welch’s $t$ or one-way ANOVA/Kruskal–Wallis as applicable.}
\end{table}

==> wordgraves-old-dont-read/CHI/01intro.tex <==
\section{Introduction}
\label{sec:intro}
Programming requires thinking like a detective, zooming in to trace through code line-by-line while simultaneously stepping back to see the bigger picture of how it all fits together. So, learning programming requires reasoning across multiple layers of understanding, from simulating execution, predicting behavior, and explaining outcomes \cite{hayatpur2023crosscode, johnson1983mental, seel2006mental}. While expert developers are able to shift flexibly between abstraction levels \cite{yates2020characterizing, sillito2008asking, von1993code}, or sketch visual metaphors to support this shift \cite{ma2020domain}, novices often struggle with thinking about this shift \cite{levy2019understanding} or sketching it \cite{sajaniemi2008study}. Visualization tools can also help experts move between abstraction levels \cite{hayatpur2023crosscode}. Widely used tools like Python Tutor have been promising \cite{guo_online_2013}, but students still report being confused by visual encodings such as arrows and call stacks early on \cite{karnalim2017effectiveness, karnalim2017use}. Moreover, while existing educational tools such as Python Tutor and debuggers allow students to see \textit{how} a program behaves in memory, they do not let them see \textit{why} the program behaves that way or \textit{what} the purpose of the program is \cite{pollock2020essence, sorva2013review}. This may encourage them to oscillate between surface-level tracing and high-level conceptualization~\cite{crichton2021role, brooks1983towards}, with gaps in their mental models impeding debugging and generalization.

Research in the learning sciences shows that the ability to move between abstract to concrete visual representations can aid understanding, reduce cognitive load, and promote integration across mental models~\cite{ainsworth2006deft, card1999readings, mnguni2014theoretical}. In programming, this may mean allowing students to focus on meaningful control-flow milestones, follow key data transformations, and reveal underlying details as needed. \textbf{Multiple External Representations} (MERs)~\cite{ainsworth2006deft} provide a theoretical \new{framework} for designing \new{coordinated views for learning}: by combining complementary representational forms, MER-based tools can scaffold progression from concrete behaviors to abstract concepts. MER's DeFT framework emphasizes cognitive design principles, complementarity, constraint, and construction, shown effective across mathematics, physics, and chemistry \cite{tripathi2008developing, treagust2017multiple, permatasari2022chemistry}.

\new{However, MER frameworks focus on how representations support learning \textit{given engagement}, implicitly assuming learners will use well-designed visualizations. This assumption may hold where uptake is self-directed, but in formal educational contexts where identity positioning and disciplinary norms matter, it can break down. Students often ignore well-designed visualizations \cite{schwonke2009multiple}, and our preliminary observations suggest they sometimes actively resist pedagogically sound representations, patterns pointing to systematic factors beyond cognitive design. Recent work by \mbox{\citet{wong2025spectrum}} has shown that tool engagement in workplace contexts reflects psychological needs like autonomy and competence, and while \mbox{\citet{hayatpur2023crosscode}} demonstrated multi-level visualization benefits for experienced programmers, how such uptake dimensions operate in formal educational settings, where disciplinary identity formation and scaffolding interact, remains uncharacterized.}

\new{We address this gap by characterizing uptake dimensions, the affective, social, and experiential factors that determine whether learners actually use visualizations, asking:}

\begin{description}[leftmargin=0.2cm, labelsep=0.2cm]
\item[\textbf{RQ:}] What factors determine whether learners engage with or resist multiple representations when learning programming, and how should these inform visualization design?
\begin{adjustwidth}{1em}{}
\begin{description}[leftmargin=0.6cm, labelsep=0.2cm]
    \item[\textbf{a:}] \new{What gaze patterns characterize students' work with synchronized code, memory, and metaphor views, and how do these align with or diverge from MER's cognitive principles?}
    \item[\textbf{b:}] \new{What affective responses characterize visualization use, and how do these shape engagement?}
    \item[\textbf{c:}] \new{What social and experiential factors influence whether students embrace or resist visualization scaffolds?}
\end{description}
\end{adjustwidth}
\end{description}

\comment{
Earlier:
\begin{description}[leftmargin=0.2cm, labelsep=0.2cm]
\item[\textbf{RQ:}] How do students engage with multi-representational and line-by-line program visualizations, and what shapes their sensemaking?
\begin{adjustwidth}{1em}{}
\begin{description}[leftmargin=0.6cm, labelsep=0.2cm]
    \item[\textbf{a:}] What meanings, uses, and affective responses do students describe when working with different views (code, memory, metaphor)?
    \item[\textbf{b:}] In what ways do students adapt to, resist, or reinterpret the representational logic of these tools?
    \item[\textbf{c:}] How do students’ prior experiences, identities, and classroom contexts influence their engagement?
\end{description}
\end{adjustwidth}
\end{description}
}

To investigate these questions, we designed and conducted our study in two stages. 
In the \textbf{first stage}, we developed a custom multi-representational design probe, refined through formative feedback from visualization researchers, instructors, and teaching assistants, that highlights relationships between code, execution state, and conceptual structure. 

In the \textbf{second stage}, we conducted within-subject study sessions with nineteen undergraduates who had recently completed the introductory programming and data structures sequence (CS1 and CS2) at a large North American research-intensive university. Each session combined task-based problem solving, think-aloud protocols, reflective interviews, and webcam-based gaze tracking as students engaged with both our probe and the widely used Python Tutor (following the comparison approach used by \citet{hayatpur2023crosscode}). We treat these sessions as situated accounts of sensemaking, shaped by disciplinary identities and prior experiences. 

With respect to paradigm, we take an interpretive stance in this study: our goal is not to identify the ``best'' tool, but to understand how students make sense of visualizations in relation to the problem, context, and their background. We foreground students’ interpretations extending prior work which shows that people may interpret analogies and reason about them differently depending on their experiences \cite{christie2020development}.

While most participants appreciated visualizations, gaze analysis showed that they mainly focused on code when problem solving. Many described using visualizations as verification rather than as primary tools for reasoning about code. We also noticed that students with prior programming experience tended to utilize memory visualizations, whereas novices fixated more on code. Participant accounts further explained these patterns. Some sought visualizations that preserved active effort (made them reflect) and technical fidelity, rejecting metaphors as ``far away from computer science,'' while others appreciated analogies that resembled the kinds of diagrams they typically drew when tracing programs. These responses indicate that students do more than follow what the visualization shows---they adapt, resist, or reinterpret representations in ways that reflect their prior experiences and contexts.

Together, our design probe and observations ground the contributions of our work, which we summarize as follows:
\begin{enumerate}
    \item[1.] \textbf{A Design Probe}: a multi-representational visualization tool, refined through formative feedback with instructors and TAs, that links code, memory, and metaphor views. Unlike prior tools such as CrossCode \cite{hayatpur2023crosscode} (designed for expert developers), ours was created as an educational probe to explore how novices interpret and move across different representations.
    \item[2.] \textbf{Empirical Insights from a Multi-Modal Study}: Through gaze tracking, think-aloud protocols, and reflective interviews with 19 students, we show that engagement with multi-view visualizations diverges systematically from MER theory's predictions, with students anchoring heavily in code despite available scaffolds \new{and reacting with wide variation to identical designs.}
    \item[3.] \new{\textbf{Theoretical Extension}: We identify three dimensions (agency preservation, representational calibration, legitimacy positioning) that characterized variation in how our participants engaged with well-designed visualizations. These dimensions suggest that MER theory for educational contexts may need to account for affective and social factors alongside cognitive design principles, a proposal that warrants empirical validation across diverse settings.}
\end{enumerate}

\subsection{Terminology} 
To clarify our usage: we use \emph{experts} to refer to professional or advanced programmers described in prior literature. Our study participants are referred to as \emph{students}. Within this group, we distinguish students with \emph{more prior programming experience} (e.g., from coursework or personal practice) and those with \emph{less prior experience}. For readability, we occasionally use \emph{novices} to describe students in the latter group, recognizing that the term \emph{novice} is relative and does not imply a complete lack of experience.


==> wordgraves-old-dont-read/CHI/02related.tex <==
\section{Related Work}
\label{sec:related}

We draw on work from the learning sciences (multiple external representations, cognitive load, mental models), computing education (notional machines, novice–expert differences), and HCI/VIS (interactive program visualizations as perceptual instruments). Together, these strands guide our study by providing theoretical foundations for how multiple views can support learning, highlighting challenges that novices face when forming program models, and offering design principles for building and evaluating interactive visualizations.

\subsection{Theoretical Grounding: MERs, and Cognitive Load}
% General Benefits
Visual representations are powerful cognitive supports: they can offload effort and memory demands \cite{scaife1996external}, support pattern recognition \cite{munzner2014visualization, ware2012information, card1999readings}, and promote deeper conceptual understanding \cite{heer2012interactive, mnguni2014theoretical}. In Mnguni’s \textit{cognitive process of visualization}, learners internalize visuals, connect them to prior knowledge, and externalize mental models via sketches, highlighting the active engagement and concept formation that visualization can foster \cite{mnguni2014theoretical}. 

% MER and DeFT
While a single view can aid learning, research in mathematics, physics, and chemistry shows that \textit{multiple coordinated views} yield greater benefits, supporting understanding of abstract concepts such as functions, forces, and molecular structures \cite{tripathi2008developing, treagust2017multiple, permatasari2022chemistry}. \textbf{Multiple External Representations (MER)} theory formalizes these findings, explaining how learners coordinate complementary but distinct sources of information \cite{ainsworth_functions_1999, ainsworth2006deft}. Ainsworth’s DeFT framework (Design, Functions, Tasks) further clarifies why and how multiple views support learning: different representations can complement one another, constrain misinterpretations, and promote constructive learning through translation across formats. These benefits, however, are not automatic. The design dimension of the framework stresses reducing redundancy, guiding attention, and preventing overload from excessive or misaligned views \cite{mayer2008increased, levy2003jeliot, wu2012affordances}, while the tasks dimension underscores the demanding but essential work of interpreting, relating, and integrating views into coherent mental models. Because of this dual focus on design and learner activity, DeFT has become a central lens for evaluating MER-based tools, including those developed for programming \cite{suh2022codetoon, suh2020coding}.

% CLT
\textbf{Cognitive Load Theory} (CLT) complements DeFT by distinguishing three kinds of mental effort: \textit{intrinsic load} (the complexity of the material itself), \textit{extraneous load} (unnecessary effort caused by poor design), and \textit{germane load }(productive effort that supports learning) \cite{paas2014cognitive, sweller2011cognitive}. CLT emphasizes minimizing extraneous demands, calibrating intrinsic difficulty, and encouraging germane effort. Learner characteristics, especially level of expertise, strongly influence these effects. For example, supports that help novices can actually hinder experts, a phenomenon known as the expertise reversal effect \cite{kalyuga2007expertise}. In practice, visualizations influence cognitive load not only through the information they display, but also the perceptual actions they may invite which guide what learners attend to, how they interpret it, and externalize their understanding \cite{adolph2015gibson, mnguni2014theoretical}.

Taken together, MER theory, DeFT, and CLT point toward a common design principle: effective programming visualizations must balance richness with efficiency. This means providing enough complementary views to foster abstraction, but not so many that they overwhelm; reducing redundancy and guiding attention with clear cues; sequencing from concrete to abstract; and tailoring support to a learner’s level of expertise~\cite{baldonado2000guidelines, fyfe2014concreteness, hassan2024evaluating}.

\textbf{Takeaway}: For our study, these frameworks highlight the promise of multiple views for supporting abstraction, while also warning that poorly coordinated or overly detailed representations can overwhelm novices rather than help them.

\subsection{Mental Models in Programming}
Programmers require layered mental models that link low-level execution (e.g., memory updates) with broader functional and structural goals \cite{johnson1983mental, brooks1978using, canas2001role, seel2017model}. Such models include program models (runtime behavior), concept models (abstract ideas such as recursion), and task/solution models (strategies for goals) \cite{heinonen2023synthesizing}. Schema-based perspectives frame them as structured templates that help learners interpret and anticipate behavior \cite{detienne1990program, balijepally2012effect, romero2001focal}. Novices often fall back on surface cues or tracing \cite{levy2019understanding}, whereas experts integrate local and global reasoning \cite{von1993code, sillito2008asking, yates2020characterizing}.  

In CS1 (introduction to programming at a university level) \cite{hertz2010cs1}, mental models are scaffolded by \emph{notional machines}, idealized representations of language behavior that support reasoning about scope, flow, and function calls \cite{juha2013notional, fincher2020notional}. Although partial and idiosyncratic \cite{greca2000mental, eckerdal2005novice}, they provide a foundation for deeper understanding. Without such scaffolds, detailed traces (e.g., Python Tutor~\cite{guo2013online}) risk focusing attention on low-level mechanics rather than conceptual ideas \cite{karnalim2017effectiveness, pollock2020essence, eckert2022loops}.  

In CS2 (second course in the introductory programming sequence) \cite{porter2018developing}, recursion, references, and hierarchical data structures require students to connect local operations to global structural intent \cite{layman2025topic, zingaro2018identifying, almadhoun2021exploratory}. Multiple external representations (MERs) can help by scaffolding representational competence (interpreting and constructing representations) and representational fluency (flexibly translating among them) \cite{ainsworth2006deft, daniel2018representational, zaqoot2019representational, schwonke2009multiple}.

\textbf{Takeaway}: This work positions our study to examine how students actually use visualization tools: do they lean on them for tracing, or do they connect them to higher-level mental models such as recursion and data structures?

\subsection{Existing Programming Visualization Tools}
\label{existing-tools}
Research on interactive program visualizations spans computing education, software engineering, and HCI. In education, they make program execution more transparent for beginners; in HCI, they act as  configurable perceptual tools for understanding, debugging, and design. Early work pairing animations with explanations improved novices’ debugging success~\cite{brusilovsky1993program}, demonstrating the benefit of linking visuals with text. More recent systems embed runtime state directly into the code. Omnicode~\cite{kang2017omnicode} shows variable values inline,  Projection Boxes~\cite{lerner2020projection} extend this with customization views, and Hoffswell et al.~\cite{hoffswell2018augmenting} provide guidelines for such in situ visualizations, stressing clarity and minimal disruption. These tools improve debugging efficiency but offer little support for cross-representational reasoning or abstraction.

Some approaches focus on redesigning code visuals or scaling visualization to broader contexts. Richer syntax and structure cues can make features easier to spot without adding overload~\cite{asenov2016richer}. Ko and Myers’ Whyline~\cite{ko2009whyline} reframes debugging as asking questions, leading to large efficiency gains. At the classroom level, VizProg~\cite{zhang2023vizprog} organizes student submissions in a semantic–progress space, helping instructors quickly identify misunderstandings. From a design angle, Ma’ayan et al.~\cite{ma2020domain} study how experts sketch and adapt diagrams, proposing a ``natural diagramming'' framework that aligns with calls in computing education to make notional machines more explicit ~\cite{sorva2013review}.
 
Eye-tracking data also highlight why design choices matter. Beginners often focus too heavily on code and neglect diagrams unless directed to them~\cite{schwonke2009multiple, bednarik2012expertise}. Layout can further shape attention---less linear arrangements trigger vertical scanning and extra effort, while experienced learners follow execution-driven strategies~\cite{bansal2021eye, bednarik2012expertise}. This is important because eye gaze has been shown more broadly to reflect cognitive processing, workload, and comprehension~\cite{just1976eye, underwood2004inspecting, pfleging2016model, ahn2020towards}, reinforcing its value for studying engagement with programming visualizations.

\textbf{Takeaway}: These tools and findings show progress in making execution transparent, but they leave open how multiple coordinated views can be designed to explicitly support cross-representational reasoning. Our study takes up this gap by probing how learners interpret and negotiate synchronized code, memory, and metaphor views.

\subsection{Positioning and Contribution}
Across these strands, we see a consistent gap. While MER/DeFT and CLT emphasize coordination and load, and mental model research highlights the need to connect execution with conceptual structure, existing visualization tools largely emphasize tracing or debugging. Our study addresses this gap by introducing a synchronized multi-representational probe that makes each view’s role explicit, aligns attention cues, and sequences representations to support abstraction and representational integration across CS1–CS2 topics.


==> wordgraves-old-dont-read/CHI/03design.tex <==
\section{Formative Design and Feedback}
\label{sec:viz-tools}
This section describes how we designed and refined our multi-representational visualization probe, drawing on theory, prior tools, and iterative feedback from instructors and teaching assistants.

We designed a multi-representational visualization probe\footnote{All visualization materials are openly available at \url{https://anonymous.4open.science/r/Multiple-Views-IntroProgramming-28DD}.} that embodies insights from MER/DeFT \cite{ainsworth2006deft} and concreteness fading \cite{fyfe2014concreteness}. Our aim was to address limitations of existing program visualization tools, which often encourage tracing but provide little support for cross-representational reasoning. The tool has three linked panels: \emph{code}, \emph{memory}, and \emph{metaphor} to help students connect concrete execution steps to more abstract ideas. 

\newbigimage[1.5]{figures/design-cycles.pdf}{Iterative design cycles for the multi-representational probe. Each cycle involved different stakeholders (instructors, researcher, TAs) and contributed  feedback that guided refinements to conceptual fidelity, representation coordination, and usability, leading to the probe used in our study.}{design-feedback}

\paragraph{Initial Design.} Two researchers reviewed program visualization systems mentioned in Subsection~\ref{existing-tools} and in~\cite{sorva2013review} to identify gaps for our probe. We found that while many tools emphasize line-by-line fidelity\footnote{We use \emph{fidelity} as a shorthand for how closely a visualization preserves relationships and behaviors considered essential to program execution (e.g., stack frames for function calls, pointer diagrams for references). Fidelity here does not imply literal correspondence to how memory is implemented in hardware, but rather alignment with canonical representations in programming visualizations.} or in-situ augmentation, they often overload learners with visual clutter, advanced programming jargon, excessive colors or text, and outdated design styles, while offering little support for building abstractions across representations. To inform our design space, we also examined pedagogical analogies from prior work~\cite{sanford2014metaphors} and drew on recurring CS1/CS2 challenges \cite{aedo2016teaching, gupta2023improving, garcia202520, zingaro2013facilitating, almadhoun2021exploratory,cherenkova2014identifying} to guide initial sketches. %The primary researcher also drew on their eight years of teaching CS1 and four years of teaching CS2, which surfaced recurring patterns of misunderstanding and informed initial sketches of the probe. 

\paragraph{Formative Design Cycles.} 
As shown in Figure~\ref{fig:design-feedback}, the tool was refined across three cycles with input from instructors, a program visualization researcher, and teaching assistants (TAs). In each cycle, a researcher led a brief, step-by-step walkthrough of each view, first asking reviewers to interpret what the visual conveyed, then offering a short explanation of the design rationale, and finally prompting concrete suggestions on what to keep or change (e.g., ``What would confuse a CS1/CS2 student?'', ``What would you change here?'', ``Where would you slow down or add a step?'').

Cycle1 involved three instructors who reviewed early prototypes for conceptual fidelity, commenting on whether the visuals captured execution faithfully and noting common student misconceptions the representations could address.
Cycle2 added two additional instructors and a program visualization designer, who reviewed representative CS1/CS2 problems, provided feedback on usability and metaphor clarity, and again surfaced target misconceptions.
In Cycle~3, nine TAs solved sample problems individually and reflected on what would confuse or help students, highlighting issues of pacing and engagement.
Feedback across cycles informed refinements such as progressive disclosure, clearer metaphor labels, and stepwise tracing.

\newbigimage{figures/general-labels.png}{The multi-representational visualization tool, showing three synchronized panel, (1) Code View, (2) Memory Analogy View, and (3) Visual Analogy View, alongside interactive controls (5–8). Colored labels in the text correspond to numbered markers in the figure.}{tool-layout}

\subsection{Layout and Components.}
The interface (Figure~\ref{fig:tool-layout}) presents three synchronized panes:  \\

\circnum{1} \textbf{\Code} A Python code view which highlights the active line with a yellow fill and orange outline to guide attention and support traceability~\cite{paivio1991dual}. TAs found this clear but suggested more meaningful variable names (e.g., ``Bunny'' instead of ``Hat 1'').

%The design follows dual coding theory by reinforcing the textual representation with spatial and color-based signals, thereby aiming to minimize extraneous cognitive load~\cite{sweller2011cognitive}.

% General framing (what it is, across examples)
% Possible variations (depending on context)
% Highlighting + greying rationale (with citation)
% Pedagogical intent (why it matters for learning) 
\circnum{2} \textbf{\Memory} depicts variable bindings and object references in the program's current state, closely aligned with Python Tutor \cite{guo_online_2013} to preserve familiarity. Reviewers appreciated familiarity but suggested more stepwise tracing in linked list tasks and suggested alternative analogies (e.g., a line of people) to highlight sequential references. 

\circnum{3} \textbf{\Metaphor} uses analogy-based depictions of program state, drawing on metaphors used in prior work~\cite{sanford2014metaphors, hermans2018thinking}. Reactions were mixed: instructors and TAs found the visuals engaging but sometimes less efficient than direct diagrams. They recommended clearer highlighting of loop conditions and metaphors emphasizing ``sequential handoff'' for linked lists.

\paragraph{Interaction Model.}
Execution is synchronized across views and controlled through four buttons:
\begin{itemize}
    \item [\circnum{5}] \texttt{\textbf{Next Step}} advances execution incrementally, showing only the effects of the current operation. This progressive disclosure~\cite{springer2019progressive} prevents overload: in CS1 each step maps to a line of code, while in CS2 steps are chunked at the function level to match learners’ abstraction skills. All views update together to maintain representational coherence~\cite{ainsworth1999functions}.
    \item [\circnum{6}] \texttt{\textbf{Previous Step}} reverses execution by one step to let learners revisit earlier states, supporting self-repair strategies~\cite{chi1994eliciting}. This button was valued in prior systems~\cite{birch1995dynalab,boroni1996dancing,sorva2013review}.
    \item [\circnum{7}] \texttt{\textbf{Reset Step}} returns the program to its initial state for quick re-exploration.
    \item [\circnum{8}] \texttt{\textbf{Last Step}} executes the remainder of the program at once, helping learners confirm predictions or shift from local tracing to global outcomes~\cite{renkl2002worked}, while retaining synchronized views.
\end{itemize}

Hover and selection events are also linked across views (\emph{brushing and linking}~\cite{roberts2006towards}), e.g., selecting a variable in \textit{Code View} highlights its memory cell and the corresponding element in the \textit{Metaphor View}.  

\paragraph{Metaphor Rationale.}
The metaphor layer in our tool is intentionally pluralistic, combining multiple analogy types to address different conceptual challenges identified in formative observations. For scope management, we adopted the ``house'' metaphor (see Figure~\ref{fig:scope-visual}), each scope as a separate room, variables as windows, treating function boundaries as ``separate spaces.'' Function calls and returns are depicted as animated arrows between rooms, sometimes annotated with ``phone'' icons to suggest message passing, highlighting the limited visibility of local variables from outside their scope. We implemented progressive disclosure of function details, based on instructor feedback that it could mitigate extraneous load~\cite{paas2014cognitive}.

\newpicture{figures/scope.png}{\textit{Coordinated representations for a function call}. The Code view (left) highlights the current line being executed. The Memory Analogy (center left) shows local and global variable bindings, with arrows indicating reference relationships. The Visual Analogy (center right) uses a ``house'' metaphor to depict separate scopes, with a phone icon representing the function call and argument passing. The Explanation panel (right) clarifies the metaphor and reinforces the distinction between local and global scope.}{scope-visual}

For while loop iteration, we chose a theatrical ``magician’s table'' scene (see Figure~\ref{fig:while-loops}, in which list elements are revealed in sequence until the sought‐after object (the bunny) appears. This visualization is Galilean \cite{frigg2020models}, it distorts structural details to make the stopping condition more recognizable.  A more Aristotelian approach \cite{frigg2020models}, like step-highlighting in a memory index diagram, would preserve fidelity but reduce salience. In contrast, our linked list depiction (see Figure~\ref{fig:linked-list}) takes an Aristotelian form: nodes are shown as connected boxes with arrows reflecting pointer references, but with mild embellishment, a relay race metaphor, to make the sequential handoff between nodes more visually salient without distorting data structure semantics~\cite{frigg2020models}.

\newpicture{figures/while-loops.png}{\textit{Coordinated representations for a while loop search}. The Code view (left) highlights the conditional assignment searching = False that terminates the loop. The Memory view (center) shows the current values of variables, including the lst array with the target ``Bunny'' at index 2. The Visual view (right) uses a magician and props metaphor to depict the search process, where the desired item (bunny) has been found and the search stops.}{while-loops}

\newpicture{figures/linked-lists.png}{\textit{Coordinated representations for linked list node creation}. The Python Code view (left) highlights the \_\_init\_\_ constructor for the Node class, showing parameter binding for self and data. The Memory Visualization (center) displays the call stack and corresponding objects in memory, with highlighted cells indicating newly created values and references. The Linked List Visualization (right) depicts the updated list structure, showing the new node containing 20 linked after the existing 10 node, with the final link pointing to None.}{linked-list}

Formative feedback guided these choices. For scope, the ``house'' metaphor resonated with most TAs more than envelopes or locked cabinets. The house was better at showing both separation and communication channels between functions. For loops, we explored mechanical metaphors (e.g., conveyor belts, clock hands) and narrative metaphors (e.g., treasure hunts). Instructors and TAs found playful metaphors engaging but slower to parse, reinforcing our need to balance engagement with fidelity. Using the feedback, we chose the magician's table for its immediate appeal and loop-stopping condition clarity. For linked structures, we weighed highly abstract pointer‐and‐box diagrams against richer physical analogies such as trains or assembly lines, or a chain of people climbing a wall, balancing recognizability with risk of over‐literal interpretation. We leaned on sticking to the traditionally used abstract linked-list analogy as the other analogies did not seem plausible to the TAs or failed to demonstrate the reference structure adequately. An instructor recommended making the linked-list a vertical chain so it could connect to students' tree visualizations.

In making these selections, we also considered accessibility for a diverse student population, including English Language Learners, prioritizing metaphors that were more likely to be widely recognizable across linguistic and cultural backgrounds.

By mixing Aristotelian and Galilean strategies~\cite{fincher2020notional}, we sought to preserve execution fidelity when accuracy is paramount (e.g., linked list pointer movement) and to amplify critical patterns where learners often miss them (e.g., loop termination). This diversity supports concreteness fading~\cite{fyfe2014concreteness}, giving learners an initial, embodied hook before transitioning toward more schematic, domain‐accurate views. All metaphors were refined with three instructors and nine TAs to ensure conceptual alignment, avoid misleading mappings, and maintain accessibility across a wide range of learner backgrounds.

\paragraph{Technical Implementation.}
The interface is a static HTML/CSS/JavaScript application with SVG rendering for diagrams. Firebase supports anonymous login and logs fine-grained interaction events (type, details, timestamp) for later analysis. The layout scales responsively, preserving spatial relations to maintain gaze economy~\cite{schwonke2009multiple}. Our code is openly available in the repository linked at the beginning of this section.

\paragraph{Comparison Baseline: Python Tutor.}
Python Tutor~\cite{guo2013online} served as a contrast case: a widely used single-view, state-of-the-art tool that shows execution with precise, line-by-line fidelity. Its strength is accuracy and detail, but its limitation is the lack of abstraction layers, leaving learners to integrate patterns across steps on their own~\cite{pollock2020essence}. This contrast surfaces different design values, precision versus abstraction support, and lets us examine how multi-representational coordination shapes sensemaking.

==> wordgraves-old-dont-read/CHI/04method.tex <==
\section{Methods}
\label{sec:methods}
We conducted a talk-aloud study to examine how students engaged with a multi-representational probe (featuring \Code, \Memory, and \Metaphor) alongside the widely used Python Tutor visualizer. Following a \textit{within-subjects design}, all participants used both tools, allowing us to compare their experiences directly. We focused on documenting learners’ reasoning processes—where they paid attention, got stuck, and how they reacted across representations. Figure~\ref{fig:procedure} shows our process which is described further in the Subsection \ref{subsec:proc}.

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{figures/procedure.pdf}
  \caption{Within-subjects, counterbalanced study design. Participants (N=19) completed three topical blocks (Scope, While Loops, Linked Lists). Each block comprised three short tasks followed by a brief reflection. Tool order was counterbalanced across participants using ABA and BAB sequences: in each topic, participants used either \textit{Python Tutor} first then the \textit{multi-representational (MR)} tool, or the reverse, before moving to the next topic. Sessions were conducted via Zoom screen sharing.}
  \label{fig:procedure}
\end{figure*}

\subsection{Participants}
Nineteen students participated in the study, with recruitment spanning two campuses of a large North American research university. All participants had completed both CS1 (introduction to programming) and CS2 (introduction to data structures, algorithms, and object-oriented programming) prior to the study. Both courses were taught in Python (version 3.10) and required to major in computer science at the university. While CS1 covered programming basics such as variables, loops, lists, dictionaries, and basic sorting algorithms, CS2 covered object-oriented programming (OOP) basics (encapsulation, inheritance), introduction to recursion, and basic abstract data structures (e.g., linked lists, n-ary trees, and binary search trees). 

Thirteen (13) participants reported having prior programming experience (\textit{PE} = Y) before university (typically a Java course in grade 12 or basics of Python in grade 11), while six (6) reported no prior experience (\textit{PE} = N). The sample included six (6) women and thirteen (13) men. Ten (10) participants completed the \textit{ABA} sequence and nine (9) completed the \textit{BAB} sequence. A detailed breakdown by participant is provided in Appendix~\ref{sec:participant-details}.

\subsection{Procedure}
\label{subsec:proc}
Recruitment emails (Appendix~\ref{recruit-email}) were distributed to all students who completed CS2 and CS1 near the end of the CS2 term, with permission from course instructors. Participants scheduled sessions directly and received standard compensation in line with institutional norms for one hour of research participation. Each session was conducted online via Zoom screen sharing.  This study was approved by the university’s research ethics board (protocol number redacted).

At the beginning of each session, the researcher introduced the study, obtained informed consent, and briefly introduced the think-aloud protocol. Participants were encouraged to verbalize their reasoning, uncertainties, and interpretations while working. For CS1-level topics, execution was revealed \emph{line by line}; for the CS2-level topic, stepping operated at the \emph{function/method level} to align with the course's increasing abstraction.  

Each participant worked through three topical blocks in fixed order, chosen to represent progressively more advanced concepts in the CS1–CS2 sequence: \textbf{Scope} (CS1; tracing variable updates in loops) \cite{aedo2016teaching, gupta2023improving, garcia202520}, \textbf{While Loops} (late CS1; reasoning about iteration) \cite{morazan2020make, cherenkova2014identifying}, and \textbf{Linked Lists} (CS2; traversing recursive pointer structures) \cite{zingaro2018identifying, almadhoun2021exploratory}. These topics are well-documented areas of novice difficulty \cite{garcia202520,cherenkova2014identifying, zingaro2018identifying} and require learners to coordinate reasoning about program purpose and runtime state, making them especially relevant for examining representational integration. Within each topical block, participants used both visualization tools in counterbalanced order (\textbf{ABA} or \textbf{BAB} sequences), a design intended to balance exposure while keeping sessions manageable in length ($\approx$60 minutes total, with $\sim$20 minutes per topic including tasks and reflection). The web application where they solved these tasks with the interviewer is shown in Appendix~\ref{example-images}. 

The interviewer used a semi-structured guide (Appendix~\ref{sec:protocol}) to elicit think-alouds and reflections while avoiding overly directive prompts. Prompts targeted \emph{perceptual uptake} (e.g., ``What do you notice in this visual representation?'') and \emph{conceptual integration} (e.g., ``How is the change in variables or control flow depicted for you?''), aligning with our interest in representational sensemaking~\cite{ainsworth2006deft}. For each topic, task probes (Appendix~\ref{sec:tasks}) asked students to trace, explain, and extend code, balancing execution details with higher-level reasoning.

After completing a task with one tool, participants reflected on its clarity, limitations, and alignment with their reasoning strategies before switching to the other tool. Post-task interviews encouraged \emph{cross-tool comparisons} (e.g., ``Which tool provided clearer visual cues for you, and why?'') to surface interpretive and affective contrasts. Sessions concluded with an open-ended debrief on perceived usefulness and suggestions for improvement.  

All sessions were screen-recorded to capture verbalizations, on-screen interactions, and tool states. Audio was transcribed verbatim and anonymized, with field notes documenting notable interaction patterns. In addition to screen recordings, we collected gaze data to better understand how learners visually engaged with each tool.  

\subsection{Analytic Approach}
We used a mixed-method approach to analyze the study data. Qualitative data such as participants' think-alouds, and reflections served as the primary evidence base, analyzed through reflexive thematic analysis (described below). Gaze data were treated descriptively, providing broad markers of visual attention that complemented and triangulated with participants' accounts. This design allowed us to link what students said with how they visually engaged with representations.


\subsection{Gaze Analysis}
We use the WebGazer.js framework~\cite{papoutsaki2018eye} to enable webcam-based eye tracking during online sessions. WebGazer infers gaze position by mapping pupil and head movements to on-screen coordinates through regression-based models. We chose webcam-based eye tracking rather than lab-based infrared systems for two reasons. First, our study was conducted remotely, and WebGazer provided a lightweight and scalable way to capture gaze without requiring specialized hardware or in-person participation. Second, prior work shows that although webcam tracking is less precise than dedicated systems, it achieves sufficient accuracy (1--2 cm median error) for identifying broad areas of interest (AOIs) in web-based studies~\cite{papoutsaki2017searchgazer, papoutsaki2018eye}. This has been further validated by recent online replications of visual world experiments~\cite{slim2023moving}, which find that WebGazer performs reliably when the AOIs are large (e.g., interface regions) but is not well-suited for distinguishing fine-grained elements such as single words or characters. This level of fidelity was appropriate for our design, since our AOIs were the three large visualization panes (Memory, Code, Visual) rather than smaller interface features. 

We defined three AOIs corresponding to the visualization panes of the MR tool: \textbf{Memory}, \textbf{Code}, and \textbf{Visual}. Fixations were parsed into transitions (e.g., Code $\rightarrow$ Memory) and aggregated into bigrams and trigrams to capture gaze sequences. This allowed us to examine how participants navigated across representational layers over time. For example, repeated Code $\leftrightarrow$ Memory oscillations suggested close attention to execution semantics, while sequences incorporating the Visual pane highlighted representational integration.

To reduce noise, we applied smoothing filters to raw gaze coordinates, ignored fixations shorter than 100 ms \cite{mahanama2022eye,scurr2014methodological, manor2003defining}, and windowed samples into 200 ms bins \cite{niehorster2020characterizing} to account for jitter. Derived metrics (first fixation, transition frequencies, AOI sequences) were used descriptively in our Results to complement the qualitative analysis of sensemaking. In Appendix~\ref{app:minimal-gaze}, we include minimal, reproducible code for resampling, AOI assignment, dwell and transition computations, and the transition/timeline figures; extended analysis and plotting code are available on OSF\footnote{\url{https://osf.io/bdcj6/?view_only=0bfdcfa330a6462e92d81ddbdc358cfc}}.

\subsection{Qualitative Analysis}
Our qualitative analysis was guided by a reflexive thematic analysis framework~\cite{braun2021one} situated within an interpretivist epistemology. We understand meaning-making as a socially and contextually situated process, and we treat the accounts shared by participants not as objective ``facts'' about tool use but as co-constructed narratives emerging in dialogue with the researcher, mediated by the interview setting, and shaped by participants’ prior experiences and disciplinary identities. Within this approach, we do not assume that there is a single correct interpretation of participants' experiences. Instead, we acknowledge the partiality and perspectival nature of any analysis, and treat diversity and even contradiction within accounts as analytically valuable. We position thematic analysis here not as a method for discovering ``themes'' latent in the data, but as a process of constructing patterns of meaning that are responsive to our research questions and grounded in participants' situated accounts.

\paragraph{Analytic process.}  
Our analysis was inductive, with two authors independently engaging in repeated cycles of:
\begin{enumerate}
    \item \textbf{Immersion:} Reading and re-reading transcripts alongside screen recordings to attend to language, gesture, pauses, and interaction rhythms.
    \item \textbf{Open coding:} Generating descriptive and interpretive codes that captured both what participants said (\emph{semantic level}) and the assumptions, values, or epistemic stances underlying those accounts (\emph{latent level}).
    \item \textbf{Memoing and reflexive note-taking:} Writing analytic memos throughout to record emergent insights, tensions, and reflexive observations, e.g., moments when the researcher's own teaching experience resonated with or diverged from participant narratives.
    \item \textbf{Theme development:} Clustering codes into higher-level patterns of meaning that captured both the feature-specific affordances of each visualization (e.g., coordination, metaphor, layout) and the affective–epistemic orientations participants adopted (e.g., trust, legitimacy, frustration, playfulness).
    \item \textbf{Iterative refinement:} Revisiting transcripts to test the coherence of emerging themes, consider alternative readings, and attend to outliers or disconfirming cases.
\end{enumerate}

\paragraph{Theoretical engagement.}  
Theoretical frameworks such as Multiple External Representations~\cite{ainsworth2006deft}, Cognitive Load Theory~\cite{paas2014cognitive, sweller2011cognitive}, and the notional machine literature~\cite{sorva2013review} informed our \emph{later} interpretation and positioning of the findings, but did not guide coding. We entered the analysis with the aim of allowing patterns to emerge inductively, attentive to what existing theory might overlook, problematize, or fail to account for.

\paragraph{Reflexivity in practice.}  
To support reflexivity, we describe the research team’s composition. The lead analyst was a graduate student trained in qualitative methods, with prior research experience in visualization, computing education, and HCI. A second researcher, an undergraduate with exposure to MER-related work in CS1/CS2 and experience closer to students to the coding. The lead analyst identifies as a ciswoman, and visible minority with extensive CS1/CS2 TA experience. Having also contributed to the design of the MER visualizations, she recognized a tendency to seek out positive evidence of their value and engaged in repeated reflexive questioning to check this bias. The undergraduate researcher, also a ciswoman and visible minority, had some prior CS1/CS2 TA experience and was closer in age to participants. Her proximity to the student experience added a complementary perspective in data review, helping the team attend to interpretations that might otherwise be overlooked.

The team held collaborative reflection sessions with a broader research group, including faculty with expertise in introductory computing instruction and visualization design, which functioned as a form of investigator triangulation. We also engaged in reflexive discussions throughout, questioning how our familiarity with program visualization tools and our own learning trajectories in CS1/CS2 might shape what we noticed and prioritized. We asked: How might our design commitments bias our reading of student accounts? Which perspectives or struggles might be underrepresented in this dataset? While such reflections cannot eliminate subjectivity, they helped us approach interpretation as a situated, dialogic process.

% \paragraph{Interpretive stance on claims.}  
% We make no claim to neutrality or exhaustiveness. Our goal is to offer one plausible, theoretically informed account of how students experienced these visualizations, recognizing that other researchers, coming from different positionalities or theoretical commitments, might construct different but equally valid interpretations. We regard this multiplicity as a strength of the interpretive paradigm.


==> wordgraves-old-dont-read/CHI/05results.tex <==
\section{Results}
\label{sec:results}

% https://arxiv.org/abs/2508.11401 -- "The four example learner groups are: KL MH =Low knowledge, high motivation; KL ML = Low knowledge, low motivation; KH ML = High knowledge, low motivation; KH MH = High knowledge, high motivation." - does it actually fit a particularly category. Different strategy targeting each personality -- could be beneficial here, they're using it with language models in educational settings

% Make sure you link it back to the RQs - make reader notice that we talk about implications and link it back to RQs
Despite carefully synchronized {\Code}, {\Memory}, and {\Metaphor} views designed to scaffold understanding, students spent nearly half their time (47\% median) focused on {\Code}, with some allocating over 70\% of attention to code even when visual representations were readily available. Why would students anchor in the representation that cognitive load theory suggests is most demanding?

This section examines how students engaged with multi-view visualizations and what shaped their selective attention. We address our research questions in two parts. Section~\ref{sec:gaze} presents gaze analyses characterizing \textit{what} students did, where they looked and how they transitioned between views (RQa). \new{Section{~\ref{sec:interviews}} draws on interview accounts to interpret \textit{why}, examining affective responses (RQb) and social positioning (RQc) that mediated uptake.}

\new{Our findings reveal three tensions that shaped engagement beyond cognitive design: control-seeking over ease, legitimacy concerns blocking playful scaffolds, and detail-fidelity as competence signals. These tensions show that visualization engagement is inseparable from emotional responses and social positioning work, \textbf{uptake dimensions} MER frameworks should account for alongside representational complementarity. External representations are not neutral tools but are filtered through learners' situated needs \cite{greeno2015commentary, greeno1997practicing}, with scaffolds working differently for novices versus experienced learners \cite{schnotz2010reanalyzing}.

Understanding these uptake dimensions matters for educational MER design: even well-designed cognitive scaffolds can fail when they conflict with students' need for control, violate disciplinary norms of what ``real learning'' looks like, or trigger social positioning concerns about appearing childish. Our observations suggest that MER frameworks for educational contexts may benefit from considering how affect and social positioning mediate engagement alongside representational complementarity. Specifically, \textbf{MER frameworks should consider incorporating}: (1) affective design principles that preserve learner agency alongside cognitive scaffolding, (2) social-positioning-aware framing that signals disciplinary legitimacy, and (3) adaptive complexity that respects students' positioning as advanced learners.}

\subsection{Gaze Patterns Across Representations}
\label{sec:gaze}

Fixation distributions varied systematically across representations and student experience (Figure~\ref{fig:gaze-subfigures}). Overall, {\Code} drew median 47\% of attention, {\Memory} 34\%, and {\Metaphor} 9\%. This pattern was task-dependent: {\Memory} engagement peaked in linked-list tasks (47\% median), while {\Metaphor} gained traction in loop tasks (19\% median).

Students with prior experience (PE, $N=13$) showed more balanced distributions ({\Code} 39.6\%, {\Memory} 43.5\%,{\Metaphor} 13.2\%), whereas novices ($N=6$) anchored heavily in {\Code} (48.1\%) with minimal {\Metaphor} use (3.3\%). Effect sizes were moderate (Cliff's $\delta = -0.28$ to 0.33) but underpowered given group sizes, consistent with prior work showing novices anchor in code traces while experienced learners coordinate multiple representations \cite{aljehane2023studying}.

Critically, transition analyses revealed integrative cross-pane movement rather than isolated viewing: {\Memory}$\leftrightarrow${\Code} transitions exceeded 11k each, with {\Metaphor} selectively consulted in {\Memory}$\rightarrow${\Metaphor}$\rightarrow${\Memory} cycles (Figure~\ref{fig:gaze-transitions}). Most participants (12/19) began with {\Memory}, then cycled between {\Code} and {\Memory} while drawing in {\Metaphor} as needed. These coordinative patterns support abstraction \cite{ainsworth2006deft} and representational flexibility \cite{hill2015online, suh2007developing}.


These patterns show students actively coordinated views rather than passively consuming them, yet with clear \Code-anchoring. To understand \textit{why} students allocated attention this way, we now examine interview accounts revealing the affective (RQb) and social (RQc) dimensions that shaped these strategies.

\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.35\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/gaze_distributions.pdf}
    \caption{Overall proportion of dwell time in each area of interest (AOI). Across all participants, the {\Code}\ pane drew the most fixations, followed by {\Memory}\ and {\Metaphor}. Because these values are medians across participants, they 
do not sum exactly to 100\%.}
    \label{fig:gaze-distribution}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.6\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/cohort.pdf}
    \caption{Median fixation distributions for learner cohorts identified via clustering on AOI dwell percentages. Symbols mark cohort medians (\emph{Code-focused}, \emph{Memory-focused}, \emph{Balanced}), with horizontal bars spanning observed ranges.}
    \label{fig:cohort}
  \end{subfigure}
  \caption{Gaze fixations across panes in MER.}
  \label{fig:gaze-subfigures}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.85\linewidth]{figures/gaze_transitions.pdf}
  \caption{Transition frequencies across AOIs, showing integrative cross-pane movement in MER vs narrower loops in Python Tutor.}
  \label{fig:gaze-transitions}
\end{figure}

\subsection{Interview Accounts: Why Students Engaged Selectively}
\label{sec:interviews}

\new{The gaze patterns above reveal \textit{what} students did. Drawing on interview accounts, we now interpret \textit{why} they engaged this way. Students' selective attention reflected not just cognitive strategies but affective responses, frustration with density, desire for control, seeking confidence, and social positioning through tool choice. We identify three tensions that mediated engagement, directly addressing questions about affective responses (RQb) and social factors (RQc) shaping uptake. We present these as dimensions that characterized variation in our sample, recognizing that their relative importance and generalizability require validation in broader contexts.}

\subsubsection{Control-Seeking Over Cognitive Ease (RQb)}

\new{Students' {\Code}-dominant gaze patterns (47\% median, with $P2_A$ at 70.9\% and $P8_A$ at 90.3\%) reflected not just habit but active \textbf{agency-seeking}}. When asked why they focused on {\Code} despite available visual scaffolds, students framed manual tracing as essential to feeling ``in control'' rather than ``just observing.'' 

As $P6_A$ explained:

\begin{myquote2}[$P6_A$ (PE, BAB, Man)]
I like tracing things on my own because I feel like I'm more in control. When I just press `Next,' I don't really know what's happening, I'm just kind of observing. But when you trace it yourself, you really have to understand how Python is going to execute the code.
\end{myquote2}

\new{$P11_A$ went further, explicitly valuing cognitive effort: ``With Python Tutor, you really have to get into the zone...It takes effort and focus not to get overwhelmed,'' \textbf{framing difficulty as productive}. This code-centricity provided an affective reward of autonomous mastery that visualization-guided exploration could not match.}

\new{\textbf{This challenges MER's assumption} \cite{sweller2011cognitive, paas2003cognitive} that reducing cognitive load increases engagement. For these students, preserving active effort was more important than visual scaffolding (RQb). The high frequency of {\Memory}$\rightarrow${\Code}$\rightarrow${\Memory} gaze transitions (11k+) further supports this: students used visualizations for \textit{verification} rather than primary reasoning, maintaining {\Code}-based mental models while selectively consulting {\Memory} for confidence-building.}

\new{\textbf{Design implication}: The instinctive response to struggling learners is to \textit{reduce} friction by automating stepping, simplifying representations, guiding attention more aggressively. Our findings reveal this intuition is inaccurate for some students. \textbf{Counter-intuitively, effective MER tools should preserve cognitive effort, not eliminate it}. Students actively resisted automation precisely because it felt passive, undermining their sense of constructive engagement. This suggests a design paradigm shift: rather than progressive \textit{simplification} (the obvious path), tools should support progressive \textit{disclosure with learner control}, scaffolding that respects agency by letting students \textit{choose} when to engage visual supports, not \textit{replacing} their mental work with visualization-driven stepping. The non-obvious insight is that \textbf{some friction is a feature, not a bug}, removing it can paradoxically decrease engagement by stripping away the very sense of mastery that motivates learning.}

\begin{designrec}{Preserve Agency Through Prediction-Based Verification}
\new{Implement learner-controlled stepping where visualizations remain hidden until students explicitly request them at self-selected checkpoints, with prediction prompts that let students commit to expected states before revealing views. This preserves agency by ensuring students control when and whether to consult visual supports, not just what they see.}
\end{designrec}

\subsubsection{Frustration with Visual Density (RQb)}
Low {\Metaphor} engagement (9\% median, 3.3\% for novices) accompanied expressions of frustration with visual complexity. Multiple students described feeling overwhelmed by metaphorical elements. \new{$P6_A$, who spent minimal time on {\Metaphor}, explained ``didn't really use it because it just looked too complicated.''} $P8_A$ elaborated on this visual overwhelm across multiple views:

\begin{myquote2}[$P8_A$ (PE, BAB, Man)]
I really don't like when there are just a bunch of arrows pointing everywhere [in {\Memory}]. Once multiple things are happening at once, there are just too many arrows on the screen, and your brain has to keep track of where they all go. It kind of ruins the clarity. [...] There were just too many things going on [in {\Metaphor}], like a house, a chimney, people calling each other. It was a lot.
\end{myquote2}

This rapid disengagement, dismissing views almost immediately rather than sustained engagement, was especially pronounced among novices. \new{The five novice participants showed varied {\Metaphor} engagement (ranging from 0.7\% to 11.2\%), but their median (3.3\%) was far below students with prior experience (13.2\%), despite identical visual designs.} When asked why, students pointed to interpretive burden: understanding what houses, chimneys, or magicians represented created additional cognitive work rather than reducing it.

However, reactions varied widely. While some found metaphors overwhelming, others embraced them as essential. $P4_B$ explained:
\begin{myquote2}[$P4_B$ (PE, BAB, Man)]
In computer science, some concepts are really abstract, and to understand them you need to connect them to something you've already experienced. Lockers for memory models, supermarket shelves for searching. Honestly, if it wasn't for that, I don't think I would have really grasped the concept.
\end{myquote2}

\new{\textbf{This challenges concreteness fading theory} \cite{fyfe2014concreteness, paivio1991dual}, which assumes concrete representations lower barriers. For students like $P8_A$, metaphorical mappings created \textit{new} interpretive demands (What does each element represent? How do they connect?) that overwhelmed them before they could benefit. The intended simplification became extraneous cognitive load \cite{paas2003cognitive} (RQb). Yet for students like $P4_B$, these same metaphors were foundational to understanding.}

\new{This reveals that representational complexity is relative to learner readiness and cognitive style, not inherent to design. As }\citet{wong2025spectrum} \new{found in their study of software developers, \textbf{psychological needs manifest along continua with substantial individual variation}, suggesting engagement dimensions operate as spectra rather than categories.}

\new{\textbf{Design implication}: Concreteness fading theory \cite{fyfe2014concreteness} and dual coding theory \cite{paivio1991dual} suggest familiar metaphors lower cognitive barriers. \textbf{Counter-intuitively, what counts as ``concrete'' or ``overwhelming' varied drastically}: $P8_A$ found even arrows overwhelming while $P4_B$ depended on metaphors for understanding. What MER frames as universally complementary \cite{ainsworth2006deft} became extraneous load \cite{paas2003cognitive} for some yet essential for others, despite identical designs. The design suggestion here is to \textbf{enable representational choice} through toggleable abstraction levels, letting learners calibrate visual density to individual capacity. There is no universal ``concrete''; MER tools need configurability as a core principle, and not just an advanced feature. This challenges MER's assumption that well-designed complementary representations universally support learning \cite{ainsworth2006deft}, revealing that complementarity is conditional on individual interpretive capacity.}

\begin{designrec}{Enable Learner-Calibrated Visual Density}
\new{Provide toggleable abstraction levels that let students progressively reveal or hide metaphorical elements (e.g., show only arrows vs. full house metaphors), with saved preferences across sessions, recognizing that what counts as ``concrete'' versus ``overwhelming'' varies drastically by learner background and current capacity.}
\end{designrec}

\subsubsection{Legitimacy Concerns Block Playful Scaffolds (RQc)}

Low {\Metaphor} engagement (9\% median overall, 3.3\% for novices vs 13.2\% for PE students) reflected not just cognitive overload but \textbf{social positioning}. Students explicitly rejected metaphors as ``childish'' and an ``ego thing,'' distancing themselves from representations they deemed illegitimate for university-level work, even when acknowledging potential pedagogical value. $P18_A$ articulated this tension:

\begin{myquote2}[$P18_A$ (no PE, BAB, Man)]
As like a university student using these kind of graphics is kind of, want to say, like, definitely not demeaning, but, like you know, kind of almost a little bit childish. But then again, it might just be like ego and personal bias.
\end{myquote2}

\new{$P1_B$ (13.1\% {\Metaphor}) echoed this, linking playful visuals to elementary education: ``when there's a bunny and a magician it kind of feels like something that would be elementary...That's kind of like an ego thing.'' Strikingly, both explicitly named ``ego.'' They didn't criticize visuals for pedagogical failure but worried about appearing childish.}

This positioning overrode learning benefits: \new{$P18_A$ (novice, 10.4\% {\Metaphor})} could have benefited most from visual scaffolds yet avoided them to signal seriousness. Others relegated metaphors to ``beginners'' ($P2_B$) or ``kids'' ($P13_A$), implicitly claiming advanced status. However, \new{$P4_B$ (23.9\% {\Metaphor}, nearly double the median) embraced analogies as central to their learning strategies: ``I always think in analogies.'' This divergence reveals that resistance can be \textbf{social, not cognitive}.}

\new{\textbf{This extends MER theory} by showing social positioning and disciplinary norms \cite{gee2000chapter, nasir2006exploring} (RQc) can block engagement independent of representational quality. Well-designed scaffolds failed when they violated students' sense of academic legitimacy.} 

\new{\textbf{Design implication}: Pedagogical theory emphasizes concrete, familiar metaphors to make abstract concepts accessible \cite{fyfe2014concreteness, paivio1991dual}, assuming approachability increases engagement. \textbf{Counter-intuitively, even effective scaffolds can fail when they threaten academic identity}, students avoided ``childish'' visualizations to signal seriousness, prioritizing legitimacy over learning support. This reveals that MER theory should account for social positioning alongside cognitive design, pedagogical effectiveness alone cannot drive adoption when tools signal inappropriate disciplinary identity.}

\begin{designrec}{Provide Framing Options for Metaphor Style}
\new{Provide explicit framing options that let students choose their preferred metaphor style at the start: `Technical Mode' (traditional diagrams, professional terminology) vs. `Conceptual Mode' (analogies, everyday metaphors) vs. `Hybrid Mode' (toggleable). Label choices to signal legitimacy (e.g., `Industry-standard notation' vs. `Pedagogical scaffolds'), allowing students to control social positioning while accessing appropriate supports.}
\end{designrec}

\subsubsection{Detail-Fidelity as Competence Signal (RQb + RQc)}

Students' heavy {\Memory} engagement in linked-list tasks (47\% median) was accompanied by resistance to function-level abstraction. $P8_A$ argued that compressing execution ``defeats the purpose'':

\begin{myquote2}[$P8_A$ (PE, BAB, Man)]
The problem with the MER {\Memory} visualization for linked lists is that it doesn't go line by line through what the append function actually does. It just executes the whole function and then shows the result. That kind of defeats the purpose of {\Memory} visualization.
\end{myquote2}

$P1_B$ preferred line-by-line pacing because it was ``especially useful for debugging.'' The issue wasn't accuracy, function-level views were correct, but whether abstraction meant skipping important learning. Students equated \textit{exhaustive tracing with real understanding} and \textit{technical fidelity with legitimacy}. \new{$P13_A$ made this explicit: ``In the context of CS2, understanding the detail behind things is expected. You need to keep the technical elements.''}

Conversely, when visualizations matched familiar practices, they felt legitimate. \new{$P12_A$ described {\Memory} as matching what they would ``draw out'' themselves, and $P14_A$ noted MER ``does all the crossing out'' they would do manually.} This suggests students validated representations through \textbf{resemblance to existing practices} \cite{reber2017processing, scheiter2020effort} rather than pedagogical value.

\new{\textbf{This reveals a tension between scaffolding and legitimacy} (RQb + RQc): function-level abstraction, designed to reduce cognitive load \cite{paas2003cognitive}, was rejected as insufficiently rigorous.}

\new{\textbf{Design implication}: Students rejected function-level abstraction not for inaccuracy but because it felt like ``skipping'' learning, equating exhaustive tracing with competence and technical detail with rigor. \textbf{Counter-intuitively, abstraction designed to reduce cognitive load} \cite{paas2003cognitive} \textbf{was perceived as pedagogically insufficient}, violating expectations that ``understanding the detail behind things is expected'' in advanced courses. This reveals a fundamental tension between MER's scaffolding goals (reduce load) and students' competence signaling (demonstrate thoroughness), suggesting that abstraction should be learner-controlled rather than designer-imposed.}

\begin{designrec}{Provide Expandable Execution Granularity with Default Detail}
\new{Implement hierarchical stepping where function calls initially expand to show line-by-line execution, with clearly labeled collapse controls students can invoke when ready, reversing typical progressive disclosure by defaulting to detail rather than simplification}
\end{designrec}

\subsubsection{Confidence Through Integrative Use (RQb)}

While frustration drove avoidance and control-seeking led to code-anchoring, some students used visualizations for \textit{reassurance}. \new{Students with balanced gaze distributions, $P9_A$ (37.5\% {\Code}, 45.8\% {\Memory}, 16.7\% {\Metaphor}) and $P10_A$ (similar balance) described using views complementarily. $P10_A$ explained: ``A lot was going on, so I started with the more abstract {\Metaphor} visual to get a basic sense, then used the {\Memory} pane to understand more in detail. Using them together worked really well.''}

\new{$P11_A$ described using {\Metaphor} for flow and {\Memory} for verification: ``The {\Metaphor} helps guide your attention...But the {\Memory} model gives you a clearer sense of what you actually have in {\Memory}...That confirmed that my foundation was solid.''} This strategic flexibility, using different representations for different epistemic needs, distinguishes integrative use from mere preference. From a learning perspective, 
such cross-representational coordination fosters representational competence as translating between complementary views helps link execution details with higher-level program structure \cite{ainsworth2006deft, daniel2018representational}.

The affective benefit was \textbf{confidence-building} (RQb): checking Code-based reasoning against visual execution. \new{This explains high {\Memory}$\leftrightarrow${\Code} transitions (11k+ transition frequencies), students were not passively viewing but actively seeking verification.} When visualizations supported rather than replaced reasoning, they provided affective rewards.

\new{\textbf{Design implication}: Balanced users strategically leveraged multiple views for different purposes, using {\Metaphor} for flow, {\Memory} for state, and {\Code} as anchor, with high transition frequencies indicating active cross-checking rather than passive viewing. \textbf{Counter-intuitively, visualizations succeeded not by explaining execution but by confirming student-driven reasoning}, providing what students called ``confirmation that my foundation was solid.'' This reframes MER tools from pedagogical guides (explaining execution) to confidence instruments (validating student reasoning), suggesting that verification workflows may be more affectively rewarding than explanation workflows in educational contexts.}

\begin{designrec}{Support Cross-Representational Verification}
\new{Provide explicit mechanisms for checking consistency across views: synchronized highlighting that shows corresponding elements across {\Code}, {\Memory}, and {\Metaphor} panes when students hover or click; visual difference indicators that flag discrepancies between predicted and actual state; and multi-view comparison modes that let students place views side-by-side for manual verification of their mental models.}
\end{designrec}
\subsection{Synthesizing Uptake Dimensions for Educational MER}
\label{sec:uptake-synthesis}

\new{The patterns above reveal three \textbf{uptake dimensions} that mediate engagement with multi-representational tools beyond cognitive design principles:

\textbf{1. Agency Preservation (RQb):} Students' need to control cognitive effort, not simply have it reduced. MER's emphasis on reducing extraneous load \cite{paas2003cognitive, sweller2011cognitive} should be balanced against preserving active construction that students associate with real understanding.

\textbf{2. Representational Calibration (RQb):} Individual variation in what counts as ``concrete'' or ``overwhelming.'' What DeFT frames as complementary constraint \cite{ainsworth2006deft} can become extraneous load depending on learner-specific interpretive capacity \cite{wong2025spectrum}.

\textbf{3. Legitimacy Positioning (RQc):} Social concerns about what tools signal regarding academic identity. Pedagogical effectiveness doesn't drive adoption when tools threaten how learners position themselves within their community \cite{gee2000chapter, nasir2006exploring}.

These dimensions operate \textit{alongside} but \textit{independently from} MER's cognitive principles of complementarity, constraint, and construction \cite{ainsworth2006deft}. A visualization can be well-coordinated yet fail if it violates agency, miscalibrates to individual needs, or signals inappropriate positioning. This explains why students with identical backgrounds responded so differently to the same designs, and why effective scaffolds were rejected when they conflicted with affective or social needs.}

==> wordgraves-old-dont-read/pre-rr/05results.tex <==
\section{Results}
\label{sec:results}
This section we present results from gaze analyses and interview accounts, organized to show how students used {\Code}, {\Memory}, and {\Metaphor} and how these uses varied by experience and task.

Program visualizations were not fixed or self-evident views of program behavior. It appeared that their perceived usefulness depended on students’ situated engagements, shaped by prior experience, disciplinary positioning, and learning goals. This aligns with the \textit{expertise reversal effect} \cite{schnotz2010reanalyzing} and with views of external representations as interpretively flexible tools whose value depends on how learners take them up \cite{greeno2015commentary, greeno1997practicing}. We foreground interview accounts from our 19 participants as primary evidence, with gaze-tracking patterns across ~{\Code}, ~{\Memory}, and ~{\Metaphor} providing descriptive context and exploratory triangulation.


\subsection{Gaze in Multi-Representation Tools}
\label{sec:gaze}
We examined fixation distributions across areas of interest (AOIs). These findings are descriptive and exploratory, and we avoid strong causal claims given the small sample.

Fixation patterns varied across tasks (Table~\ref{tab:task-dwell-mini}). {\Code} generally drew the largest share (Table~\ref{tab:task-dwell-mini}), but {\Memory} was especially prominent for linked lists (median 47\%), while {\Metaphor} gained traction in while-loop tasks (median 19\%). 
This suggests that learners used {\Code} as an anchor, supplemented by {\Memory} for structural reasoning and by {\Metaphor} when reasoning about iteration (Figure~\ref{fig:gaze-distribution}).

\input{figures/bars-gaze}

Students with prior experience (PE, $N=13$) showed a more balanced distribution ({\Code} 39.6\%, {\Memory} 43.5\%, {\Metaphor} 13.2\%), whereas novices ($N=6$) relied on {\Code} (48.1\%) with little {\Metaphor} use (3.3\%). Across tasks, {\Code} remained a central anchor, dominating for novices (47–79\%) and still substantial for PE students (36–48\%), even when {\Memory} was equally or more prominent. Median contrasts were moderate (Cliff’s $\delta=-0.28$ for {\Code}, $\delta=0.33$ for {\Metaphor}) but not significant after correction, consistent with prior work that novices anchor in code traces while experienced learners coordinate multiple representations~\cite{aljehane2023studying}.


Task-level analysis showed the same pattern. In scope tasks, novices ($N=3$) were almost entirely code-focused ({\Code} 79\%, {\Metaphor} 0\%), while students with PE balanced {\Code} (48\%), {\Memory} (42\%), and {\Metaphor} (11\%). In while-loops, both groups used {\Metaphor} more (PE 19\%, N 13\%), but novices again relied on {\Memory}$\rightarrow${\Code} transitions (38\%) compared to students with PE (22\%). In linked lists, novices fixated heavily on {\Code} (47\%) and showed few transitions to {\Metaphor} (2\%), while students with PE distributed time across {\Memory} (45\%) and {\Metaphor} (16\%) and showed more {\Memory}$\rightarrow${\Metaphor} transitions (14\%). Effect sizes for these contrasts were moderate to large (Cliff’s $\delta$ values around $\pm$0.45 to 0.64), though small group sizes limited statistical power.


Transitions overall revealed integrative cross-pane movement (Figure~\ref{fig:gaze-transitions}). The most frequent were {\Memory}$\leftrightarrow${\Code} (over 11k transitions each). {\Metaphor} was selectively integrated, especially in loops ({\Memory}$\rightarrow${\Metaphor}$\rightarrow${\Memory}). Entry analyses showed most learners began with {\Memory} (12 participants), then cycled between {\Code} and {\Memory}, drawing in {\Metaphor} as needed. These results suggest that learners were not only viewing the panes but coordinating them, which supports abstraction~\cite{ainsworth2006deft} and representational flexibility~\cite{hill2015online,suh2007developing}.

\textbf{Summary (RQa).} Overall, gaze data show that learners treated {\Code} as primary while using MER’s tri-pane layout for integration. Students with prior experience used {\Metaphor} more often and switched between views more flexibly, while novices focused on code and returned to it repeatedly. These patterns show how students used the three synchronized views: they focused on code while selectively consulting memory and metaphor views, with experienced students integrating views more flexibly than novices. This reveals that students filter representations through their experience and task needs. In the following section, we draw on interview accounts to interpret \textit{why} these patterns emerged, examining the affective responses (RQb) and social factors (RQc) that shaped students' selective attention and tool-use strategies.

\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.35\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/gaze_distributions.pdf}
    \caption{Overall proportion of dwell time in each area of interest (AOI). Across all participants, the {\Code}\ pane drew the most fixations, followed by {\Memory}\ and {\Metaphor}. Because these values are medians across participants, they 
do not sum exactly to 100\%.}
    \label{fig:gaze-distribution}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.6\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/cohort.pdf}
    \caption{Median fixation distributions for learner cohorts identified via clustering on AOI dwell percentages. Symbols mark cohort medians (\emph{Code-focused}, \emph{Memory-focused}, \emph{Balanced}), with horizontal bars spanning observed ranges.}
    \label{fig:cohort}
  \end{subfigure}
  \caption{Gaze fixations across panes in MER.}
  \label{fig:gaze-subfigures}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.85\linewidth]{figures/gaze_transitions.pdf}
  \caption{Transition frequencies across AOIs, showing integrative cross-pane movement in MER vs narrower loops in Python Tutor.}
  \label{fig:gaze-transitions}
\end{figure}

\subsection{Interview Accounts}

\new{The gaze patterns above (Section~{\ref{sec:gaze}}) reveal \textit{what} students did. Drawing on interview accounts, we now interpret \textit{why} they engaged this way. Students' selective attention reflect not just cognitive strategies, but also their affective responses: frustration with density, desire for control, seeking confidence, and social positioning through tool choice. These dimensions directly address our questions about affective responses (RQb) and social factors (RQc) shaping engagement.}%



\comment{
The interview data form the core of our analysis, from which we constructed the following themes:
(1) \textit{Code as Anchor}, 
(2) \textit{Overwhelmed by Detail}, 
(3) \textit{Using Visuals in Combination}, 
(4) \textit{Ease and Effort}, 
(5) \textit{Line-by-Line vs. Function-Level}, and 
(6) \textit{Familiarity, Playfulness, and Legitimacy}. 
Gaze findings from above are included where they provide descriptive support.
}

\subsubsection{Affective Dimensions of Engagement (RQb).}
\new{Three affective patterns showed how students allocated attentions: code-anchoring as a means for control, visual overwhelm, and integrative use of visuals for confidence-building.}

\paragraph{Code as Anchor: Control as Affective Need.}
Gaze analyses showed that participants fixated most on {\Code} (\new{median 47\%, Section{~\ref{sec:gaze}}}). Interviews revealed this reflected a need for \textit{control}. As $P6_A$ explained, they traced {\Code} step by step, with {\Memory} being a secondary focus:
\begin{myquote2}[$P6_A$ (PE, BAB, Man)]
For me, I mostly stuck to tracing the {\Code}. I could just go step by step, like, okay, it goes here, then here, and then I can say, `X is this, Y is that.' I found that approach helpful. I also found the {\Memory} analogy helpful because I could see it visually and follow what was happening. But the {\Metaphor} analogy, I didn’t really use it. It just looked too complicated.
\end{myquote2}

\new{This code-centricity was especially pronounced for some participants: $P2_A$ spent 70.9\% of time on Code (1.0\% on {\Metaphor}), while $P8_A$ allocated 
90.3\% to Code (0.7\% {\Metaphor}). When asked about this preference, students framed self-directed tracing as essential to confidence:}

\begin{myquote2}[$P6_A$ (PE, BAB, Man)]
I like tracing things on my own because I feel like I'm more in control. When I just press `Next,' I don't really know what's happening, I'm just kind of observing. But when you trace it yourself, you really have to understand how Python is going to execute the code, if that makes sense.
\end{myquote2}

$P11_A$ went further, suggesting that cognitive ease might undermine learning:
\begin{myquote2}[$P11_A$ (PE, ABA, Man)]
With Python Tutor, you really have to get into the zone. You need to consciously put yourself in the mindset of, `Okay, now I'm looking at Python Tutor. These elements are placed in specific positions, and I have to remind myself what each one means.' It takes effort and focus not to get overwhelmed.
\end{myquote2}

The code-dominance pattern thus reflected not just habit, but that the \textit{feeling} of control, even if it meant more work, was valued over the ease of visualization-guided exploration. This affective dimension helps explain why students allocated so much attention to {\Code} even when synchronized {\Memory} and {\Metaphor} views were readily available, code-tracing provided an affective reward of autonomous mastery that visualization could not match.


\paragraph{Overwhelmed by Visual Density.}
Students also mentioned focusing on {\Code} because they found {\Memory} and {\Metaphor} too cluttered. \new{The low engagement with {\Metaphor} (median 9\% dwell time) was accompanied by expressions of frustration. $P8_A$, who spent only 0.7\% of time on {\Metaphor} despite 90.3\% on {\Code} and 9\% on {\Memory}, described both {\Metaphor} and {\Memory} views as overwhelming.}

\begin{myquote2}[$P8_A$ (PE, BAB, Man)]
I really don’t like when there are just a bunch of arrows pointing everywhere [in {\Memory}]. Once multiple things are happening at once, there are just too many arrows on the screen, and your brain has to keep track of where they all go. It kind of ruins the clarity. [...]. There were just too many things going on [in {\Metaphor}], like a house, a chimney, people calling each other. It was a lot.
\end{myquote2}

\new{Similarly, $P6_A$ found the {\Metaphor} pane ``too complicated'' and ``didn't really use it.'' The phrase ``didn't really use it'' suggests rapid disengagement, students appeared to dismiss these views almost immediately rather than spending some time understanding them. This pattern was particularly pronounced among novices. In Section {\ref{sec:gaze}}, we reported that novices allocated only 3.3\% median time to {\Metaphor} compared to 13.2\% for students with prior experience, despite encountering identical visual designs. The five novice participants showed varied {\Metaphor} engagement: $P15_A$ 0.7\%, $P16_A$ 2.9\%, $P19_A$ 9.0\%, $P17_A$ 11.2\%, and $P18_A$ 10.4\%. The difference suggests that engaging with metaphorical scaffolds requires cognitive capacity, novices, already managing high intrinsic load from unfamiliar programming  concepts, experienced metaphorical elements (houses, magicians, rabbits) as additional burdens rather than helpful scaffolds.}

\new{This challenges a core assumption in concreteness fading and dual coding theory~\cite{fyfe2014concreteness, paivio1990mental}, that concrete representations lower barriers to entry. For these students, metaphorical mappings created \textit{new} interpretive work (What does the house represent? Why is there a chimney?), overwhelming learners before they could benefit from the scaffold. The intended simplification became extraneous load~\cite{paas2003cognitive}.}

\new{However, some students drew the opposite conclusion. For $P18_A$ (no PE, 10.4\% {\Metaphor}, 69.3\% {\Memory}) visualizations in advanced courses had to retain technical fidelity, even if that increased complexity.}
\begin{myquote2}[$P13_A$ (PE, ABA, Woman)]
In the context of CS2, understanding the detail behind things is expected. You need to keep the technical elements in the visualizations.
\end{myquote2}

\new{These accounts reveal a design dilemma: adding visual elements to support understanding can paradoxically reduce clarity when learners experience each 
additional element as something new to track. For $P13_A$, arrows in {\Memory} weren't helpful annotations, they were \textit{more things to manage}. This suggests the issue wasn't just visual density, but whether visual elements provided meaningful structure or felt like arbitrary decoration. The same design choice (adding concrete metaphors) that helps experienced learners overwhelms novices, suggesting that representational complexity might be relative to learner readiness, not inherent to the design.}


\paragraph{Confidence Through Integrative Use.}
\new{While frustration drove avoidance and control-seeking led to code-anchoring, some 
students used visualizations for \textit{reassurance}. Students with balanced gaze distributions, $P8_A$ (37.1\% {\Code}, 52.2\% {\Memory}, 10.7\% {\Metaphor}) and $P9_A$ (37.5\% {\Code}, 45.8\% {\Memory}, 16.7\% {\Metaphor}), described using views complementarily. $P10_A$ explained:}

\begin{myquote2}[$P10_A$ (PE, BAB, Man)]
A lot was going on, so I started with the more abstract {\Metaphor} visual to get a basic sense, then used the {\Memory} pane to understand more in detail. But I also looked at the {\Code} line by line. Using them together, side by side, worked really well.
\end{myquote2}

\new{$P11_A$ described using {\Metaphor} for flow and {\Memory} for verification:}

\begin{myquote2}[$P11_A$ (PE, ABA, Man)]
The {\Metaphor} analogy helps guide your attention, it shows you where things are going. But the {\Memory} model gives you a clearer sense of what you actually have in {\Memory}. [...] What the {\Memory} visualization lets me do is verify whether that initial assumption is actually correct. And in this case, I could clearly see that the outer \texttt{a} wasn't changed, it really was just a local variable. That confirmed that my foundation was solid.
\end{myquote2}

\new{These students positioned visualizations as tools for \textit{checking} code-based reasoning, not replacing it. The affective benefit was reassurance, confirming that mental simulation matched actual execution. This explains the high {\Memory}$\leftrightarrow${\Code} transition frequencies (over 11k transitions, Section{~\ref{sec:gaze}}): students weren't passively viewing, but actively seeking verification. $P3_B$ articulated this task-specific usage explicitly:}

\begin{myquote2}[$P3_B$ (PE, ABA, Man)]
If I wanted to trace something or go through a loop, I would definitely prefer the {\Metaphor} visualization. But maybe for implementing functions, I'd prefer something that's closer to Python Tutor, so I know how it works and can use that to my advantage.
\end{myquote2}

\new{$P11_A$ described shifting strategically between modes: passive (letting visuals guide), reactive (debugging with visuals), and proactive (verification). This strategic flexibility, using different representations for different epistemic needs, is what distinguishes integrative use from mere preference. From a learning perspective, such cross-representational coordination fosters representational competence as translating between complementary views helps link execution details with higher-level program structure~\cite{ainsworth2006deft, daniel2018representational}.

\textbf{Summary (RQb).} Three affective patterns shaped engagement: (1) frustration with visual density drove {\Metaphor} avoidance, especially among novices; (2) desire for control led to code-anchoring even when other views were available; (3) confidence-seeking supported integrative use of {\Memory} for verification. Visualization engagement was shaped not just by cognitive load, but by how tools supported students' need for control, manageable complexity, and reassurance that their understanding was correct.}

\subsubsection{Social Positioning and Resistance (RQc)}
\label{sec:positioning}
\new{Beyond affective responses, students' engagement reflected how they positioned themselves as learners, with judgments about which tools were legitimate for serious study. Students rejected visualizations they deemed ``childish,'' demanded technical fidelity, and gravitated toward representations matching familiar practices.}

\begin{myquote2}[$P18_A$ (no PE, BAB, Man)]
As like a university student using these kind of graphics is kind of, want to say, like, definitely not demeaning, but, like you know, kind of almost a little bit childish. But then again, it might just be like ego and personal bias.
\end{myquote2}

\new{$P1_B$ (13.1\% {\Metaphor}} echoed this concern, linking it explicitly to academic pride.

\begin{myquote2}[$P1_B$ (PE, ABA, Man)]
It's like when there's a bunny and a magician it kind of feels like something that would be elementary. Especially in a university setting, I feel like people would want more formal things to justify what they're learning. That's kind of like an ego thing.
\end{myquote2}

\new{It is striking that both students mentioned ``ego'' here. They didn't criticize the visuals for failing to help them learn. Instead, they worried about legitimacy, not wanting to look childish for learning with visual metaphors. This shows that concerns about how they appeared actually influenced where they looked. $P18_A$ was a beginner who could have benefited most from the abstract {\Metaphor} visuals, yet spent only 10.4\% of their time looking at them. This suggests that worries about their identity can outweigh learning benefits.}

Students also distanced themselves by assigning playful visuals to other audiences. $P2_B$ and $P13_A$ validated metaphors for ``beginners'' or ``kids,'' implicitly claiming advanced status for themselves:

\begin{myquote2}[$P2_B$ (PE, BAB, Man)]
[{\Metaphor}] would be great for a beginner, especially someone who doesn't yet understand frames. The houses, the people, and the visuals showing how values are returned help make things clearer. But once you have a general idea, [{\Memory}] is easier to follow.
\end{myquote2}

\begin{myquote2}[$P13_A$ (PE, ABA, Woman)]
If the learners are kids, then I'd prefer the bunny-style {\Metaphor} visual, it's more playful and approachable. But in the context of a course like [CS2], we should definitely include the global frame, because that's part of the curriculum.
\end{myquote2}

$P13_A$ \new{(0.7\% {\Metaphor}, 90.3\% {\Code}), who spent minimal time on {\Metaphor} despite high engagement overall}, framed this preference in curricular terms: technical fidelity became a marker of belonging to advanced coursework. By relegating metaphors to others, students protected their positioning as serious learners.

Yet not all students experienced playfulness as threatening. $P4_B$ \new{(23.9\% {\Metaphor}, 40.2\% {\Memory}, 35.9\% {\Code})} described analogy as essential to their learning identity:

\begin{myquote2}[$P4_B$ (PE, BAB, Man)]
I always think in analogies. In computer science, some concepts are really abstract, and to understand them you need to connect them to something you've already experienced. Lockers for memory models, supermarket shelves for searching. Honestly, if it wasn't for that, I don't think I would have 
really grasped the concept.
\end{myquote2}

This divergence shows how representational choices filtered through positioning: what felt illegitimate to some anchored others' sensemaking. \new{$P4_B$'s high {\Metaphor} engagement (23.9\%, nearly double the median) matched their stated reliance on metaphorical thinking, demonstrating that when analogies align with learning identity, students embrace rather than resist playful scaffolds.}


\paragraph{Line-by-Line vs. Function-Level Execution}
Students also resisted design decisions that compressed execution details. In linked-list tasks, where students fixated heavily on {\Memory} \new{(median 47\%,} Section~\ref{sec:gaze}), $P8_A$ argued that function-level stepping undermined visualization's purpose:

\begin{myquote2}[$P8_A$ (PE, BAB, Man)]
The problem with the MER {\Memory} visualization for linked lists is that it doesn't go line by line through what the append function actually does. It just executes the whole function and then shows the result. That kind of defeats the purpose of {\Memory} visualization.
\end{myquote2}

$P1_B$ preferred line-by-line pacing in visualizations because it was ``especially useful for debugging.'' The issue wasn't accuracy (function-level views were correct) but whether skipping steps meant skipping important details in learning. Students wanted to see every detail because they believed `real' understanding meant tracing each step, not just seeing summaries. They viewed function-level abstraction as taking a shortcut that, like playful visuals, didn't feel right for serious learners.

This resistance reveals a tension between pedagogical scaffolding and legitimacy. Line-by-line pacing can help novices manage complexity~\cite{khalil2005interactive}, but may also reinforce notions that legitimate learning requires exhaustive manual 
tracing~\cite{layman2025topic, zingaro2018identifying}. Function-level views emphasize program structure but risk being dismissed as insufficiently rigorous. When students equate detailed simulation with serious learning, designs that promote abstraction may be rejected not for pedagogical reasons, but because they violate expectations about what university-level work should look like.

\paragraph{Familiarity as Legitimacy Marker.}

Finally, students judged visualizations by ``fit,'' how closely they matched existing sketching practices. When representations aligned with habits of drawing variables, 
stack frames, or pointer flows, they felt natural and legitimate. $P12_A$ described {\Memory} as matching what they would ``draw out'' themselves:

\begin{myquote2}[$P12_A$ (PE, BAB, Man)]
The {\Memory} analogy was most helpful for me, because in my courses I usually draw memory stack frames myself. Having it visualized saved me from doing that manually, and it matched the way I usually think through these problems.
\end{myquote2}

$P14_A$ \new{(9.0\% {\Metaphor})} echoed that MER simply automated existing practice:

\begin{myquote2}[$P14_A$ (no PE, BAB, Woman)]
I think honestly, like me writing a test, this is exactly what I would draw out, it already does all the crossing out.
\end{myquote2}

Students who had seen MER-style diagrams before felt they were effective simply because they were familiar~\cite{reber2017processing, scheiter2020effort}. But this raises a question: should visualizations match what learners already know and do, or should they be deliberately different to teach new ways of thinking? Matching their existing knowledge can help understanding but might prevent them from learning more abstract concepts. Unfamiliar visualizations can push students to think harder and struggle productively~\cite{gaver2003ambiguity, cox2016design, young2024productive}, though familiar ones may just feel effective without actually improving learning~\cite{scheiter2020effort}.

\textbf{Summary (RQc).} Students' backgrounds and positioning as learners influenced visualization uptake. Ego protection and legitimacy concerns led some to resist metaphor-based scaffolds regardless of pedagogical value, while others embraced the same analogies as essential tools. Students also resisted compression and gravitated toward familiar representations. Visualization engagement was thus inseparable from social positioning: students used tool choices to signal where they positioned themselves in the learning hierarchy, serious university students versus novices needing playful supports.

Across these affective and social dimensions, students showed that visualizations cannot be judged in isolation. Their value was relative to emotional responses 
(frustration, control, confidence), task demands, and the positioning students performed as learners. MER and Python Tutor each offered affordances, but these mattered differently depending on whether students sought autonomous mastery, manageable load, or signals of academic legitimacy. The ``best'' visualization was never fixed but depended on these situated factors.

==> wordgraves-old-dont-read/pre-rr/06discussion.tex <==
\section{Discussion}
\label{sec:discussion}
% They should consider while making sure to attend to blablabla -- any nuance that I can add to design implications so they see that no one with superficial knowledge could say that -- high-level guideline but something they may not have known

We conducted a within-subjects talk-aloud study in which students worked through three topical blocks using two different visualization tools in counterbalanced order. Our design probe presented synchronized \Code, \Memory, and \Metaphor panes which allowed us to compare gaze behavior and interview reflections across representations.

\paragraph{Key Takeaways:} Across our study, students focused most on \Code, and focused selectively on \Memory and \Metaphor. Rather than using the visuals as tools of understanding  \cite{hmelo1996black, sorva2013review}, they were interpreted in varied and sometimes conflicting ways. Our results contrast with prior findings that abstract visuals are valuable for novices \cite{ainsworth2006deft, rexigel2024more} as they might for experts \cite{hayatpur2023crosscode}. In our study, novices often engaged least with visual representations, while experienced learners preferred the technical detail in \Memory over the relatable analogies in \Metaphor. These patterns highlight that the value of program visualization depends not only on the form itself but may also depend on how learners are prepared to use it through training, scaffolding, and framing that align with their goals, experience, and sense of disciplinary legitimacy.

\paragraph{Code as Anchor}
Students’ descriptions and gaze data consistently pointed to \Code as their primary point of focus, which many framed as the ``real'' work of programming. In this sense, MERs supported learning by offering additional checks rather than replacing code itself. Interestingly, more experienced students anchored their reasoning but did not dwell on it. They were more fluid in their use of visualizations than novices were. 

Students mentioned using \Memory and \Metaphor when they wanted to verify an assumption or avoid sketching the program by hand.  Even when visuals were synchronized and easy to access, students still kept \Code at the center of their reasoning. This emphasis on code-as-anchor echoes prior findings that novices often ignore diagrams unless prompted \cite{schwonke2009multiple}. It also connects to work on productive struggle as students treated effortful engagement with code as central, positioning MERs as tools to reflect and confirm rather than to bypass that effort \cite{bjork2011making, young2024productive}.

For design, this raises a tension: if students see reading \Code as the only ``real'' programming, their judgments of legitimacy may limit how much they engage with supportive visualizations, even when those tools could help them. Visualizations may need to be framed and integrated as extensions of coding practice rather than as optional add-ons, so that students view them as a part of the ``real'' programming work.

\paragraph{Fidelity, Concreteness, and the Expertise Reversal Effect}
In upper-introductory programming contexts (CS2), where abstraction and structural reasoning are central, we were surprised to see some students’ preference for visual fidelity in \Memory. Rather than favoring simpler \Metaphor views, some expected diagrams to show technical details like function frames and reference links. This contrasted with our assumption, since CS2 is thought to require connecting local operations to broader structural intent in data structures  \cite{layman2025topic, zingaro2018identifying, almadhoun2021exploratory}. We expected students to lean more on conceptual representations (\Metaphor) to support this shift, yet students mentioned leaning on \Memory. However, gaze data told a more complex story as students with prior experience in fact did use \Metaphor on the linked list tasks. This suggests that learners may already be making the representational shift in practice, even if they do not frame it that way themselves.

For some, the everyday analogies in \Metaphor felt distracting or ``childish,'' while others described them as essential for making sense of abstract content. These divergent responses echo the expertise reversal effect \cite{kalyuga2007expertise}. Supports that help novices can later feel constraining or illegitimate to advanced learners. In this way, fidelity itself became a marker of rigor and seriousness. We note that we use fidelity here to mean preserving canonical details of execution (e.g., stack frames, pointer links), rather than literal correspondence to hardware.

For design, this suggests that tools may need to support both kinds of views: detail-rich \Memory for advanced learners, and approachable \Metaphor for novices. Allowing learners to switch or toggle between models could help them move from approachability toward technical detail over time.


\paragraph{Fit, Fluency, and the Role of Friction}
Some students looked for ``fit'' --- how familiar a visual felt to tools they used or diagrams they drew. When a visualization was familiar, it felt fluent, natural, and effective. These perceptions align with metacognitive judgments of fluency, where what feels easy is often taken as effective, even if ease reflects surface familiarity rather than deeper understanding \cite{reber2017processing, scheiter2020effort}. This creates a design tension. Visuals that fit learners’ habits can validate their practices but may also reinforce superficial fluency. Visuals that depart from those habits can create friction, which, if scaffolded, can lead to productive struggle and deeper learning \cite{gaver2003ambiguity, young2024productive}. Work in HCI on ambiguity and friction highlights this same point \cite{sengers2005reflective, cox2016design}. In visualization for learning, intentional departures from familiar forms can be used to slow learners down, prompting reflection and deeper processing.

We distinguish this sense of familiarity from legitimacy, which we discuss later. Familiarity reflects whether a visual feels resonant with one's own habits, whereas legitimacy is used to talk about what \textit{counts} as professional computer science. While distinct, the two may be linked---what feels unfamiliar can also be dismissed as illegetimite when it diverges too far from disciplinary norms.

For design, this means that mirroring learners’ practices can reduce effort and increase acceptance, but some friction may be necessary to move learners beyond surface fluency. The challenge is determining when and how that friction would be effective in inviting reflection without being overwhelming.  


\paragraph{Granularity and Temporal Pacing}
Our results also highlight tensions in the granularity of execution steps. Students valued stepwise, line-by-line progression for its sense of control and clarity, particularly in linked-list tasks. Function-level execution, in which entire functions were shown as a single step, was criticized as undermining the very purpose of program visualization. Stepwise displays can support novices by breaking execution into small pieces, but they may also encourage line-by-line tracing habits that limit higher-level reasoning \cite{layman2025topic, zingaro2018identifying}. Showing whole functions in one step can make program structure clearer, but may confuse learners if intermediate states are hidden.  

For design, this suggests that tools should let students move between detailed and function-level views, while seeking other ways to make them reflect on higher-level reasoning.

\paragraph{Legitimacy and Perceptions of Seriousness}
Students’ judgments were not purely about comprehension or problem-solving. Some perceived relatable \Metaphor visuals as ``childish,'' inappropriate for the seriousness of university-level learning or the computer science discipline. Others enjoyed seeing the same features and called them memorable, approachable, and personally resonant. 

These contrasting views show how students made decisions about what counts as legitimate in their context. We distinguish this idea of \textit{legitimacy} from \textit{familiarity} which we spoke about earlier. Familiarity concerned whether a visualization matched students' own prior habits or sketching. Legitimacy concerned whether a visualization signaled professional seriousness, shaping how students thought they or their peers would be perceived. In this framing, everyday analogies were often associated with novices or children, while detailed \Memory diagrams were reserved for advanced learners. Such positioning can shape uptake as much as clarity or fidelity. Students may even avoid helpful scaffolds such as concreteness fading if they fear appearing unserious. This connects with Legitimation Code Theory \cite{maton2015knowledge}, which highlights how forms of knowledge are valued differently across contexts.  

For design, the implication is less about choosing one style over the other and more about managing how different styles are framed. Analogy-based visuals can support learning for some students, but they need to be introduced in ways that signal legitimacy. At the same time, formal ~\Memory diagrams remain important for students who equate fidelity with rigor. Tools that allow both modes and that help normalize their use in different stages of learning may avoid forcing students into a choice between what feels useful and what feels serious.  

\paragraph{Integration Rather Than Substitution}
Finally, our data show that learners did not seek a single ``best'' visualization. Instead, they described using representations for different purposes: code to anchor, memory to verify, and the metaphor to follow program flow. Gaze transitions across panes also revealed integrative use, not substitution. This aligns with DeFT’s emphasis on representational complementarity~\cite{ainsworth2006deft} and with recent findings that translation among representations fosters representational competence and flexibility~\cite{daniel2018representational}. Students even imagined sequencing tools developmentally, starting with analogy-based supports in CS1, fidelity-rich diagrams in CS2. 

For design, this reinforces the value of multi-representational approaches. While many program visualization systems aim to perfect a single view, our findings show that learners value and appear to reason with multiple coordinated views. Designing for complementarity, rather than optimization of one visual, may better support the representational competence and flexibility students need.  

Ultimately, our study highlights that program visualizations do not carry fixed value, but are taken up through learners’ goals, identities, and contexts. Designing with this in mind—treating visuals as resources to be integrated, framed, and adapted—may open pathways for students to engage more flexibly and meaningfully with code.

\input{sections/07limitations}

\subsection{Future Work}  
We see a few directions for future work building on this study:  

\begin{itemize}  
    \item \textbf{Real-World Experiments.} Our study examined students in a controlled within-subjects setting. Future research can embed multi-representational tools in classroom practice, where it might be easier to measure long-term learning benefits, and how factors such as instruction can influence the uptake of these visualizations.

    \item \textbf{Longitudinal perspectives.} Our results suggest that students’ judgments of legitimacy and their preferences for fidelity versus metaphor may change as they progress through the curriculum. Longitudinal studies could trace how learners’ positioning of ~\Code, ~\Memory, and ~\Metaphor evolves from CS1 to CS2 and beyond.  

    \item \textbf{Instructional framing and scaffolding.} Students sometimes avoided visuals they viewed as ``childish'' or not serious. Future work could explore concrete ways to frame these visuals as legitimate learning tools. For example, instructors might introduce them as expert strategies rather than as beginner aids, or interfaces could label them as ``conceptual models'' to emphasize their role in abstraction. 


    \item \textbf{Programming paradigms.} Our probe focused on imperative Python examples. Comparative studies could test whether multi-representational approaches function similarly in other paradigms such as functional or object-oriented programming, where abstraction and visualization needs may differ.  

    \item \textbf{Adaptive design features.} Students in our study wanted both fidelity-rich and approachable visuals, but at different times. Future designs could support adaptive switching between views, allowing learners to move from approachability to technical detail as their goals and expertise shift.  

\end{itemize}  

Together, these directions would extend our findings from a controlled probe to broader settings, helping to identify when, how, and for whom multi-representational visualizations best support representational competence and learning.  

==> wordgraves-old-dont-read/pre-rr/results.tex <==
\comment{
\subsubsection{Using Visuals in Combination}
Students' gaze frequently moved between {\Code} and {\Memory}, with some transitions to {\Metaphor}. Qualitative data suggests that students used the views in a complementary way: while one view primed their understanding, other views helped verify or deepen it. 


\begin{myquote2}[$P10_A$ (PE, BAB, Man)]
A lot was going on, so I started with the more abstract {\Metaphor} visual to get a basic sense, then used the {\Memory} pane to understand more in detail. But I also looked at the {\Code} line by line. Using them together, side by side, worked really well.
\end{myquote2}

$P11_A$ described using {\Metaphor} for flow, and {\Memory} for technical detail:
\begin{myquote2}[$P11_A$ (PE, ABA, Man)]
The {\Metaphor} analogy helps guide your attention, it shows you where things are going. But the {\Memory} model gives you a clearer sense of what you actually have in {\Memory}.
\end{myquote2}

$P3_B$ described a more concept-specific usage: {\Metaphor} for tracing loops or flow, and {\Memory} for implentation details and correctness:
\begin{myquote2}[$P3_B$ (PE, ABA, Man)]
If I wanted to trace something or go through a loop, I would definitely prefer the {\Metaphor} visualization. But maybe for implementing functions, I’d prefer something that’s closer to Python Tutor, so I know how it works and can use that to my advantage.
\end{myquote2}
We note that this relates to the higher views of {\Metaphor} in the gaze data.

Some students, like $P2_B$ (PE, BAB, Man), anticipated changing their preferences with courses: valuing the the simpler MER visuals at first (CS1), then finding Python Tutor more useful once technical accuracy and scope rules mattered in CS2. This is surprising, since advanced topics like recursion and encapsulation might seem to call for coordinating multiple views, yet students described relying more on memory diagrams alone for technical fidelity.

Overall, student did not want a single ``best'' visualization. They combined views in tandem, aligning each with goals: orienting, checking logic, and ensuring accuracy. From a learning perspective, such cross-representational use fosters representational competence as translating between complementary views helps link execution details with higher-level program structure~\cite{ainsworth2006deft, daniel2018representational}.

\subsubsection{Ease and Effort}
Interviews suggested that students shifted between views not only for the information they provided, but also for how much thinking the visualization allowed them to avoid or required them to do. Some gravitated toward visuals that made execution obvious, while others engaged with those that slowed them down and forced reasoning, and some moved between the two. These orientations point to different learning values: ease may support quick clarity, but avoidance of effort risks undermining deeper understanding.

Some valued simplicity, praising MER for making execution clear at a glance:
\begin{myquote2}[$P11_A$ (PE, ABA, Man)]
Honestly, you could probably not even be sober and still make sense of it, because the visuals guide you through what’s happening.
\end{myquote2}

In Python Tutor, they explained, effort was unavoidable:
\begin{myquote2}[$P11_A$ (PE, ABA, Man)]
With Python Tutor, you really have to get into the zone. You need to consciously put yourself in the mindset of, `Okay, now I’m looking at Python Tutor. These elements are placed in specific positions, and I have to remind myself what each one means.' It takes effort and focus not to get overwhelmed.
\end{myquote2}

One student noted the value of cues such as next-step highlighting, which provided direction while still requiring thought:
\begin{myquote2}[$P10_A$ (PE, BAB, Man)]
What I really like is that [Python Tutor] tells me the next line that will be executed. That’s super helpful, because in a lot of code, execution doesn’t always go top to bottom, so knowing what comes next gives me a clear sense of direction.
\end{myquote2}

$P6_A$ felt that true understanding came from tracing on their own:
\begin{myquote2}[$P6_A$ (PE, BAB, Man)]
I like tracing things on my own because I feel like I’m more in control. When I just press `Next,' I don’t really know what’s happening, I’m just kind of observing. But when you trace it yourself, you really have to understand how Python is going to execute the code, if that makes sense.
\end{myquote2}

$P11_A$ described modes of use of the visualizations that shifted depending on context.
\begin{myquote2}[$P11_A$ (PE, ABA, Man)]
So really, there are three possible paths I might take when using a visual:  
Passive mode – I let the visual carry me through without much mental effort.  
Reactive mode – I’ve already made a mistake, and I turn to the visual to figure out what went wrong.  
Proactive mode – I use the visual to guard against errors, verifying as I go, even if I think I understand.
\end{myquote2}

Taken together, these accounts point to a design challenge: finding a balance where visualizations draw students into reasoning without overwhelming them. Some students gravitated toward tools that made execution obvious, while others described the value of slower, more effortful engagement. The goal is not to satisfy preferences for ease, but to design representations that keep learners engaged in productive struggle, where effort is required but still manageable~\cite{young2024productive, bjork2011making}.



\subsubsection{Line-by-Line vs. Function-Level Execution}

When working with linked lists, students fixated heavily on {\Memory}, often struggling to keep track of how values changed across lines. Interviews suggest that line-by-line unfolding helped them stay oriented, while function-level execution (treating a whole method as one step) left gaps that were harder to bridge.

$P8_A$ argued that compressed displays undermined the very purpose of visualization:  
\begin{myquote2}[$P8_A$ (PE, BAB, Man)]
The problem with the MER {\Memory} visualization for linked lists is that it doesn’t go line by line through what the append function actually does. It just executes the whole function and then shows the result. That kind of defeats the purpose of {\Memory} visualization.
\end{myquote2}

By contrast, stepwise pacing was described as keeping learners grounded in the execution:  
\begin{myquote2}[$P10_A$ (PE, BAB, Man)]
Seeing each frame introduced step by step makes it easier to follow.
\end{myquote2}

Others, like $P1_B$ (PE, ABA, Man), connected this directly to practice, noting that line-by-line pacing was ``especially useful for debugging.''

Overall, these accounts show how pacing shaped both attention and interpretation. Stepwise views anchored learners in {\Memory}, making control flow and variable changes explicit, while compressed execution provided overviews that some found too abrupt. For learning, line-by-line pacing can scaffold novices by breaking execution into manageable chunks~\cite{khalil2005interactive}, but may also reinforce simulation strategies that limit abstraction~\cite{layman2025topic, zingaro2018identifying}. Function-level views emphasize program structure but are harder for novices without intermediate states. Designs that let students move flexibly between granular and compressed views may best support the transition from tracing mechanics to abstract mental models~\cite{fyfe2014concreteness, ainsworth2006deft}.


\subsubsection{Familiarity and Fit}
A recurring theme was what students themselves called the ``fit'' of a visualization---how closely it resembled the sketches they would normally draw when tracing code. When a representation matched their habits of drawing variables, stack frames, or pointer flows, it felt natural and efficient. When it differed from those practices, students described the extra effort of re-mapping information.

$P12_A$ described MER’s {\Memory} as closely aligned with their own sketching practices: 
\begin{myquote2}[$P12_A$(PE, BAB, Man)]
The {\Memory} analogy was most helpful for me, because in my courses I usually draw memory stack frames myself. Having it visualized saved me from doing that manually, and it matched the way I usually think through these problems.
\end{myquote2}

$P14_A$ echoed that the tool simply automated what they already did:  
\begin{myquote2}[$P14_A$ (no PE, BAB, Woman)]
I think honestly, like me writing a test, this is exactly what I would draw out, it already does all the crossing out.
\end{myquote2}

For students who had seen MER-style diagrams in coursework, this familiarity made the representation feel especially intuitive ($P17_A$, $P9_A$). Such reactions reflect metacognitive judgments of fluency: when a representation feels natural, learners often equate that ease with effectiveness~\cite{reber2017processing, scheiter2020effort, bjork2011making}.  

Taken together, these accounts highlight a design tension: should visualizations mirror learners’ intuitive sketches, streamlining translation and validating their practices, or should they deliberately differ to cultivate new representational habits? Alignment with personal drawing styles can serve as a bridge to understanding, but may also constrain learners from adopting more abstract perspectives. Prior work in HCI and the learning sciences suggests that deliberate departures from familiar layouts can act as a design resource, sparking reflection and fostering productive struggle~\cite{gaver2003ambiguity, sengers2005reflective, cox2016design, young2024productive}. From a learning perspective,  familiar visuals may feel effective without strengthening mental models, while productive difficulty can encourage deeper reasoning and lasting learning~\cite{scheiter2020effort, young2024productive}.

\subsubsection{Playfulness and Legitimacy}
Some students interpreted the visuals based on how they positioned them as learners. Formal-looking visuals signaled academic legitimacy, while playful or ``childish'' ones raised concerns about pride and belonging in a university context.

Some wrestled openly with this tension. $P18_A$ describes them as childish, but noted that it might reflect his ego:
\begin{myquote2}[$P18_A$ (no PE, BAB, Man)]
As like a university student using these kind of graphics is kind of, want to say, like, definitely not demeaning, but, like you know, kind of almost a little bit childish. But then again, it might just be like ego and personal bias.
\end{myquote2}

Another echoed the concern more explicitly, linking it to academic pride:  
\begin{myquote2}[$P1_B$ (PE, ABA, Man)]
It's like when there's a bunny and a magician it kind of feels like something that would be elementary. Especially in a university setting, I feel like people would want more formal things to justify what they're learning. That's kind of like an ego thing.
\end{myquote2}

It is striking that both students explicitly mentioned \textit{ego} in framing their discomfort.  Their critiques focused less on comprehension than on legitimacy: the concern was not whether the visuals worked when learning, but the social stakes of being seen to learn with metaphors coded as childish. In this framing, formal visuals signaled rigor, while playful ones risked infantilizing.

$P2_B$ and $P13_A$'s strategy was to validate playful visuals by assigning them to a different audience: appropriate for novices, but not legitimate for university students:
\begin{myquote2}[$P2_B$ (PE, BAB, Man)]
``[{\Metaphor}] would be great for a beginner, especially someone who doesn’t yet understand frames. The houses, the people, and the visuals showing how values are returned help make things clearer. But once you have a general idea, [{\Memory}] is easier to follow.''
\end{myquote2}

\begin{myquote2}[$P13_A$ (PE, ABA, Woman)]
``If the learners are kids, then I'd prefer the bunny-style {\Metaphor} visual, it's more playful and approachable. But in the context of a course like [CS2], we should definitely include the global frame, because that's part of the curriculum.''
\end{myquote2}

Yet not all students experienced playfulness as threatening. For some, analogy was central to sensemaking and even personal style:  
\begin{myquote2}[$P4_B$ (PE, BAB, Man)]
I always think in analogies. In computer science, some concepts are really abstract, and to understand them you need to connect them to something you’ve already experienced. For me it’s always analogies. Lockers for memory models, supermarket shelves for searching. Honestly, if it wasn’t for that, I don’t think I would have really grasped the concept.
\end{myquote2}

For this learner, analogy was not incidental but a consistent practice across courses and essential for comprehension. Playful details were even welcomed, with whimsical elements like the ``hats'' analogy making concepts more memorable rather than trivializing. What one student dismissed as infantilizing, another framed as humorous and mnemonic. These divergences show how representational choices are filtered through identity: for some, seriousness and legitimacy; for others, playfulness and personal resonance. Through the lens of Legitimation Code Theory (LCT) \cite{maton2015knowledge}, playful visuals grounded abstract ideas in everyday metaphors, while formal diagrams signaled disciplinary rigor, a progression many students described as concrete supports ``for beginners'' and abstract forms for advanced learners. Calling visuals ``childish'' was thus less about effectiveness than about positioning within academic norms.

These perceptions matter for learning because they shape which scaffolds students allow themselves to use. Playful visuals can support concreteness fading and conceptual grounding~\cite{fyfe2014concreteness, mnguni2014theoretical}, but if learners deem them illegitimate, they may skip prematurely to abstract forms. More broadly, this tension highlights an unresolved question about the role of visual analogy in higher education: should such supports be embraced as essential bridges for understanding, or resisted as too playful for academic legitimacy? We return to this tension in the discussion, where we consider how analogy and formality might be productively combined.


Across these themes, students showed that visualizations cannot be judged in isolation. Their value was relative to prior habits, task demands, and the identities students performed as university learners. MER and Python Tutor each offered affordances, but these mattered differently depending on whether students sought ease, rigor, alignment with drawing practices, or help managing load. Some even combined views strategically across tasks or courses. The ``best'' visualization was never fixed but contingent. In the discussion that follows, we show how identity, effort, detail, and combination intersect in broader design tensions.
}

==> wordgraves-old-dont-read/references.tex <==
@unpublished{anon,
 author = {{Anonymous}},
 doi = {10.1093/nq/s4-iv.98.408e},
 note = {Anonymized for Review},
 title = {Anonymous},
 year = {2025}
}

@unpublished{anon2025,
 author = {{Anonymous}},
 doi = {10.1093/nq/s4-iv.98.408e},
 note = {Manuscript under review},
 title = {Anonymous},
 year = {2025}
}

==> wordgraves-old-dont-read/version0/00abstract.tex <==
\begin{abstract}
\textbf{Motivation}: CS2 students often struggle to connect low-level memory operations with high-level data structure behavior. Existing visualization tools tend to emphasize step-by-step execution without scaffolding structural abstraction, leaving learners with fragmented or shallow mental models. \\ 
\textbf{Goal}: We investigate whether multiple external representations (MERs)--a strategy widely used in disciplines like chemistry, physics, and mathematics to support abstraction--are perceived by CS2 students as usable, clear, and manageable when applied to structural abstraction tasks.
\\
\noindent
\textbf{Method}: We used a tri-pane interface, grounded in Ainsworth’s DeFT framework, as a design probe to examine how synchronized MERs are experienced by CS2 students. The system synchronized source code, memory diagrams, and abstract structural views, and was embedded in a 12-week CS2 course ($n = 695$) covering linked lists, trees, and recursion. Students interacted with weekly visualizations aligned to course content; 440 completed an end-of-term survey and 301 provided open-ended feedback. We analyzed perceived clarity, cognitive effort, and usability using validated instruments and descriptive thematic analysis.

% We used a tri-pane visualization system as a design probe to examine how synchronized MERs are experienced by CS2 students. The tool was deployed in a 12-week CS2 course (n = 695) covering linked lists, trees, and recursion. Students engaged with the visualizations weekly as part of required course activities. We collected survey responses from 440 students and analyzed clarity, usability, and cognitive load.\\ 
\noindent
\textbf{Results}: Students described the MER visuals as clear and easy to navigate, particularly for recursive and reference-based reasoning. Survey responses suggested moderate effort and strong usability, with some variation across language background and prior experience. Open-ended feedback highlighted both perceived benefits--e.g., conceptual coherence--and challenges, such as representational density.\\
\noindent
\textbf{Implications}: Synchronized, theory-informed visualizations can support CS2 learners in engaging with structural abstraction without increasing perceived cognitive load. While this study centers on perception and usability, the findings suggest that MER-based designs are interpretable, affectively engaging, and promising for future investigation. These results lay a foundation for examining how layered visual scaffolds might support learning, transfer, and abstraction in computing education.
\end{abstract}

==> wordgraves-old-dont-read/version0/01intro.tex <==
\section{Introduction}
\label{sec:intro}
\hlpink{todo: motivate looking at cognitive load earlier} \\

Despite passing CS1, students in CS2 frequently report struggling with abstraction-heavy challenges, particularly around linked lists, recursive logic, and class-based design \cite{layman2020toward, yang2018evaluations}. Visualization tools such as Python Tutor, jGRASP, and JaguarCode attempt to expose runtime behavior through detailed stack and heap diagrams \cite{guo2013online, miller2017jgrasp, cross2004jgrasp}, but they often emphasize step-by-step execution without supporting learners in generalizing to higher-level structures. Meanwhile, data structure and algorithm visualizers--such as JHAVE \cite{naps2000jhave} and VisuAlgo \cite{halim2015visualgo}--highlight structural transformations like traversals or rotations but typically omit memory-level behavior and control flow \cite{shaffer2010algorithm}. While such abstractions are appropriate for algorithm courses, CS2 students often need to reason across both layers: tracing concrete memory changes and understanding their effects on recursive structures \hlpink{[cite]}. Without explicit scaffolding across these layers, learners may struggle to integrate the control flow of recursive methods with their structural consequences \cite{sorva2013review,karnalim2017effectiveness}.

The learning-sciences literature argues that \emph{multiple external representations} (MERs) can reduce extraneous cognitive load, spur active engagement, and foster conceptual insight, especially when designs employ \emph{concreteness fading} to guide learners from concrete details toward abstractions \cite{ainsworth2006deft,fyfe2014concreteness,munzner2014visualization}.  Despite these theoretical advantages, most program-visualization tools adopted in computing classrooms still use a \emph{single}, highly detailed execution trace and offer little scaffolding for abstraction \cite{sorva2013review}. While such fine‐grained views are indeed necessary--especially for reasoning about aliasing, pointer manipulation, and low-level memory behavior--they can overwhelm novices who have not yet formed robust mental schemas for these patterns \cite{karnalim2017effectiveness, karnalim2017use}.

Building on this, interactivity may play a crucial role: prior laboratory studies suggest that interactive diagrams can lower cognitive load \cite{de2017attention}, yet others show that too much visual detail overwhelms novices \cite{ainsworth2006deft}.  How a \emph{classroom-embedded}, abstraction-focused MER design affects engagement, mental effort, and perceived clarity—and whether these effects differ by language background or prior experience—remains under-explored.

We therefore created a set of \emph{interactive MER visuals} that synchronize three panes: (i) source code, (ii) a traditional memory diagram, and (iii) an intentionally abstracted view that progressively fades detail.  Building on work done with MER representations in CS1, where students reported finding multiple representations of a program engaging \cite{anon2025}, we embedded the widgets in weekly online preparation for a 12-week CS2 course on linked lists, $n$-ary trees, and BSTs.  All 440 enrolled students saw these visualizations. As our aim was to characterize student perceptions rather than compare instructional conditions, no control-group was used. Start- and end-of-term surveys captured user experience, perceived learning benefits, cognitive load, and affect; click-stream logs recorded every interaction.

\smallskip\noindent\textbf{Research Questions.}
\begin{description}[leftmargin=0.8cm,style=sameline,labelsep=0.5cm]
    \item[\textbf{RQ1—Helpfulness \& Clarity.}] How clear and helpful do students report finding the MER visuals at the end of CS2?
    \item[\textbf{RQ2—Cognitive Load \& Usability.}] How much mental effort do students report, and how usable do they perceive the visualization system to be?
    \item[\textbf{RQ3—Learner Differences.}] Do perceptions in RQ1–RQ2 vary with language background, prior programming experience, or final grade?
    \item[\textbf{RQ4—Affect.}] What affective impressions do students hold of the MER visuals? 
    \item[\textbf{RQ5—Feature Feedback.}] Which features do students describe as most beneficial or limiting, and why?
\end{description}

To address these questions, we employ a pragmatist mixed-methods design \cite{shannon2016making} using structured and open-ended survey data collected across the term. Quantitative scales assess students’ perceptions of clarity, cognitive load, and usability, while open-ended responses are analyzed descriptively to capture affective reactions and feedback on specific features. We also examine how factors--such as language background, prior programming experience, and final grade--relate to these perceptions. This approach emphasizes practical insight into student experiences, using established instruments and descriptive summaries to inform design and instruction.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Noting: not writing contributions yet because it seems to just become the list of RQs.
% \smallskip\noindent\textbf{Contributions.}  
% This work  
% \begin{enumerate}[label=\arabic*)]
%     \item presents the first large-scale classroom evaluation of an \emph{abstraction-oriented} MER tool for CS2 data-structure topics,  
%     \item characterizes students’ reported clarity, helpfulness, mental effort, and perceived usability of the system,  
%     \item distils design guidelines for balancing detail and abstraction in future novice-oriented visualizations.  
% \end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The remainder of the paper reviews related work (Section~\ref{sec:related}), details our method (Section~\ref{sec:method}), reports results (Section~\ref{sec:results}), and discusses implications for pedagogy and tool design (Section~\ref{sec:discussion}).


==> wordgraves-old-dont-read/version0/02related-recent.tex <==
 \section{Related Work}
\label{sec:related}
In this section, we first examine \textbf{mental models} to explain why novices might need to coordinate multiple layers of understanding, yet struggle to do so. Second, we draw on CS2-specific evidence to show where and why novice mental models collapse as students understand \textbf{recursion and memory models}. Third, using cognitive load theory and Ainsworth's \emph{Design-Functions-Tasks} (DeFT) framework, we argue that multiple external representations (MERs) offer a solution to these challenges by \textbf{scaffolding connections} across abstraction layers which novices might struggle with. Finally, we describe existing program visualization tools, highlighting their emphasis on execution detail and setting the stage for the tri-pane, MER-driven approach introduced in Section~\ref{sec:method}.

\subsection{Layered Mental Models}
Understanding programs requires more than knowing syntax. Program comprehension research emphasizes that effective understanding depends on layered, goal-directed mental models that link concrete execution details with abstract program goals \cite{brooks1978using, canas2001role}.

\citet{heinonen2023synthesizing} identify three such models: \emph{program models} (how code works), \emph{concept models} (how ideas like recursion behave), and \emph{task/solution models} (how to solve problems). Schema-based theories describe comprehension as activating structured mental ``templates'' that help organize and interpret new information \cite{detienne1990program, detienne2002understanding, balijepally2012effect, romero2001focal}. Crucially, problem solving requires shifting between abstraction levels---connecting low-level operations like \textit{variable updates} to broader \textit{design intentions} and \textit{data structure roles }\cite{yates2020characterizing, levy2019understanding, sillito2008asking}. Experts make these shifts fluidly, but novices often rely on surface features, leading to misconceptions about scope, mutation, and aliasing \cite{chi2005commonsense, fisler2017assessing}.

Studies of developers’ information needs show how cognitively demanding this process is: even experienced programmers frequently switch between goals (``what is this function for?'') and specifics (``where does this pointer change?''), traversing semantic and syntactic layers as needed \cite{von1996identification, anneliese1998program, levy2003jeliot, fleming2008refining, letovsky1987cognitive, von1993code, von1994comprehension, bratthall2001program, von1997program}. These shifts impose cognitive load, especially in the absence of visual or spatial scaffolds. For novices, this often results in fragmented mental models that collapse during debugging or reasoning tasks \cite{mazumder2024correctness}.

\subsection{Challenges in CS2}
Transitioning from CS1, where students typically trace small programs line-by-line, CS2 introduces recursion, reference-based structures, and complex state changes that demand more abstract reasoning \cite{almadhoun2021exploratory}. Yet, assessments often emphasize code tracing and writing over structural abstraction \cite{simon2010making}, creating a cognitive bottleneck: \textbf{students must reason structurally but are trained procedurally}.

In a study by \citet{zingaro2018identifying}, 67\% of students could add a node to a linked list tail, but fewer than half could implement balanced BST insertion, suggesting brittle mental models tied to memorized procedures rather than conceptual understanding. Qualitative data further reveal breakdowns: students' struggle to simulate recursion, track pointers, and align control flow with memory \cite{almadhoun2021exploratory, feijoo2021effects}. Eye-tracking studies have demonstrated that students often ignore visualizations in favor of textual cues, exacerbating confusion \cite{bansal2021eye, mtaho2024difficulties}. Binary trees, in particular, overwhelm students due to their recursive structure \cite{feijoo2021effects}.

Large-scale surveys reinforce that the issue lies less in abstract concepts than in their implementation: students report confusion around references, lack of visual support, and poor metaphors \cite{layman2025topic, layman2020toward}. Without tools that clearly link behavior to structure, misconceptions persist into upper-year courses \cite{fisler2017assessing, chi2005commonsense}.

\subsection{Scaffolding with MER}
Multiple external representations (MERs) can bridge the gap between execution detail and structural abstraction. Ainsworth’s DeFT framework identifies three key functions---complementarity, constraint, and construction---that foster understanding across representations \cite{ainsworth2006deft}. MERs also align with cognitive load theory, helping reduce extraneous load while enhancing germane load \cite{paas2014cognitive, heer2012interactive}.

In CS2, MERs may link block-based views to full code or connect memory diagrams to abstract goals. Tools that align structural representations with execution flow improve reasoning about recursion and suppress syntax overload \cite{feijoo2021effects}. Goal-oriented modeling can foreground design rationale and clarify conceptual distinctions \cite{franch2021goal}.

However, few existing tools support a fading approach that gradually transfers responsibility to learners. While tools like Python Tutor \cite{guo2013online}, jGRASP \cite{miller2017jgrasp, cross2004jgrasp}, JaguarCode, JHAVE, and VisuAlgo \cite{naps2000jhave, halim2015visualgo, shaffer2010algorithm} target different aspects of understanding, they primarily expose stack/heap states or animate algorithm steps. Critically, they rely on a single representation and emphasize execution detail over structural inference \cite{sorva2013review}.

This emphasis can reinforce surface-level reasoning. Novices may focus on loops or control flow without grasping structural roles \cite{eckert2022loops, karnalim2017effectiveness, karnalim2017use}, and even interactive features like stepping or zooming rarely support higher-level inference \cite{de2017attention}. As a result, students often fall back on memorized behaviors without building durable conceptual models \cite{devathasan2022abstraction, rubio2015closing}.

To address these limitations, we developed a synchronized, theory-informed visualization system that supports structural abstraction through multiple coordinated views. Our MER prototypes, guided by DeFT principles, align CS2 data structures across abstraction layers to bridge low-level operations with structural transformations (see Section~\ref{method}). The next section outlines our implementation and study design.





==> wordgraves-old-dont-read/version0/02related.tex <==
\section{Related Work}
\label{sec:related}
We position our work on abstraction-oriented, multi-representation visualizations in CS2 data structures with four key subsections of literature. First, we synthesize work on mental models to argue why novices may need to coordinate multiple layers of understanding when learning to do so, but often find it challenging to do so. Next, we use CS2 specific evidence to demonstrate where, how, and why students' mental models collapse when memory references and recursion enter the picture. Third, drawing on the cognitive load theory and Ainsworth's \emph{Design-Functions-Tasks} (DeFT) framework, we argue that well-designed \emph{multiple-external-representations} (MERs) can bridge the gap between memory-level detail and structural abstraction, supporting students' in linking layers of understanding. Fourth, we discuss existing program-visualization tools in this space, noting their emphasis on fine-grained execution detail, and show how our MER-driven tri-pane design broadens that focus to support higher-level inference.


\subsection{Mental Models: Layered But Fragile}
Understanding code requires more than just following syntax--it involves coordinating multiple layers of reasoning. Program comprehension research argue that effective understanding depends on building layered, goal-directed mental models that help learners move between concrete execution details and abstract program goals \cite{brooks1978using, canas2001role}. In their review of over 150 studies, \citet{heinonen2023synthesizing} identify three key types of mental models: \emph{program models} (how code works), \emph{concept models} (how ideas like recursion behave), and \emph{task/solution models} (how to solve problems). These models evolve through processes like hypothesis testing and the recognition of familiar patterns—skills that experts use fluently but novices struggle to apply.

Schema-based theories describe comprehension as activating structured knowledge in memory—mental ``templates'' that help organize and interpret new information \cite{detienne1990program, detienne2002understanding, balijepally2012effect, romero2001focal}. Crucially, effective problem solving requires shifting between abstraction levels: learners need to connect low-level actions like variable updates to broader design intentions and data structure roles \cite{yates2020characterizing, levy2019understanding, sillito2008asking}. While experts navigate these shifts with ease, novices often fall back on surface features—leading to persistent misconceptions about scope, mutation, and aliasing \cite{chi2005commonsense, fisler2017assessing}.

Studies of developers’ information needs show just how demanding this process can be. Even experienced programmers frequently jump between goals (``what is this function for?'') and specifics (``where does this pointer change?''), traversing semantic and syntactic layers of a program as needed \cite{von1996identification, anneliese1998program, levy2003jeliot, fleming2008refining, letovsky1987cognitive, von1993code, von1994comprehension, bratthall2001program, von1997program}. These shifts impose cognitive load, especially when visual or spatial scaffolds are lacking. For novices, this often leads to fragmented mental models that break down during debugging or reasoning tasks \cite{seel2006mental}.

\subsection{When Mental Models Break Down in CS2}
Second-semester computing courses place new demands on students’ mental models by introducing recursion, reference-based structures, and complex state changes \cite{almadhoun2021exploratory}. However, assessment practices often remain fixated on low-level tracing and code writing, with few opportunities for abstraction-oriented reasoning \cite{simon2010making}. This mismatch creates a cognitive bottleneck: students are expected to reason structurally but are only trained and evaluated procedurally.

Performance data reinforce this concern. In a multi-institutional study, only 67\% of students could correctly add a node to the tail of a linked list, and fewer than half could design a balanced binary search tree insertion sequence \cite{zingaro2018identifying}. These results suggest that many students rely on memorized procedures—like blindly looping to the end of a list—even when shortcuts (e.g., tail pointers) exist, revealing gaps in their ability to connect low-level code with high-level data structure goals.

Qualitative and cognitive studies further highlight these disconnects. Students struggle to mentally simulate recursive behavior, track pointer mutations, and map control flow onto evolving memory structures \cite{almadhoun2021exploratory, feijoo2021effects}. Eye-tracking and self-report studies show that students often default to familiar textual cues, even when visualizations are available, leading to shallow engagement and increased confusion \cite{bansal2021eye, mtaho2024difficulties}. Binary trees, in particular, overwhelm working memory due to their nested and self-referential structure \cite{feijoo2021effects}.

Recent large-scale surveys confirm that these challenges are less about conceptual recognition and more about implementation bottlenecks \cite{layman2025topic}. Students cite difficulty managing references, poor visualization support, and a lack of intuitive metaphors—all of which impede their ability to integrate layers of meaning across code, structure, and behavior \cite{layman2020toward}.

These challenges call for stronger scaffolding—not just in instruction and assessment, but also in the representational tools available to learners. Without explicit support for linking concrete behavior to structural intention, students' mental models remain shallow, fragmented, and vulnerable to overload.

\subsection{Multiple Representations: Scaffolding Abstraction Through Design}
To help students bridge the gap between low-level execution and high-level structure, the learning sciences advocate for multiple external representations (MERs) that work in tandem to support understanding. According to Ainsworth’s \textit{Design–Functions–Tasks} (DeFT) framework, MERs are most effective when they serve to complement different aspects of a concept, constrain misinterpretation, and construct new knowledge by linking representations through active reasoning \citep{ainsworth2006deft}. These functions align with broader cognitive principles: MERs reduce extraneous load by offloading memory demands and improve germane load by scaffolding abstraction \citep{paas2014cognitive, heer2012interactive}.

Well-designed MERs also help learners move from concrete traces toward generalized understanding—a process supported by concreteness fading and representational transformation \citep{fyfe2014concreteness}. In CS2 contexts, this can mean fading from visual block-based tools into full code, or progressively linking memory diagrams with abstract structural goals. For example, block-based environments that align code with structural views improve students’ reasoning about recursive tree operations while shielding them from syntactic noise \citep{feijoo2021effects}. Similarly, goal-oriented modeling tools foreground \textit{why} a structure satisfies certain design requirements, making abstract distinctions more perceptible \citep{franch2021goal}.

Yet, not all visualizations support these cognitive goals. Highly detailed line-by-line traces—like those in Python Tutor—often lack abstraction cues, leading students to revert to familiar textual views or memorize steps without internalizing structure \citep{bansal2021eye, sorva2013review}. Without synchronized layers that tie code, memory, and conceptual views together, learners may fail to generalize, despite engaging with visual tools.

To be effective in CS2, MER designs must therefore do more than display data: they must synchronize layers, highlight conceptual roles, and manage cognitive load. Despite strong evidence supporting these principles, such integrated approaches remain uncommon in existing tools. Our work takes up this challenge by explicitly designing MER-driven visualizations that prioritize abstraction, not just traceability.

\subsection{Existing Tools}
Many programming visualizations promise to ``show what the computer sees.'' Tools like Python Tutor \citep{guo2013online}, jGRASP \citep{miller2017jgrasp, cross2004jgrasp}, and JaguarCode expose stack and heap frames, while JHAVE and VisuAlgo animate standard algorithms \citep{naps2000jhave, halim2015visualgo, shaffer2010algorithm}. However, most rely on a single representation and emphasize low-level mechanics—highlighting how code executes without clarifying why it behaves that way \citep{sorva2013review, card1999readings, munzner2014visualization, ware2012information, heer2012interactive}.

This emphasis on granular detail can hinder learning. Novices often fixate on line-by-line traces, reinforcing surface-level misconceptions about loops and control flow \citep{eckert2022loops, karnalim2017effectiveness, karnalim2017use}. Even when tools support interactivity—such as stepping through code or zooming into memory—they rarely help students form broader inferences or link behavior to structural intent \citep{de2017attention}. Without explicit scaffolding, students may memorize what the code does, but struggle to generalize or reason conceptually \citep{devathasan2022abstraction, rubio2015closing}.

Meta-reviews in computing education consistently point to this gap. Existing tools tend to prefer detail over inference and often fail to support the notional machines that students need to build robust mental models of program behavior \citep{sorva2013review}.

\subsection{Positioning and Contribution.}
We identify a core disconnect in CS2 instruction: students are expected to reason across abstraction layers, but both teaching practices and visualization tools often fail to support that process. Mental models remain fragile, especially when recursion and references are introduced. Learners struggle to coordinate code behavior with structural goals, and existing visualizations—while abundant—tend to emphasize detail without scaffolding inference.

We address this gap through a theory-driven visualization design grounded in principles of multiple external representations (MERs), drawing on Ainsworth’s DeFT framework to support coordination across layers of understanding \citep{ainsworth2006deft}. Our tri-pane interface synchronizes source code, memory diagrams, and a progressively abstracted structural view, aiming to reduce extraneous load and foster expert-like hypothesis cycling \citep{brooks1978using, heinonen2023synthesizing}. We evaluate this design at scale in a 12-week CS2 course with 440 students, providing new evidence that well-aligned MERs can help learners connect layers of meaning and improve perceived clarity during complex data structure tasks.

==> wordgraves-old-dont-read/version0/04results.tex <==
\section{Results}
\label{sec:results}
In this section, we report our mixed-methods findings for each of our three research questions. We begin with \textbf{RQ1}, which examines how students experienced the multi-representation (MER) visualizations, drawing on both open-ended feedback and Likert-scale ratings of clarity and helpfulness. We then turn to \textbf{RQ2}, which assesses the usability and cognitive load associated with the visualizations. Finally, \textbf{RQ3} explores variation in these experiences across learner subgroups, including prior experience, language background, and final course grade.

\subsection{RQ1: Student Experience}
\textit{Quantitatively}, students rated the MER visualizations as significantly clearer and more helpful than neutral. On a five-point Likert scale, the composite \emph{Clarity/Helpfulness} score averaged $M=3.83$, $SD=0.74$, well above the midpoint of 3, $t(306)=19.66$, $p<.001$, Cohen’s $d=1.12$ (Table~\ref{tab:clarity}).

\input{tables/clarity}

\textit{Qualitatively}, we constructed three distinct themes in student experience: the value of layered, coordinated representations; their role in enabling structural reasoning beyond surface-level tracing; and their particular utility for recursive and pointer-based logic. 


\subsubsection{Value of Layered, Coordinated Representations}
Students emphasized how the side-by-side presentation of code, memory, and structural views aligned with how \textit{they} wanted to conceptualize data structures. Rather than passively following execution, students described active sensemaking across representations:
\begin{myquote2}[Survey xCpy]
``Very clear flow/top down structure. Actually follows the theoretical structure of the adt from How a human would perceive it compared to that of the original which is closely aligned to how python perceives it ''
\end{myquote2}
Here the student expresses a desire to see a simple representation that a human might make when looking at code, as opposed to lower-level representations that a view of memory might offer. 
This quote also reflects Ainsworth’s DeFT principle of \textit{constraining interpretation}: the visual layout serves not merely to illustrate code behavior but to nudge learners toward expert-like, goal-oriented reasoning. By visually separating control flow from structural outcome and memory reference, the MER interface helps learners build layered mental models that connect syntactic steps with semantic intent \citep{heinonen2023synthesizing, brooks1978using}.

A student also appreciated being able to see ``the bigger picture'' hinting at the benefits of using multiple-representations in mapping low-level details of the code to bigger conceptual links.
\begin{myquote2}[Survey 5KxQ]
``I liked the full diagram/image visualizations, since they made it easier to see what was fully happening in the bigger picture, and made it easier for my mind to visualize the code.''
\end{myquote2}

\subsubsection{Supporting Structural Reasoning}
A central benefit of the MER visualizations was their ability to shift students’ focus from line-by-line execution to the structural properties and transformations of data types. Rather than merely tracing changes in variable values, students described using the coordinated diagrams to infer \textit{why} a structure behaved as it did—aligning with our focus on \textit{structural abstraction}. This involved reasoning about overall shape, recursive patterns, and high-level goals, such as maintaining tree invariants or visualizing pointer-linked relationships.


\begin{myquote2}[Survey LYXV]
``The visualization for each data type is very useful for me to directly understand the structure of each data type. The highlight in text, memory and data type structures makes the code easier to follow.''
\end{myquote2}

This comment exemplifies how the system supported synthesis across representational layers: the student links code highlighting to both memory layout and structural configuration. Others noted how visualizations enabled them to internalize recursive structures or complex data shapes:

\begin{myquote2}[Survey LQ6B]
``The visual layout and diagrams at use that helps give a visual to each data structure making it far easier to consume the information and code that uses more complex data structures likes trees/linked-lists.''
\end{myquote2}

\begin{myquote2}[Survey ZpvY]
``Similiar with python tutor, it also gives me a clearer understanding of implementation of abstract data types. Instead of having tables of variables, the visualization helps to understand complex data structures like Trees easier.''
\end{myquote2}

These responses underscore a shift from operational to structural understanding—a hallmark of expert reasoning, but often elusive for novices without visual scaffolds \citep{detienne2002understanding, zingaro2018identifying}. The MER interface appears to help bridge this gap by making abstract, recursive, and hierarchical relationships directly perceptible.

Another student  emphasized that the ability to see a structure in its canonical, semantic form alongside the program helped them see what the program was doing overall:

\begin{myquote2}[Survey C09A]
``I like how they displayed Trees in a proper tree format instead of just messy memory diagrams; helps paint  better picture of what the program is doing.''
\end{myquote2}

This response illustrates how semantic alignment in the visualizations supports conceptual abstraction: instead of focusing on pointer addresses or memory slots, students could reason about structural properties like parent-child relationships, recursive composition, and invariants. Such alignment enables learners to move beyond operational detail toward expert-like mental models, as emphasized in program comprehension research \citep{detienne2002understanding, yates2020characterizing}. We note that this also connects to the earlier quote on appreciating the ``bigger picture'' through multiple representations: students were not only able to see high-level structure more clearly, but also trace how individual code lines and memory operations contributed to those larger patterns. This dual support--of both local mechanics and global organization--is a defining affordance of well-coordinated MERs.

\subsubsection{Support for Recursive and Reference-Based Reasoning}
MERs were particularly impactful when students encountered recursion and reference-based data structures—topics known to challenge mental models due to their layered, state-dependent nature. Several students articulated how visualizations helped make recursive control flow more tractable:

\begin{myquote2}[Survey BMee]
``In recursion I often don't know how to ensure that the next one will be successful, but if I visualize a small process I can figure out the completed recursion like doing a puzzle.''
\end{myquote2}

\begin{myquote2}[Survey fOb7]
``It was beneficial to see how the code was actually processing the abstract nature of certain things like recursion.''
\end{myquote2}

\begin{myquote2}[Survey BMee]
``I was using these visualizations to understand how recursion works for some simple algorithms like BST, inorder/postorder traversal''
\end{myquote2}
This comment reinforces the importance of visual scaffolding in recursive contexts \citep{feijoo2021effects, almadhoun2021exploratory}, especially for making abstract control flow concrete and sequentially interpretable.

In addition to recursion, students described using the memory diagrams to reason about object creation, deletion, and referencing -- key challenges in understanding reference=based data structures such as linked lists and trees:
\begin{myquote2}[Survey nLh4]
``I appreciated the memory models the most. It helped me see how exactly the objects were created, deleted, and referenced.''
\end{myquote2}
This reflection suggests an emerging understanding of reference semantics — a core source of misconception in upper years too \citep{fisler2017assessing}. The ability to visualize memory operations alongside structural outcomes appears to support a more integrated mental model of how data structures evolve over time.

\subsubsection{Desired Extensions}
In addition to usability and load-related concerns (discussed in RQ2), several students highlighted limitations in the scope and flexibility of the visualizations. A few students felt that while the diagrams helped with structural understanding, they sometimes glossed over important conceptual nuances, such as the distinction between mutable and immutable objects, or between primary and secondary computational ideas:

\begin{myquote2}[Survey IbHo]
``I cannot tell the difference between mutable and immutable things from the visual still.''
\end{myquote2}

% \begin{myquote2}[Survey cSzu]
% ``We can't particularly clearly distinguish between primary and secondary ideas, and we need to use logical reasoning to deduce them.''
% \end{myquote2}

A second limitation concerned the fixed, instructor-defined nature of the visual examples. Several students wanted the ability to explore more complex or customized structures, particularly beyond the canonical tree or list examples provided:
\begin{myquote2}[Survey nooV]
``I found it somewhat limiting that there were no options for the user to create their own data structures... it would be very useful for me to create a more complex tree.''
\end{myquote2}
Lastly, a few participants critiqued the overall visual interactivity and control, expressing a desire for features such as zooming, resizing, or more fine-grained navigation:

\begin{myquote2}[Survey f65H]
``The ability to resize the visuals would be helpful as it would allow me to focus on specific areas of the visuals or choose to see the visual as a whole whenever I needed to.''
\end{myquote2}

A related comment suggested that the ability to construct diagrams--rather than only viewing pre-generated ones freely--could deepen learning through active reconstruction:
\begin{myquote2}[Survey IbHo]
``I think that something like dogma whiteboard where you can make your own diagram from scratch would be cool since that makes you practice writing them out yourself.''
\end{myquote2}
This response emphasizes not just the desire for flexibility, but the pedagogical value of generative practice: creating representations as a means of internalizing structural relationships. This relates to the idea of drawing to learn in science \cite{ainsworth2011drawing}, which can help students discern key features and challenges of new tasks \cite{schwartz2004inventing}.

While these comments reflect a minority of the dataset, they underscore important directions for future work: namely, the need for more flexible, user-driven, and semantically expressive visualizations that support both conceptual fidelity and learner agency. 

\subsection{RQ2: Usability and Cognitive Load}
We next examined the cognitive and usability demands of the MER visualization system, focusing on mental effort, navigation experience, and perceived usability. Quantitative results showed that the system was broadly usable, with students reporting moderate cognitive effort. Open-ended feedback provided more detail about when and why effort increased.

Students reported moderate levels of mental effort while using the MER visualizations ($M = 3.03$, $SD = 0.72$, on a reversed five-point scale where higher scores reflect \emph{lower} effort). While these ratings do not indicate a strong reduction in perceived cognitive load, they suggest that the interface did not overwhelm students despite the abstract content. A longitudinal comparison revealed a significant reduction in reported effort from CS1 to CS2 ($W = 2{,}191$, $p < .001$), hinting at improved cognitive efficiency over time.

Qualitatively, we constructed three themes that deepen our understanding of students’ cognitive and usability experiences: (1) the distinction between productive effort and representational overload; (2) affective responses linked to intuition, confidence, and conceptual ``click'' moments; and (3) individual variation in how learners strategically navigated multiple representations. 

\subsubsection{Effort as Productive vs. Overwhelming}
Several students described needing time to interpret complex transitions or cross-reference across views, especially when structural changes were dense:

\begin{myquote2}[Survey Slih]
``Steps that changed a lot required me to sit and stare for a while to understand how it went from the previous to the next.''
\end{myquote2}

This comment highlights a specific kind of cognitive load associated with visual discontinuity--where learners must focus on following the visuals carefully across non-trivial state changes. Another student expressed a related challenge when multiple panes changed simultaneously:

\begin{myquote2}[Survey WYQF]
``Since there were 3 screens to keep track of simultaneously, it was confusing and cumbersome to understand.''
\end{myquote2}

Together, these responses suggest that while MERs can support integration, they may also introduce temporal coordination costs—especially when multiple representations shift in rapid succession or diverge visually. Our design intentionally foregrounded larger, structural transformations, aiming to push learners beyond the more granular, line-by-line tracing typical of CS1. However, the responses indicate that this shift was not uniformly accessible: some students struggled to infer intermediate steps or align changes across panes. This highlights the continued need for transitional scaffolding—such as pacing controls, visual annotations, or intermediate state cues—to help learners bridge the gap between operational and structural reasoning while mitigating cognitive overload.


\subsubsection{Affective Experience and the ``Click'' of Understanding}
Students frequently used affectively charged or metaphorical language to describe their learning experience. Several mentioned moments where visualizations helped make abstract logic ``click,'' reducing confusion and making the examples more \textit{interesting}:

\begin{myquote2}[Survey 2Wad]
``Being able to visualize code helped me learn about them in a more intuitive manner. It speeds up the time it takes to have that click in my head.''
\end{myquote2}

\begin{myquote2}[Survey ytBu]
``The interactive design and visual clarity made it more interesting to work through examples. It felt like I was `watching the code think'.''
\end{myquote2}

These affective responses align with research on cognitive-affective engagement, which suggests that intuitive, semantically meaningful representations can foster deeper conceptual integration and motivation to persist when doing tasks \cite{pekrun2006control}.

\subsubsection{Representation Fit and Strategic Learning Preferences}
Student responses revealed a wide variation in how learners approached the multiple--representation system--both in terms of preference and strategic sequencing. Some students preferred to begin with a single, familiar representation to build confidence and conceptual grounding before layering on others. This often reflected a concern about cognitive overload or representational inconsistency:

\begin{myquote2}[f65H]
``I prefer starting by using a single representation and working through it until I understand the best I can... Only after this will I reach for other representations to supplement and verify my understanding.''
\end{myquote2}

Others embraced variety from the outset, describing how different views highlighted different facets of a concept and helped them triangulate understanding. For these students, diversity of representation was not a distraction but a way to reinforce understanding through multiple entry points:

\begin{myquote2}[Survey nooV]
``I prefer using multiple visual representations over a single representation since I like to first figure out which representation best helps me understand any concept... Seeing multiple representations also helps me better understand the concepts.''
\end{myquote2}

Students also reflected critically on the strengths and limitations of specific views. Some found memory models essential for understanding low-level storage, while others prioritized structural diagrams or metaphorical animations for grasping high-level logic:

\begin{myquote2}[Survey ytBu]
``Code flow diagrams show the sequence of operations, while memory maps help visualize how data is stored... metaphorical animations can bring abstract ideas to life by connecting them to something tangible.''
\end{myquote2}

These comments highlight a broader epistemic point: learners did not merely consume representations--they used them as tools in a self-directed process of making sense of abstraction. However, this flexibility also introduces risks: several students noted that too many representations, or poorly aligned ones, could lead to confusion, especially early in the learning process. These findings suggest that, while multiple representations are valued, they must be curated, aligned, and scaffolded to match the readiness of the student and the conceptual focus.

\subsubsection{Feature-Specific Reflections and Design Trade-offs}
To better understand how particular design features shaped students’ experiences, we examined recurring references to interface elements across both RQ1 (experience) and RQ2 (usability and load). Table~\ref{tab:features_summary} summarizes the most commonly cited features, highlighting both perceived benefits and limitations.

\input{tables/features}

Students broadly appreciated features that scaffolded interpretive control, such as step-by-step pacing, color-based highlights, and tri-pane coordination. These elements supported cognitive clarity, especially in recursive or structurally complex examples. The ability to slow down and replay transitions was particularly valuable for fostering what some described as “click” moments of understanding.

However, nearly all of these affordances also carried trade-offs. The tri-pane layout, while enabling layered mental modeling, could be visually dense or cumbersome on smaller screens. Color and highlighting, though helpful for focusing attention, were sometimes judged insufficient without more explicit labels or annotations. Step-by-step pacing, though clarifying for many, occasionally felt slow or overly rigid, especially for more advanced learners or during review.

Perhaps most notably, students pointed to a desire for deeper interactivity—highlighting limitations in the ability to edit code, create custom structures, or explore beyond instructor-defined examples. While visual clarity and sequencing were generally strong, learner agency and semantic flexibility emerged as growth areas for future refinement.

These findings reflect broader design tensions in educational interfaces: the same feature that enhances clarity for one learner may constrain agency for another. Future iterations should prioritize adaptability—both in representational configuration and in the affordance of learner-driven exploration—to meet the diverse epistemic strategies students bring to complex content.

\subsection{RQ3: Subgroup Analysis}
Non-native English speakers rated the MER visualizations significantly clearer ($M=4.07$) than native speakers ($M=3.86$), Welch’s $t(129.4) = -2.32$, $p = .022$, $d = 0.28$, indicating a small but meaningful difference. No significant differences emerged in perceived cognitive load or ease of use. This suggests that the visual format may have been especially supportive for students navigating a second language, consistent with prior work showing the value of visual scaffolds in reducing linguistic barriers.

\paragraph{Prior programming experience.}
Students with no prior experience reported similar clarity ($M=3.97$) to their peers with experience ($M=3.89$), with no significant differences on any of the three scales ($p > .05$). This suggests that the MER system was accessible regardless of prior programming exposure.

\paragraph{Final course grade.}
To explore whether overall course performance influenced student perceptions, we compared clarity/helpfulness scores by final grade band (A, B, C or lower). No significant differences were observed, indicating that students across performance levels found the visualizations similarly helpful.

\paragraph{Gender.}
Although not a focal variable for RQ3, we include gender comparisons for completeness. No significant differences were found across any measure (ANOVA $F = 0.08$–$0.05$, $p > .75$).

\input{tables/subgroups}



%%%%%%%%%%%%%%%%%%%
% Other Quotes
%%%%%%%%%%%%%%%%%%%

% it allows me to actually visualize how the data structure looks like which would allow me to write implementations for that specific data structure.


% I think that these visualizations could be improved by incorporating user-defined data structures. Rather than seeing the same visualization being applied to only one tree, it would be much more useful if I could also create my own trees and see the visualization run on those.

% Multiple visual representations aids in understanding the concepts from various aspects like memory vs code flow vs the visual data structure. It provides for a more well-rounded understanding of the concept.

% The visual breakdown of code execution and tree structures made it easier to understand how algorithms like Huffman encoding work step by step.

% The multiple-representation visuals provided a more holistic view by showing code, variables, and diagrams together, which made it easier to connect concepts.




==> wordgraves-old-dont-read/version0/05discussion.tex <==
\section{Discussion}
\label{sec:discussion}

This study examined how students experienced a novel tri-pane, multi-representation (MER) visualization system in a CS2 course, focusing on clarity, usability, cognitive load, and learner subgroups. In this section, we integrate findings from our quantitative and qualitative analyses to reflect on the implications for visualization design, abstraction scaffolding, and inclusive computing education.

\subsection{MER Support for Structural Abstraction}
Our findings suggest that students broadly perceived the MER visualizations as clear and helpful, supporting H1. This aligns with prior work showing that layered visual representations can facilitate reasoning about recursive structures and memory references when they align with students’ mental models~\cite{brooks1978using, detienne2002understanding, heinonen2023synthesizing}. Students in our study often described the interface as ``easy to follow,'' ``simple,'' or ``intuitive,'' and praised its use of color, highlighting, and step-by-step execution. These feature-level appreciations reflect Ainsworth’s \emph{Design–Functions–Tasks} (DeFT) framework~\cite{ainsworth1999functions}, which emphasizes that representational choices must support specific cognitive tasks—in this case, tracking aliasing, mutation, and structural transformations across dynamic code execution.

Importantly, students highlighted how multiple representations (e.g., stack frames, pointer graphs, and abstract trees) helped reinforce conceptual understanding. These comments reinforce the argument that MERs can help learners coordinate distinct mental models by making visible both low-level operational details and higher-level structural outcomes.

\subsection{Managing Complexity Without Overload}
% massive rewording needed
Students reported moderate levels of cognitive load, with no strong skew toward either extreme of the scale. In the absence of a meaningful benchmark or baseline for comparison, we interpret these scores descriptively rather than inferentially. Qualitative feedback further supports this interpretation: while many students described the visualizations as helpful and well-paced, some acknowledged that they still required effort to interpret—especially in complex or cluttered scenarios.

These findings align with perspectives that emphasize the productive role of cognitive effort in learning~\cite{paas1992, layman2020toward}. As one student explained, the tool made learning ``easier'' but not effortless—it provided ``support,'' not simplification. Interactive elements, such as step-by-step control and visual alignment, appeared to help students manage abstraction without feeling overwhelmed. At the same time, comments about visual clutter, rapid state changes, or lack of explanation remind us that cognitive support must be carefully designed to avoid introducing extraneous load~\cite{mayer2008increased}.

At the same time, a subset of students reported feelings of overload, visual clutter, or a lack of visual depth. These critiques caution that cognitive benefits are not uniformly distributed and that MERs must be carefully designed to avoid introducing extraneous processing~\cite{mayer2008increased}. Students cited moments where the layout felt ``clogged,'' where transitions between steps were hard to follow, or where the visual structure lacked alignment with expected metaphors. Such feedback underscores the importance of iterative design and empirical validation of cognitive fit.

\subsection{Usability and Interface Interaction}
Students rated the system as usable (supporting H3), with scores significantly above the neutral benchmark. Qualitative data further highlighted that interactivity--through buttons, step control, and replayability--played a crucial role in student engagement. This echoes findings from visualization and educational tool research that learners benefit not just from passively viewing animations, but from actively navigating representations~\cite{guo2013online, burkhardt2020learned}. Still, several students noted friction around limited IDE interaction or difficult-to-trace transitions. These concerns suggest that usability is not just a matter of interface polish, but of design affordances that match learners’ mental goals.

\subsection{Toward More Inclusive Visual Tools}
RQ3 examined how learner characteristics shaped perceptions. While no differences emerged by gender or prior programming experience, we observed that non-native English speakers rated the visuals as significantly clearer than native speakers, supporting H4. This finding complements prior work suggesting that visual explanations can reduce linguistic barriers in computing contexts~\cite{guo2018non, lee2023clue}. Students also commented on how the visual modality reduced intimidation and enabled them to re-engage with complex material at their own pace. Taken together, these findings suggest that MER-based systems may not only support abstraction, but promote equity in how that abstraction is accessed and experienced.

\subsection{Design Implications and Future Directions}
\label{sec:design-implications}

Our findings point to several design principles for visualization systems in abstraction-heavy CS contexts, grounded in the experiences reported by students across the study.

\begin{itemize}
    \item \textbf{Layered Representations Support Conceptual Alignment.} 
    Students frequently praised the alignment between source code, memory diagrams, and abstract structure, with qualitative feedback emphasizing how the tri-pane layout helped them ``connect what the code is doing to what the structure becomes.'' This supports MER theory and suggests that visual tools should not isolate concrete and abstract layers, but instead coordinate them spatially and temporally.

    \item \textbf{Cognitive Load Can Be Managed Through Pacing and Framing.} 
    Although cognitive load scores were moderate (not low), students described feeling supported rather than overwhelmed. Many referenced the ``step-by-step'' nature of the interface and the ability to ``go back'' or ``replay'' execution. This suggests that interactivity and granularity can help manage intrinsic load, even when the content remains complex. Importantly, some reports of overload were tied to rapid state changes and dense layout—pointing to the need for more deliberate pacing and state anchoring in complex diagrams.

    \item \textbf{Visual Clarity Depends on Layout, Not Just Representation.} 
    While most students rated the visuals as clear, those who described confusion often cited layout issues rather than representational choices. For instance, several students mentioned that ``everything felt too close together,'' or that changes between steps were ``easy to miss.'' This suggests that even with appropriate representational mappings, diagram design must carefully balance visual density, white space, and alignment to avoid perceptual overload.

    \item \textbf{Inclusive Design Benefits From Reduced Verbal Reliance.} 
    Non-native English speakers rated the visualizations significantly clearer than native speakers, and students described being able to ``understand the structure without needing to read too much.'' This points to the potential of visual explanations to reduce language-based barriers, reinforcing prior work on the accessibility of multimodal instruction. Visual scaffolding should be prioritized not just for clarity, but for equity.

    \item \textbf{Feature Interactivity Shapes Engagement and Re-engagement.} 
    Students repeatedly cited control over the visualization—especially step-by-step navigation—as key to their engagement. Some noted that they ``used the tool to check [their] own reasoning'' or ``went back to earlier steps to figure out what changed.'' These comments suggest that interaction is not simply a usability feature, but a pedagogical mechanism for reflection and error recovery.
\end{itemize}

Future work should examine how these principles transfer to other contexts (e.g., CS1, data structures-heavy algorithms courses), and whether learners benefit from features like toggling representations, reordering panes, or integrating scaffolding prompts. Triangulating student perception data with behavioral traces (e.g., eye tracking or clickstream) may further clarify how learners engage with multiple representations—and where cognitive alignment breaks down.


==> wordgraves-old-dont-read/version0/05results1-eye.tex <==
\subsection{Gaze in Multi-Representation Tools}
To complement the interview analysis, we examined gaze traces to characterize how learners visually engaged with the MER tool. Figure~\ref{fig:gaze-distribution} reports fixation distributions across areas of interest (AOIs). Across participants, the largest share of fixations fell on the \textbf{Code} pane, reflecting its role as a reference point for reasoning. Attention was also distributed across \textbf{Memory} and \textbf{Visual/Output}, indicating that learners engaged with multiple representational layers rather than focusing on code alone.


\paragraph{Task-level patterns.}
Fixation distributions varied by topic. In \textbf{Linked List} tasks, median dwell time was balanced across Code (38.8\%) and Memory (46.8\%), with Visual playing a modest role (12.5\%). In \textbf{Scope} tasks, learners devoted more attention to Code (49.6\%) than Memory (41.0\%), with Visual receiving the least attention (10.4\%). By contrast, \textbf{While loop} tasks showed relatively lower Code focus (36.2\%), and a higher proportion on Visual (19.2\%), suggesting that learners looked more often to dynamic output when reasoning about iteration.


\paragraph{Transitions across panes.}
Transition analyses indicated frequent cross-pane movement (Figure~\ref{fig:gaze-transitions}). Counts here represent the total number of transitions aggregated across all participants. The most common were \textit{Memory $\rightarrow$ Code} (11,456 transitions) and \textit{Code $\rightarrow$ Memory} (11,454), showing a strong oscillation between these panes. Visual played a secondary but consistent role, especially in loops such as \textit{Memory $\rightarrow$ Visual $\rightarrow$ Memory} (4,842) and \textit{Visual $\rightarrow$ Memory $\rightarrow$ Visual} (2,562).


\paragraph{Sequence entry points.}
Sequence analyses report how many participants exhibited particular fixation patterns. The most common first fixation was on the Memory pane (12 participants), followed by Code (2) and Visual (2). Subsequent cycles typically centered on \textit{Code $\leftrightarrow$ Memory}, with occasional inclusion of the Visual pane. These cycles are consistent with interview accounts of learners ``checking execution against expectation,'' with code serving as an anchor and memory as validation.

Overall, the gaze data suggest that learners treated code as primary, but MER’s tri-pane layout afforded regular integration of memory and visual output. These results provide a complementary perspective to the qualitative accounts, highlighting how interface design can structure not only where learners look, but also how they shift attention across representational layers.



\begin{figure}[t]
  \centering
  % First subfigure: gaze distribution
  \begin{subfigure}[t]{0.35\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/gaze_distributions.png}
    \caption{Distribution of gaze fixations across AOIs in MER.}
    \label{fig:gaze-distribution}
  \end{subfigure}
  \hfill
  % Second subfigure: cohort dot plot
  \begin{subfigure}[t]{0.6\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/cohort.png}
    \caption{Cohort-level distribution of fixation patterns.}
    \label{fig:cohort}
  \end{subfigure}
  %
  \caption{Gaze fixations (left) and cohort-level distributions (right).}
  \label{fig:gaze-subfigures}
\end{figure}


\begin{figure}[t]
  \centering
  \includegraphics[width=0.85\linewidth]{figures/gaze_transitions.pdf}
  \caption{Transition frequencies (bigrams/trigrams) across AOIs, showing integrative cross-pane movement in MER vs. narrower loops in Python Tutor.}
  \label{fig:gaze-transitions}
\end{figure}


==> wordgraves-old-dont-read/version0/05results2.tex <==
\section{Results}
\label{sec:results}
\input{sections/05results1-eye}

Code visualizations did not function as fixed or self-evident representations of program behavior. Their meaning and pedagogical utility emerged through students’ situated engagements, shaped by prior experiences, disciplinary positioning, and habitual ways of reasoning. What one student found useful, another might overlook, misinterpret, or actively resist, depending on how the visualization aligned with their interpretive strategies and learning goals. 

These findings resonate with research on layered mental models~\cite{heinonen2023synthesizing}, which emphasizes that program understanding depends on integrating execution-level reasoning with higher-order conceptual and structural models. Yet students did not always encounter visualizations as straightforward aids to that integration. Their uptake was shaped by moment-to-moment decisions about whether, when, and how to engage with different representations, a process contingent on epistemic stances and self-regulatory strategies.

From a learning sciences perspective, this variability aligns with Ainsworth’s DeFT framework~\cite{ainsworth2006deft}, which stresses that the effectiveness of multiple external representations (MERs) depends not only on their design, but also on the cognitive tasks learners undertake. In our study, those tasks were lived experiences of sensemaking, often, but not always, falling within the ``constructive'' mode of Chi’s ICAP framework~\cite{chi2009active}, where learning emerges through generating inferences, explanations, and mental models. The presence of a visualization did not guarantee such engagement; it was actively negotiated.

We present five interpretive themes that trace how students took up, adapted, and at times resisted visualizations.



\subsection{Epistemic Sovereignty and Strategic Visualization Use}

For many participants, code tracing was not a passive walkthrough but an assertion of epistemic sovereignty, the conviction that their own reasoning should anchor the work, with visualizations serving only as strategically timed consultants. This stance reframed the visualization from a step-by-step driver into a selectively summoned resource, useful only when it aligned with the learner’s own interpretive trajectory.

\begin{myquote2}[P1\_B]
``I like tracing things on my own because I feel like I’m more in control. When I just press ‘Next’, I don’t really know what’s happening, I’m just kind of observing. But when you trace it yourself, you really have to understand how Python is going to execute the code.''
\end{myquote2}

Here, ``control'' is not just about interface pacing; it is a statement of authority over meaning-making. P1 positions self-generated reasoning as the primary source of truth, treating the visualization as secondary and confirmatory. This logic echoed across sites:

\begin{myquote2}[P5\_B]
``The first thing I usually do is look at the code on its own, without checking the steps, just to see if I understand what's happening. And then, if I get to a spot where I’m confused, that’s when I turn to the visualization to help me figure it out.''
\end{myquote2}

From an ICAP perspective~\cite{chi2009active}, this sequencing enacts a \emph{constructive} process, generating inferences independently, then testing them against an external referent. For some, this calibration was highly explicit: \textit{``What the visualization lets me do is verify whether that initial assumption is actually correct''} (P6\_A). For others, the visualization became a high-resolution lens in debugging contexts: \textit{``If you were debugging code and wanted to really see what's happening, this MER visual would be great''} (P2\_A).

This stance creates a productive tension for visualization design. On one hand, prioritizing self-explanation can deepen understanding and encourage flexible reasoning. On the other, a strong sovereignty stance may limit exposure to alternative representations that could challenge or expand a learner’s model. In this sense, epistemic sovereignty is both a protective filter and a potential gatekeeper, shaping not just when a tool is used, but what forms of insight it is allowed to deliver.

\subsection{Representational Resonance: When Tools ``Think'' Like Learners}

Participants engaged most readily with visualizations that aligned with the representational forms they already used to reason about programs, whether spatial memory diagrams, self-drawn sketches, or everyday analogies. When a view ``spoke their language,'' it slotted directly into their workflow, requiring little cognitive translation.

\begin{myquote2}[P7\_A]
``This is exactly the kind of diagram I draw for myself during an exam.''
\end{myquote2}

Here, the tool is not introducing a new epistemic frame but validating one the learner already inhabits. This \emph{resonance}, a merging of representational form and habitual reasoning, can reduce the perceived distance between ``my way'' and ``the official way,'' potentially reinforcing learner confidence and authority.

For some, this resonance was metaphorical rather than diagrammatic:

\begin{myquote2}[P4\_B]
``Yes, I always think in analogies. Like with a while loop: we’ve all been to the supermarket looking for a specific item. In that moment, we’re basically running an algorithm in our minds.''
\end{myquote2}

In such cases, the visualization does not so much translate code into a new form as surface and legitimize analogies the learner already relies on, affirming their personal notional machine~\cite{ma_using_2008}.

Where resonance was absent, learners sometimes disengaged from a view entirely, not because it was objectively unclear, but because it spoke in a ``cognitive accent'' unfamiliar to their repertoire. This reframes clarity as relational: what is intuitive for one learner may feel opaque or cumbersome for another, depending on prior representational fluency.

For designers, representational resonance poses a tension. Aligning closely with learners’ existing strategies can boost initial uptake but risks narrowing exposure to alternative conceptual framings. Introducing a dissonant form may expand representational repertoire, but at the cost of early fluency. Balancing these dynamics is key if visualizations are to both meet learners where they are and invite them into new ways of thinking.


\subsection{The Politics of Seriousness in Visual Design}

Playful or metaphorical visuals often functioned as a representational \textit{Rorschach}: the same design choice could be experienced as either a conceptual bridge or a breach of disciplinary decorum. For some, metaphor was not a distraction but an essential scaffold into abstraction:

\begin{myquote2}[P4\_B]
``Even in a second-year systems course, they used analogies, like lockers for memory. Honestly, if it weren’t for that, I don’t think I would have grasped the concept.''
\end{myquote2}

Here, metaphor extends the learner’s conceptual reach, recasting an unfamiliar abstraction in the terms of an accessible everyday schema. The visual becomes an epistemic ally, shrinking the gap between novice and expert discourse.

Yet for others, the same style of representation provoked discomfort, not because the content was wrong, but because the form seemed to misalign with their sense of what ``serious'' university-level learning should look like:

\begin{myquote2}[P13\_A]
``As a university student using these kinds of graphics... it kind of feels like it’s for younger students. But then again, it might just be ego and personal bias.''
\end{myquote2}

This ambivalence points to a sociocultural layer in visualization design. Representations are not neutral encodings of program state, they are also signals of audience, legitimacy, and pedagogical stance. A visual style can mark the work as ``academic'' or ``childish,'' ``professional'' or ``introductory,'' depending on the viewer’s identity, experience, and perceived position in the disciplinary hierarchy.

Several participants voiced this tension within the same interview, appreciating metaphor as a conceptual aid while simultaneously distancing themselves from its aesthetic, as if wary of what using it might say about their competence. In this way, design choices become entangled with identity negotiation: adopting a playful view can feel like claiming a novice position, while rejecting it can be a performance of expertise.

For designers, the implication is that metaphoric or playful visuals operate in a contested symbolic space. Their success hinges not only on cognitive fit but on whether they align with learners’ desired identities and the norms of the learning context. Supporting interpretive flexibility, allowing learners to adopt or bypass such views without penalty, may be key to sustaining both engagement and perceived legitimacy.

\subsection{Cognitive Ergonomics: Clarity, Load, and Aesthetics}

Participants consistently linked perceived clarity to a sense of cognitive lightness. Designs with minimal arrows, strong spatial partitioning, and stable mappings were praised for reducing the mental effort needed to track relationships:

\begin{myquote2}[P2\_A]
``The memory diagram in the MER visual is very clean. Especially because of the borders. It clarifies what belongs where.''
\end{myquote2}

Conversely, visual clutter, especially dense clusters of overlapping arrows, was described as cognitively abrasive:

\begin{myquote2}[P3\_A]
``I really don’t like when there are just a bunch of arrows pointing everywhere... it kind of ruins the clarity.''
\end{myquote2}

While these preferences resonate with cognitive load theory~\cite{sweller2011cognitive}, they also highlight that ``load'' is not purely a function of visual complexity, it is a negotiated perception shaped by prior representational fluency, aesthetic sensibilities, and even expectations of what    ``good'' instructional design looks like. A diagram that one learner finds elegantly information-rich may, for another, feel visually oppressive.

Some participants framed clear MER layouts as active aids to working memory, ``prosthetics'' they could rely on under time pressure (\textit{``If we were taught this way, it would have been easier to keep track of that in the midterm or the exam''}, P10\_A). Others disengaged entirely from visuals they perceived as ``dated,'' ``messy,'' or ``overdesigned,'' suggesting that affective responses and judgments of modernity are not peripheral, but central, to whether a representation is even worth investing effort in.

In this sense, cognitive ergonomics encompasses both the informational architecture of a visualization and its aesthetic and emotional affordances. A design that minimizes unnecessary mental effort while aligning with learners’ aesthetic preferences and self-image may sustain engagement far more effectively than one that optimizes for clarity in purely technical terms.

\subsection{Shifting Visual Needs Across Learning Trajectories}

Participants’ relationships with visual tools were not fixed; they evolved alongside their conceptual fluency. Early in a topic, especially when confronting unfamiliar abstractions, multiple coordinated views were welcomed as scaffolding, helping to ``fill in the gaps'' between incomplete mental models. Later, as those models solidified, the same visuals shifted into the background, functioning as occasional reference points rather than primary guides.

\begin{myquote2}[P14\_A]
``For starting off learning about linked lists, it’s really helpful to see both the memory model and the visual analogy together. Over time, you can just use the visualization as a rough way of tracing.''
\end{myquote2}

Such accounts suggest that MERs operate most powerfully at transitional moments in learning, when students are still stitching together execution-level details with higher-order conceptual structures. Once those connections feel stable, the cost–benefit of engaging deeply with a visualization changes; some learners prefer to work ``off-model,'' relying on internalized representations, while others keep the tool at arm’s reach for spot checks.

From a design perspective, this underscores the need for \emph{temporal adaptability}: visual tools should support intensive, high-resolution engagement during early encounters, but also remain usable in lighter, more selective modes later on. Importantly, this is not a linear progression, students may cycle back to heavier reliance when encountering new or more complex variants of a concept. In this sense, visualizations are not static scaffolds but dynamic actors whose perceived value is continually renegotiated in relation to shifting epistemic goals, identity positions, and learning contexts.


==> wordgraves-old-dont-read/version0/06limitations.tex <==
\section{Limitations}
\label{sec:limitations}

As with any classroom-based study, our findings should be interpreted in light of several limitations concerning internal, external, and construct validity.

\paragraph{Internal Validity.}
Although our mixed-methods design allowed for rich triangulation, we cannot make strong causal claims about the effects of the visualization system. Students were not randomly assigned to different conditions, and many other course components—assignments, lectures, peer support—may have contributed to the outcomes we observe. While we included start- and end-of-term comparisons and subgroup analyses to identify patterns, these are observational and exploratory. We also cannot rule out demand characteristics in self-report measures, particularly if students inferred our interest in positive experiences.

\paragraph{Construct Validity.}
To measure cognitive load, usability, and clarity, we adapted validated scales (e.g., the Paas mental effort scale~\cite{paas1992}, SUS~\cite{brooke1996sus}), but these may not fully capture students’ nuanced experiences. In particular, the reverse-scored cognitive load scale may obscure asymmetries in interpretation (e.g., what counts as “moderate” effort to one student may differ for another). Likewise, our clarity/helpfulness scale was custom-constructed and internally consistent, but not externally validated. While qualitative data helped elaborate these constructs, further work is needed to develop instruments that better reflect the layered nature of understanding in abstraction-heavy CS contexts.

\paragraph{External Validity.}
This study was conducted in a large, research-intensive university’s CS2 course, where students had relatively strong CS1 backgrounds. Results may not generalize to other contexts—such as smaller institutions, flipped classrooms, or early-stage learners—where instructional structures and learner profiles differ. Our sample was demographically diverse, but still shaped by a selective admissions context, and experiences of clarity, effort, and usability may vary across settings, curricula, or tool


==> wordgraves-old-dont-read/version0/intro.tex <==
% Even after an introductory course, many beginning programmers wrestle with tracing and \emph{conceptually} understanding how variables, references, and control flow interact when code manipulates dynamic data structures such as linked lists or binary-search trees (BSTs) \hlblue{cite cite cite}.  Widely used visualisers like \textit{Python Tutor} expose stack frames and heap objects step-by-step. Yet, novices frequently fail to generalize to higher-level models and report feeling overwhelmed by granular memory diagrams \cite{guo2013online,sorva2013review}.  These challenges are exacerbated for learners who arrive with little or no prior programming experience--a factor that predicts persistent grade gaps across CS1–CS2 and shapes self-efficacy, engagement, and retention \cite{bui2023prior, sibia2024examining}.




==> wordgraves-old-dont-read/version0/old-04results.tex <==
\section{Results}
\label{sec:results}
\hlpink{Naaz: I still need to add more connections and critical thoughts to the codes, but for now I'm looking at whether the broader connections make sense!}

\subsection{RQ1--Student Experience with MER Visualizations}

We first examined how students experienced the multi-representation (MER) visualizations in CS2, focusing on perceived clarity, affective response, and feature-specific feedback.

\subsubsection{Perceived Clarity and Helpfulness}
Quantitatively, students rated the MER visualizations as significantly clearer and more helpful than neutral. On a five-point Likert scale, the composite \emph{Clarity/Helpfulness} score averaged $M=3.83$, $SD=0.74$, well above the midpoint of 3, $t(306)=19.66$, $p<.001$, Cohen’s $d=1.12$ (Table~\ref{tab:clarity}).

\input{tables/clarity}

Students' qualitative responses further indicated themes about what students found helpful in the visuals.  The most common themes emphasized visual clarity and intuitive flow. Students often contrasted the visualizations favorably against dense text or less interactive tools:

\begin{myquote2}
``The visualization for each data type is very useful for me to directly understand the structure of each data type. The highlight in text, memory and data type structures makes the code easier to follow.''
\end{myquote2}
% \begin{myquote2}
% ``Very easy and has many ways of us to watch.''
% \end{myquote2}
In the quote above, in addition to talking about the ease of use, the student also notes finding the many ways of viewing the visuals (i.e. the multi-representational design) helpful. 

% \begin{myquote2}
% ``Just easier than reading whole paragraphs of text.''
% \end{myquote2}
% In this case, the student found the visual easier than reading paragraphs of text. -- Something about using the visual for a different purpose and cite. 

Students also appreciated the alignment between the visual layout and their conceptual models:
\begin{myquote2}
``Very clear flow/top-down structure. Actually follows the theoretical structure of the ADT from how a human would perceive it.''
\end{myquote2}

These sentiments align with the quantitative results and underscore the importance of representational clarity in facilitating conceptual understanding. \hlpink{links to theory}.

\subsubsection{Affective Responses}

Beyond instructional utility, students also reported a range of affective impressions. Survey responses showed a moderately high mean enjoyment rating ($M=3.82$, $SD=0.94$). Longitudinal analyses (n=283) revealed that affect improved over time: Wilcoxon signed-rank tests showed small but significant increases in perceived usefulness ($W=5{,}531$, $p=.006$) and enjoyment ($W=5{,}509$, $p=.014$) from CS1 to CS2.

Open-ended responses echoed these positive engagement ratings. Many students described the visualizations as enjoyable, engaging, or even confidence-boosting:
\begin{myquote2}
``These visualizations will help me learn to visualize a program so that I can visualize it without the visualizer during a computer science test.''
\end{myquote2}

\begin{myquote2}
``It was easy to understand and I didn’t feel as lost as I usually do.''
\end{myquote2}

However, not all responses were positive. A smaller subset of students reported frustration, particularly with visual clutter or overly simplified representations:

\begin{myquote2}
``Sometimes the memory visualization gets a little clogged, and it can be difficult to see or interpret.''
\end{myquote2}

\begin{myquote2}
``The UI was overwhelmingly it was shown too many things at once making it hard to follow.''
\end{myquote2}
These tensions highlight the tradeoff between conceptual richness and cognitive load, which is taken up in RQ2.

\subsubsection{Feature-Specific Benefits and Limitations}
Open-ended feedback revealed specific features that students found especially helpful:

\textbf{Process-oriented flow}: Step-by-step tracing was the most frequently praised design element.
\begin{myquote2}
``Being able to go step by step and visualize what each line of code truly does. It helps truly understand more complex topics like BSTs.''
\end{myquote2}

\textbf{Color and highlighting}: These visual cues helped students track dynamic changes.
\begin{myquote2}
``Highlighted areas made it easier to follow, and to know when stack frame or something else is deleted.''
\end{myquote2}

% \begin{myquote2}
% ``Yes, the different versions of visualizations seems beneficial.''
% \end{myquote2}

\textbf{Interactivity and pacing control}:
\begin{myquote2}
``Being able to go step by step and visualize what each line of code truly does. This helps truly understand more complex topics like BSTs.''
\end{myquote2}
% \begin{myquote2}
% ``the reset and run all steps features were super useful to know the before and after.''
% \end{myquote2}

These features were frequently cited as supporting understanding, clarity, and learner autonomy.

Yet, students also identified several limitations:

\textbf{Overwhelm and visual clutter}:
\begin{myquote2}
``Since there were 3 screens to keep track of simultaneously, it was confusing and cumbersome to understand.''
\end{myquote2}

\textbf{Styling and legibility issues}:
\begin{myquote2}
``The code editor has no colours. it makes code harder to read.''
\end{myquote2}

\textbf{Non-interactive limitations}:
\begin{myquote2}
``The IDE on the left didn’t allow changes to the code. It would be better for experimentation.''
\end{myquote2}

\textbf{Lack of depth or scaffolding}:
% \begin{myquote2}
% ``If wanting to use it as a more rigorous tool, it would not help.''
% \end{myquote2}

\begin{myquote2}
`` the code itself wasn't extremely helpful since it was very simple. I would only recommend for people who have learned the concept and are still confused with the basics.''
\end{myquote2}

This criticism underscores opportunities for refinement, especially around interactivity and visual design.

\begin{takeawaybox}
Students valued the visual clarity, pacing, and representational diversity of the MER interface. However, feedback also pointed to areas for improvement—including interactivity, layout density, and visual styling.
\end{takeawaybox}

\subsection{RQ2--Cognitive Load and Usability}

We next examined the cognitive and usability demands of the MER visualization system, focusing on mental effort, navigation experience, and perceived usability. Quantitative results showed that the system was broadly usable, with students reporting moderate cognitive effort. Open-ended feedback provided more detail about when and why effort increased.

Students reported moderate levels of mental effort while using the MER visualizations ($M = 3.03$, $SD = 0.72$, on a reversed five-point scale where higher scores reflect \emph{lower} effort). While these ratings do not indicate a strong reduction in perceived cognitive load, they suggest that the interface did not overwhelm students despite the abstract content. A longitudinal comparison revealed a significant reduction in reported effort from CS1 to CS2 ($W = 2{,}191$, $p < .001$), hinting at improved cognitive efficiency over time.

Qualitative feedback offered a more nuanced view. While many students described the pacing and visual clarity as supportive (see RQ1), others flagged moments of difficulty. These concerns often emerged when visual complexity spiked—such as during recursive calls or structural transformations that led to large or abrupt diagram changes:

\begin{myquote2}
``Steps that changed a lot required me to sit and stare for a while to understand how it went from the previous to the next.''
\end{myquote2}

Other comments pointed to interpretive effort required to coordinate the three panes:

\begin{myquote2}
``It sometimes takes mental effort to connect what’s happening across the three parts of the visualization—especially when it’s all changing at once.''
\end{myquote2}

These reflections suggest that representational richness comes with tradeoffs: although abstraction-focused visuals can aid understanding, they may introduce interpretive load when transitions are rapid or poorly segmented.

\subsubsection{Perceived Usability and Interface Design}

Students generally rated the system as easy to use. The composite \emph{Ease of Use} score averaged $M=3.58$, $SD=0.70$, significantly above the neutral midpoint ($t(306)=14.65$, $p<.001$), with a medium-to-large effect size ($d=0.84$). This supports H3 and suggests that the interface supported intuitive navigation and use.

In open-ended responses, several students emphasized features that enhanced usability—particularly the ability to scrub through steps, reset views, and replay segments. However, a smaller subset described persistent friction across five dimensions:

\begin{itemize}
    \item \textbf{Layout density and clutter}: Some students found the tri-pane design visually overwhelming, especially on small screens or during complex transitions.
    \item \textbf{Navigation limitations}: Difficulty skipping to relevant execution steps or fine-tuning playback speed reduced efficiency.
    \item \textbf{Interactivity constraints}: Students noted the inability to modify code or experiment with parameters within the tool itself.
    \item \textbf{Styling and accessibility issues}: Visual contrast and screen-fitting problems were occasionally cited, particularly on mobile devices.
    \item \textbf{Conceptual oversimplification}: A few students felt the system lacked depth for more advanced conceptual exploration.
\end{itemize}

Unlike the clarity or affect ratings in RQ1, usability critiques often referred to system-level concerns: visual congestion, control limitations, or styling choices that interfered with smooth interaction. Although these issues were not widespread, they offer concrete targets for iterative design improvement.

\input{tables/features}

\begin{takeawaybox}
Students rated the interface as broadly usable and cognitively manageable. Still, feedback pointed to challenges with visual density, pacing, and interactivity—highlighting key design tradeoffs in MER-based tools.
\end{takeawaybox}


\subsection{RQ3--Learner Characteristics and Perceptions}
We next examined whether students’ experiences of the MER visualizations varied by key learner characteristics: language background, prior programming experience, and final course grade. We focused on three outcome measures—clarity/helpfulness, cognitive load, and ease of use—using independent-sample $t$-tests and ANOVA/Kruskal–Wallis tests as appropriate. Results are summarized in Table~\ref{tab:subgroups}.

\paragraph{Language background.}
Non-native English speakers rated the MER visualizations significantly clearer ($M=4.07$) than native speakers ($M=3.86$), Welch’s $t(129.4) = -2.32$, $p = .022$, $d = 0.28$, indicating a small but meaningful difference. No significant differences emerged in perceived cognitive load or ease of use. This suggests that the visual format may have been especially supportive for students navigating a second language, consistent with prior work showing the value of visual scaffolds in reducing linguistic barriers.

\paragraph{Prior programming experience.}
Students with no prior experience reported similar clarity ($M=3.97$) to their peers with experience ($M=3.89$), with no significant differences on any of the three scales ($p > .05$). This suggests that the MER system was accessible regardless of prior exposure to programming.

\paragraph{Final course grade.}
To explore whether overall course performance influenced student perceptions, we compared clarity/helpfulness scores by final grade band (A, B, C or lower). No significant differences were observed, indicating that students across performance levels found the visualizations similarly helpful.

\paragraph{Gender.}
Although not a focal variable for RQ3, we include gender comparisons for completeness. No significant differences were found across any measure (ANOVA $F = 0.08$–$0.05$, $p > .75$).

\input{tables/subgroups}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Other interesting quotes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\comment{
Being able to visualize codes helped me learn about them in a more 
intuitive manner. It speeds up the take it takes to have that click in 
my head when picking up new content.
}

==> wordgraves-old-dont-read/version0/old-old-04results.tex <==
\section{Results}
\label{sec:results}

\subsection{Preliminary Analyses}
\paragraph{Scale Reliability.} Internal‐consistency reliability was strong for each composite scale: \emph{Clarity/Helpfulness} ($\alpha=.89$), \emph{Cognitive Load} ($\alpha=.87$), and \emph{Ease of Use/SUS} ($\alpha=.84$). Item–total correlations were all $\ge .52$.

\paragraph{Data Screening.} Of the 440 students enrolled in CS2, 307 (69.8\%) contributed complete end‑of‑term questionnaire data suitable for quantitative analysis. Listwise deletion of incomplete rows left $n=307$ for RQ1–RQ2 analyses and $n=283$ for longitudinal CS1–CS2 comparisons.

\subsection{RQ1—Helpfulness \& Clarity}
We first examined students’ perceptions of the visuals' clarity and helpfulness. Students judged the MER visuals to be clear and helpful. On a five‑point Likert scale, the composite \emph{Clarity} score averaged $M=3.83, (SD=0.74)$, significantly above the neutral midpoint of~3, $t(306)=19.66$, $p<.001$, Cohen’s $d=1.12$. This result supports H1, indicating that students perceived the visuals as meaningfully clearer than neutral.

\begin{table}[t]
\centering
\caption{Descriptive statistics and one-sample $t$-tests for overall scales (RQ1--RQ2).}
\label{tab:clarity}
\begin{tabular}{lcccccc}
\toprule
Scale & $n$ & $M$ & $SD$ & Midpoint & $t$ & $d$ \\
\midrule
Clarity/Helpfulness & 307 & 3.83 & 0.74 & 3 & 19.66*** & 1.12 \\
Cognitive Load$^{\dagger}$ & 307 & 3.03 & 0.72 & 3 & 0.73 & 0.04 \\
Ease of Use (SUS proxy) & 307 & 3.58 & 0.70 & 3 & 14.65*** & 0.84 \\
\bottomrule
\multicolumn{7}{l}{\footnotesize $^{\dagger}$Higher scores indicate \emph{lower} perceived mental effort after reverse-coding. ***$p<.001$.} \\
\end{tabular}
\end{table}


\begin{takeawaybox}
Students generally rated the abstraction-oriented MER visuals as clear and helpful.
\end{takeawaybox}

\subsection{RQ2—Cognitive Load \& Usability}
\hlpink{Needs to be rewritten: noting from our discussion from last time: I don't have a cognitive load benchmark and I can't compare to the neutral value}

We next assessed perceived mental effort and usability. Mean mental effort ratings ($M=3.03$ on a 5‑point reversed scale) did not differ from the neutral benchmark, $t(306)=0.73$, $p=.467$, suggesting no evidence for reduced load. This fails to support H2. By contrast, students rated the system as easy to use ($M=3.58$), significantly exceeding the neutral benchmark, $t(306)=14.65$, $p<.001$, $d=0.84$. This supports H3 and suggests that the interface was broadly usable. Notably, cognitive load remained stable even as visuals became more abstract, suggesting effective load management over time.

\begin{takeawaybox}
Usability was high, but cognitive load remained neutral—suggesting the visuals did not reduce mental effort, but also did not overwhelm students, even as concepts grew more complex.
\end{takeawaybox}

\subsection{RQ3—Learner Differences}
We then explored whether perceptions of the MER visuals varied by learner background (Table~\ref{tab:subgroups}).
\begin{itemize}[leftmargin=0.6cm]
\item \textbf{Language background.} Non‑native English speakers rated the visuals significantly clearer ($M=4.07$) than native speakers ($M=3.86$), Welch’s $t(129.4)=-2.32$, $p=.022$, $d=0.28$. No significant differences emerged in cognitive load or usability.
\item \textbf{Prior programming experience.} Students with no prior experience reported equivalent clarity, ease of use, and cognitive load scores to their peers with any prior experience (all $p>.05$).
\item \textbf{Gender.} Ratings were statistically indistinguishable between men and women across all scales (ANOVA $F=0.08$, $p=.778$; Kruskal–Wallis $H=0.01$, $p=.933$).
\end{itemize}

\begin{table}[t]
\centering
\caption{Subgroup comparisons for clarity, cognitive load, and usability (RQ3).}
\label{tab:subgroups}
\begin{tabular}{llccc}
\toprule
Subgroup & Measure & Group Means (SD) & $t$/stat & $p$ \\
\midrule
\textbf{Language (Native vs. Non-native)} \\
\quad Clarity           & 3.86 vs 4.07 (0.75 / 0.71)   & $t=-2.32$ & .022* \\
\quad Cognitive Load    & 3.16 vs 3.06 (0.72 / 0.84)   & $t=1.03$  & .305 \\
\quad Ease of Use       & 3.62 vs 3.75 (0.70 / 0.63)   & $t=-1.67$ & .097 \\
\addlinespace
\textbf{Prior Experience (Any vs. None)} \\
\quad Clarity           & 3.89 vs 3.97 (0.72 / 0.79)   & $t=-0.89$ & .377 \\
\quad Cognitive Load    & 3.19 vs 3.01 (0.72 / 0.81)   & $t=1.93$  & .055 \\
\quad Ease of Use       & 3.64 vs 3.68 (0.67 / 0.70)   & $t=-0.44$ & .664 \\
\addlinespace
\textbf{Gender (Men vs. Women)} \\
\quad Clarity           & 3.90 vs 3.94 (0.71 / 0.77)   & $F=0.08$  & .778 \\
\quad Cognitive Load    & 3.14 vs 3.11 (0.72 / 0.81)   & $F=0.02$  & .885 \\
\quad Ease of Use       & 3.65 vs 3.67 (0.66 / 0.72)   & $F=0.05$  & .826 \\
\bottomrule
\multicolumn{5}{l}{\footnotesize *$p<.05$. Values reflect Welch's $t$ or one-way ANOVA/Kruskal–Wallis as applicable.}
\end{tabular}
\end{table}
\newimage{figures/lang-ratings.png}{Perceived helpfulness of visuals by first language background.}{lang-ratings}

\newimage{figures/pe-ratings.png}{Perceived clarity/helpfulness by prior programming experience.}{pe-ratings}

\newimage{figures/mer-grades.png}{Clarity/helpfulness ratings by final course grade.}{mergrades}


\begin{takeawaybox}
Perceptions of clarity and usability were broadly consistent across gender and prior experience. Non-native English speakers rated the visuals slightly clearer, indicating inclusive benefits.
\end{takeawaybox}

\subsection{RQ4—Affect Across the Two‑Course Sequence}
Finally, we examined whether students’ attitudes toward the visuals changed over time. For the matched cohort ($n=283$) who completed both CS1 and CS2 surveys, Wilcoxon signed‐rank tests indicated small but significant improvements in two enjoyment items: visual usefulness ($W=5{,}531$, $p=.006$) and perceived helpfulness ($W=5{,}509$, $p=.014$). Students also reported a reduction in self‑reported mental effort on tree/linked‑list tasks ($W=2{,}191$, $p<.001$). These findings suggest modest gains in affective response and reduced effort with continued use. Other common items, including ease of use and overall clarity, did not change significantly across terms (all $p>.05$), indicating that initial positive impressions were sustained.

\newimage{figures/diff.png}{Difference scores for CS1 and CS2 respondents on shared survey items.}{diff}

\begin{takeawaybox}
Affective responses improved modestly over time, with students reporting greater enjoyment and reduced effort, which highlights the potential of visuals for sustained engagement.
\end{takeawaybox}

==> wordgraves-old-dont-read/version1/06discussion.tex <==
\section{Discussion}
\label{sec:discussion}
Program visualizations are often framed as neutral scaffolds, bridging abstraction, reducing cognitive load, and clarifying execution for novices. Our findings complicate this view. Students engaged with these tools as \emph{negotiated resources}: adopting, adapting, or resisting them in ways that reflected not just the demands of the task, but their interpretive repertoires, self-conceptions, and sense of belonging. In this way, visualizations influenced not only how students understood programs, but how they positioned themselves as learners.  

We interpret these dynamics through four interlinked lenses: the situated utility of multiple external representations (MERs), epistemic calibration as an interpretive practice, the sociocultural politics of visual legitimacy, and the evolution of representational repertoires over time.

\subsection{MERs as Situated and Contingent Supports}
Ainsworth’s DeFT framework~\cite{ainsworth2006deft} treats coordination, complementarity, and constraints as central to MER effectiveness. Our data suggest an additional dimension: \emph{contingency}. Students did not engage all views equally or consistently; they shifted between code, memory diagrams, and metaphors based on local task demands and personal reasoning style.  

The same affordance, such as synchronized highlighting, anchored abstraction for one student but created distraction for another. What made the difference was not simply the intrinsic complexity of the visual but whether it offered \emph{narrative coherence}: a sequence or spatial logic that fit the learner’s existing cognitive ``story'' of program execution.  

This implies that load reduction is not solely a matter of minimizing information density; it is also about designing for multiple plausible interpretive arcs. MERs must anticipate that coherence will vary across learners, and that features which scaffold one interpretive pathway may create friction for another.

\subsection{Epistemic Calibration as Interpretive Strategy}
While ICAP~\cite{chi2009active} distinguishes between constructive and interactive engagement, our participants demonstrated that such modes can be strategically toggled in real time. Many began by mentally tracing code, then consulted a visualization for verification; others reversed this order when mental energy or confidence was low, effectively outsourcing part of the reasoning to the external tool.  

We call this \emph{epistemic calibration}: the ongoing metacognitive judgment of when to rely on internal simulation versus external representation. Calibration decisions were often moment-to-moment, shaped by perceived task difficulty, error likelihood, and available cognitive resources. This practice aligns with distributed cognition~\cite{card1999readings} in that the external artifact extends thinking, but only when deliberately integrated into the learner’s reasoning cycle. It also parallels trust-in-automation dynamics~\cite{lee2004trust}, where users must decide when to accept, verify, or override a system’s guidance.  

Designing for calibration means offering learners fine-grained control over granularity, pacing, and viewpoint, enabling them to shift the epistemic ``weight'' between self and system as circumstances change. Poorly designed tools risk constraining this flexibility, either by overwhelming learners with fixed, high-detail views or by oversimplifying in ways that prevent deeper inspection. Calibration-aware design would therefore provide scaffolds that are both accessible and relinquishable, supporting transitions between dependence, co-reasoning, and independence without penalty or friction.


\subsection{The Politics of Visual Legitimacy}
Visuals carry aesthetic and cultural signals about what counts as ``real'' computer science. Choices of style, metaphor, and tone are not neutral; they position the learner in relation to perceived disciplinary norms. Playful or metaphorical designs, boxes for memory, analogies to everyday routines, lowered anxiety and anchored abstraction for some. For others, the same designs risked infantilization or signaled misalignment with the seriousness of university-level work.

These tensions are not mere matters of taste; they are part of the \emph{identity work} students perform when deciding which resources to embrace. As in other epistemic cultures~\cite{cetina1999epistemic}, legitimacy is conferred through alignment with community values and aesthetics. A single learner could describe a metaphor as both ``helpful'' and ``too far from the code'' in the same interview, revealing moments of affective dissonance where cognitive benefit was weighed against perceived social cost.

Such negotiations have implications for inclusion: a design language that feels accessible to some may signal marginality to others, reinforcing boundaries about who ``belongs.'' Legitimacy is also temporally contingent; visuals that feel appropriate early in a learning trajectory may later be rejected as overly simplified once fluency increases.  

Acknowledging this politics means treating style and tone not as incidental, but as part of the representational contract between tool and learner. Beyond simple customization, designers might consider \emph{legitimacy-aware} modes, allowing learners to shift visual tone, metaphor, and granularity, while making these options visible in ways that avoid marking one choice as remedial and another as advanced. This framing invites future work on how visual legitimacy is constructed, contested, and re-negotiated across diverse learning contexts.

\subsection{Representational Resonance and Trajectories}
Students gravitated toward visuals that ``thought'' like they did, whether in the spatial logic of a self-drawn diagram or the analogy structures they habitually used. We term this \emph{representational resonance}: an alignment between a tool’s representational grammar and the learner’s established habits of reasoning, diagramming, or narrating program behavior. When resonance occurred, translation costs were low; the visual could be read almost as an extension of the learner’s own notional machine~\cite{sorva2013review}.  

Resonance, however, was neither universal nor static. What fit one learner’s cognitive style could feel awkward or alien to another, and what resonated early in a topic could later feel redundant or even constraining. Participants often described a trajectory in which they initially relied heavily on multiple coordinated views to assemble a mental model, then shifted to selective, lightweight consultation once that model stabilized. In some cases, resonance weakened over time as learners developed new abstractions that the original visual grammar did not capture.  

Designing for trajectories means supporting this fluidity and enabling tools to shift between explanatory richness and minimalist efficiency without losing coherence. This may involve modular representations, user-adjustable abstraction levels, or adaptive systems that can match visual framing to the learner’s evolving repertoire. By treating resonance as a moving target rather than a fixed property, designers can better sustain engagement across both early scaffolding and later expertise-building phases.

\medskip
Across these lenses, visualizations emerge not as static aids but as \emph{dynamic actors} in a negotiation between design intent and learner appropriation. They succeed when they are adaptable, technically, cognitively, and culturally, supporting multiple interpretive pathways, enabling epistemic calibration, and affirming diverse learner identities.  

Future work could explore how such adaptability might be made learner-controllable in real time, and how systems might surface not just program state but metacognitive cues to support calibration and identity alignment.

